GraphReader: Building Graph-based Agent to Enhance Long-Context Abilities of Large Language Models

Long-context capabilities are essential for large language models (LLMs) to tackle complex and long-input tasks. Despite numerous efforts made to optimize LLMs for long contexts, challenges persist in robustly processing long inputs. In this paper, we introduce GraphReader, a graph-based agent system designed to handle long texts by structuring them into a graph and employing an agent to explore this graph autonomously. Upon receiving a question, the agent first undertakes a step-by-step analysis and devises a rational plan. It then invokes a set of predefined functions to read node content and neighbors, facilitating a coarse-to-fine exploration of the graph. Throughout the exploration, the agent continuously records new insights and reflects on current circumstances to optimize the process until it has gathered sufficient information to generate an answer. Experimental results on the LV-Eval dataset reveal that GraphReader, using a 4k context window, consistently outperforms GPT-4-128k across context lengths from 16k to 256k by a large margin. Additionally, our approach demonstrates superior performance on four challenging single-hop and multi-hop benchmarks.

==> content/cache/0_abstract_cache_20240619.tex <==
\begin{abstract}

% With the advancement of large language models (LLMs), there is an increasing demand for long-context capabilities to tackle more complex tasks. Despite numerous efforts to optimize LLMs for long contexts, challenges persist in robustly processing long inputs.
Long-context capabilities are essential for large language models (LLMs) to tackle complex and long-input tasks. Despite numerous efforts made to optimize LLMs for long contexts, challenges persist in robustly processing long inputs.
% In this paper, we introduce \ourmethod, a graph-based agent system designed to enhance long-range dependencies by structuring long texts into a graph. This system employs an agent that autonomously explores the graph. Upon receiving a question, the agent first undertakes a step-by-step analysis and devises a rational plan. It then invokes a set of predefined functions to read node content and neighbors, facilitating a coarse-to-fine exploration of the graph. Throughout this exploration, the agent continuously records new insights and reflects on current circumstances to optimize the process until it has gathered sufficient information to generate an answer.
In this paper, we introduce \ourmethod, a graph-based agent system designed to handle long texts by structuring them into a graph and employing an agent to explore this graph autonomously. Upon receiving a question, the agent first undertakes a step-by-step analysis and devises a rational plan. It then invokes a set of predefined functions to read node content and neighbors, facilitating a coarse-to-fine exploration of the graph. Throughout the exploration, the agent continuously records new insights and reflects on current circumstances to optimize the process until it has gathered sufficient information to generate an answer.
% Experimental results on the LV-Eval dataset reveal that \ourmethod, employing a 4k context window, significantly outperforms GPT-4, which utilizes a 128k context window, across various context lengths up to a maximum of 256k. Moreover, our approach shows superior performance on four challenging single-hop and multi-hop benchmarks.
Experimental results on the LV-Eval dataset reveal that \ourmethod, using a 4k context window, consistently outperforms GPT-4-128k across context lengths from 16k to 256k by a large margin. Additionally, our approach demonstrates superior performance on four challenging single-hop and multi-hop benchmarks.
\end{abstract}

==> content/cache/1_intro_cache_20240619.tex <==
%-----注释过多的版本放在了cache的intro cache2中

\section{Introduction}

\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{0.15cm}  
    % \setlength{\belowcaptionskip}{-0.2cm}
    \includegraphics[width=0.99\linewidth]{source/figure1.pdf}
    \caption{Performance on LV-Eval at 5 context length levels. GraphReader outperforms existing open-sourced and closed-source models while demonstrating a scalable performance in very long contexts. In contrast, other models exhibit a significant decrease in performance as context length increases.}
    \label{fig: motivation}
    \vspace{-5mm}
\end{figure}

Large language models~(LLMs) have made great progress on natural language understanding and generation~\citep{Zhao-2023-arxiv-survey}. However, transformer-based LLMs still struggle in handling long contexts due to the limitation of context window and memory usage. 


Current techniques for solving the long-context tasks of LLMs can be divided into two perspectives: 1) Model-level, which includes finetuning with modified positional embeddings~\cite{chen2023extending,zhu2023pose,peng2023yarn,ding2024longrope}, and applying transformer variants with modified attention mechanisms~\citep{dai2019transformer,munkhdalai2024leave,gu2023mamba}; 2) Agent-level, \aka employing retrieval-augmented LLM or agent to process long contexts with a limited context window LLM~\cite{nakano2021webgpt,lee2024human}.

However, model-level methods typically train LLMs with target length texts, posing challenges in constructing training datasets and incurring high training costs~\cite{zhu2023pose}. Additionally, long-context LLMs optimized with these methods tend to overlook crucial details in long contexts, known as ``lost in the middle''~\cite{liu2024lost}, limiting their ability to address complex tasks, such as multi-hop questions. Agent-level approaches transform input text into a tree~\citep{chen2023walking} or paginated pages~\citep{lee2024human}, failing to capture multi-hop and long-range dependencies, thus limiting their effectiveness on very long contexts, as shown in Figure~\ref{fig: motivation}.


To address these issues, we propose a graph-based agent named \textbf{\ourmethod}. As illustrated in Figure~\ref{fig: ourmethod}, \ourmethod first segments long texts into discrete chunks, extracts essential information, and compresses these into key elements and atomic facts. These key elements and facts are then used to construct a graph with nodes representing key elements and their associated atomic facts. This graph structure effectively captures long-range dependencies and multi-hop relationships within long text.
Subsequently, \ourmethod autonomously explores this graph using predefined functions, guided by a step-by-step rational plan. Based on a given question, the agent progressively accesses information from coarse key elements and atomic facts to detailed original text chunks, taking notes and reflecting until it gathers sufficient information to generate an answer.
In summary, our main contributions are threefold:

\begin{itemize}[leftmargin=4mm]
\vspace{-0.08cm}
\item We introduce \ourmethod, a novel agent system designed to organize long texts into a graph structure, leveraging predefined functions and notebook to facilitate planning and reflection during exploration.%, thereby enabling the effective handling of long-context tasks.

\item \ourmethod establishes a scalable long-context capability based on a 4k context window, demonstrating performance that is comparable to or surpasses GPT-4 with a 128k context window across varying context lengths.

\item Extensive experiments conducted on four challenging benchmarks demonstrate that \ourmethod achieves superior performance in complex single-hop and multi-hop QA tasks.
\end{itemize}






% draft
% Large language models~(LLMs) have made great progress on natural language understanding and generation~\citep{Zhao-2023-arxiv-survey}. However, transformer-based LLMs still struggle in handling long contexts due to the limitation of context window and memory usage. 


% Current work primarily implemented four strategies to improve the capability of LLMs in processing long context: finetuning with modified positional embeddings~\cite{chen2023extending}, training directly on long-context data, applying transformer variants with modified attention mechanisms~\citep{} and employing agent to process long contexts with the limited context window LLM~\cite{wu2020memformer, lee2024human}. Despite the effectiveness, there are several shortcomings in these four methods. For the first three methods, they typically rely on training with texts of the target length~\citep{}, which results in the challenge of constructing training datasets and incurs high training costs. Furthermore, long-context LLMs optimized with these three methods tend to overlook crucial details in long contexts, \aka lost in the middle~\cite{liu2024lost}, limiting handling multi-hop problems of long-context LLMs. For approaches that employ agents to handle long context input, typically, they transform the input text into paginated pages~\citep{lee2024human} or a tree~\citep{chen2023walking}, which fail to support the agents in capturing multi-hop and long-range dependencies, thus limiting the effectiveness of these methods.


% \ignore{
% We draw inspiration from the cognitive processes that humans employ for reading comprehension of long texts in the real world. When tackling long-text QA problems, humans typically divide the process into four-stage process:(1) understanding the question and reasoning the key information to answer it; (2) identifying several key terms based on the question; (3) searching the content in long text related to the selected key terms; and (4) integrating the gathered information to generate the response of the question. Drawing on these insights, we propose \textbf{\ourmethod}, a novel approach that organizes information from long text into a graph, and employ an agent to travel on the graph based on the input question to search and summarize information within the graph as needed. Specifically, we first segment long texts into chunks, followed by extracting key elements and atomic facts from them. Then we construct a graph with these key elements as nodes and incorporating atomic facts and original chunks as their content to model the global information of input long text. Lastly, our \ourmethod performs a depth-first search from the selected initial nodes. It dynamically reads, accumulates memories, and concludes, responding interactively to user input until it gathers enough information to fulfill the given question.
% }

% To address these issues, in this paper, we propose a method that extracts critical information from long texts and organizes it into a graph, subsequently employing an agent for interactive reading input long text and follow user instructions, namely \textbf{\ourmethod}. Specifically, as illustrated in Figure~\ref{}, our method comprises two main stages: Firstly, we divide the long text into multiple chunks, followed by extracting key information from these chunks. Secondly, we construct a graph wherein key information as nodes and incorporating original chunks as nodes' content. Through this structure, we achieve modeling the long-range dependencies and multi-hop relation within the key information of input long text. Secondly, the \ourmethod employs pre-planned strategies to conduct a depth-first search from multiple initial nodes within the graph. Based on user input, it interactively reads, generates memory, responding interactively to user input until it gathers enough information to fulfill the given question.


% In summary, our main contributions are as follows:
% \begin{itemize}[leftmargin=4mm]
% \vspace{-0.08cm}
% \item We propose \ourmethod, a novel agent system that utilizes a memory mechanism and graph-driven traversal to handle long-context tasks with limited context window LLMs.
% \vspace{-0.08cm}
% % \item Our approach, leveraging smaller language models, approximates and even surpasses the performance of GPT-4-turbo with a 128K context window, demonstrating a David-versus-Goliath dynamic, as well as scalability in handling text length.
% \item In addressing long text issues, our approach leverages the LLM with 4K context window, achieving performance on par with or even exceeding that of LLM with 128K context window.
% \vspace{-0.08cm}
% \item Experimental results show that \ourmethod achieves superior performance in single-hop and multi-hop long context tasks. Notably, Info-Graph Agent achieves a xx of xx on HotpotQA, xx on 2WikiMultiHopQA, and xx on MuSiQue based on GPT-4 with 4K context window, even outperforming GPT-4-turbo with 128K context window.
% \end{itemize}


==> content/cache/2_related_cache_20240619.tex <==
\vspace{-0.35cm}
\section{Related Work}
\vspace{-0.1cm}
\paragraph{Long-Context LLMs}


% Developing larger models with increasingly larger window sizes has been a notable trend. 
% Various methods have been developed to extend the window of LLMs, primarily including training on target long-context data~\citep{chen2023extending,fu2024data,bai2024longalign}, ~\citep{chen2023extending,ding2024longrope,peng2023yarn,zhu2023pose}, and transformer variants with modified attention mechanisms~\citep{dai2019transformer,wu2020memformer,gu2023mamba,munkhdalai2024leave}. However, enlarging the context window size tends to show information loss,
% which is shown in the ``lost in the middle'' phenomenon~\cite{liu2024lost}.
% % referring to the dramatic decline in accuracy when the correct information is located in the middle. 
% Our methodology builds upon these existing techniques to extend the maximum text length and enhances the models' comprehension of lengthy texts without model modifications or additional training phases.
% Various methods have been developed to extend the context window of LLMs. 
Recent efforts~\citep{chen2023extending,ding2024longrope,peng2023yarn} have focused on positional interpolation (PI) to enhance long-context capabilities. However, these methods require training on full-length texts, leading to significant increases in data and training costs~\cite{chen2023longlora,fu2024data,bai2024longalign}. Thus, PoSE~\cite{zhu2023pose} and SkipAlign~\cite{wu2024long} investigate data skip strategy, but tend to neglect detailed information in long texts~\cite{liu2024lost}. Furthermore, despite how extensively the context window is expanded, it remains constrained by a predefined fixed length. To address these limitations, transformer variants with modified attention mechanisms have been proposed \citep{dai2019transformer,gu2023mamba,munkhdalai2024leave}. However, these models are prone to losing earlier information.



\paragraph{Retrieval}
% Retrieval refers to extracting relevant document fragments from a long context. The most typical one is the Retrieval Augmented Generation (RAG) technique, which extracts task-related information from a large database of documents~\citep{chen2017reading,izacard2020leveraging}. A variety of different retrieval granularity appears in existing research, ranging from tokens~\citep{khandelwal2019generalization} or entities~\citep{fevry2020entities,de2021mention} to chunk or larger text blocks~\citep{lee2024human}, as well as different retrieval methods (e.g.,  BM25~\citep{rasooli-tetrault-2015}, learning–based strategies~\citep{khattab2020colbert,sachan2023questions,sun2021long}.
% % and using LLMs as retrievers recently~\citep{sun2021long,yu2022generate}.
% % However, these traditional retrieval methods might not be suitable for complex queries. 
% However, existing works are prone to overlooking detailed information and struggle with dealing with long-range dependencies.
% In contrast, our method exhibits greater flexibility in extracting the necessary information fragments and has an excellent performance on complex queries.

Retrieval Augmented Generation (RAG) leverages an extensive database of documents to extract task-related information that aids in response generation. Many efforts investigate various levels of retrieval granularity, including tokens \citep{khandelwal2019generalization}, entities \citep{fevry2020entities,de2021mention}, and chunks \citep{LlamaIndex, LangChain}. Other approaches have explored diverse retrieval methods, such as BM25 \citep{rasooli-tetrault-2015} and learning-based strategies \citep{khattab2020colbert,sachan2023questions,sun2021long}. Despite its capabilities, RAG faces challenges in addressing complex questions due to difficulties in developing robust decision-making mechanisms. In contrast, we employ agents that use planning and reflection to gather essential information, effectively tackling complex problems.




\paragraph{Agent for Retrieval}

% LLMs  can be effectively utilized to deal with long-context data interactively~\cite{chen2023walking,sarthi2024raptor}. 
% The WebGPT~\citep{nakano2021webgpt} simulates human actions to search for the requested answer on the internet. 
% % The MemWalker~\citep{chen2023walking} finds supporting facts by browsing the hierarchical structure of summaries. 
% % The PEARL~\citep{sarthi2024raptor} proposes action plans for better long-document comprehension through iterative prompting.
% The KGP~\citep{wang2024knowledge} designs an LLM-based graph traversal agent that searches on the graph, and there are also many similar graph-based agents for retrieval~\citep{sun2023think,mavromatis2024gnn,edge2024local}. The ReadAgent~\citep{lee2024human} proposes a human-inspired LLM agent that generates gist memories and looks up information as needed. However, these methods struggle to capture critical information across various granularities and long-distance dependencies.

Recent work has increasingly leveraged LLMs as agents to tackle complex problems, utilizing their strong planning and reflection abilities \cite{yao2022react,park2023generative}. These abilities have been applied to complex tasks such as function call \cite{li2023chain} and KGQA \cite{sun2023think, luo2023reasoning}. Agents are also capable of retrieving unstructured information. For example, WebGPT \cite{nakano2021webgpt} simulates human actions to search on internet for specific answers. Additionally, MemWalker \cite{chen2023walking} and PEARL \cite{sarthi2024raptor} organize documents into a tree structure, while ReadAgent \cite{lee2024human} condenses documents into a gist memory directory. However, these approaches often struggle with multi-hop questions. KGP \cite{wang2024knowledge} organizes documents into graphs, but it primarily uses the agent to generate queries, thereby not fully exploiting the agent's capabilities for planning and reflection.

==> content/cache/3_approach_cache_20240619.tex <==
\section{Approach}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{source/approach_v5.pdf}
    \caption{The illustration of our \ourmethod approach, consisting of graph construction, graph exploration, and answer reasoning.}
    \label{fig: ourmethod}
    \vspace{-4mm}
\end{figure*}

\subsection{Preliminary}

\ourmethod is built on a graph $\mathcal{G}=\left\{\mathcal{V}, \mathcal{E}\right\}$, where each node $v_i \in \mathcal{V}$ contains a key element $k_i$ and a set of summarized content, namely atomic facts $\mathcal{A}_i$. In other words, $v_i = \left\{k_i, \mathcal{A}_i\right\}$. And each edge $e_{ij} \in \mathcal{E}$ represents the relationship between nodes $v_i$ and $v_j$. This graph structure enables \ourmethod to capture global information from the input document $D$ within a limited context window, allowing it to decide whether to explore the current node in detail or jump to a neighboring node. During graph exploration, \ourmethod collects supporting facts and terminates the exploration once sufficient information has been gathered to answer the question. As illustrated in Figure~\ref{fig: ourmethod}, the entire process of \ourmethod consists of the following three phases: graph construction, graph exploration, and answer reasoning.
The prompts utilized in these three stages are detailed in Appendix~\ref{app: graphreader_prompt}, and a detailed example of our process can be found in Appendix \ref{app: case}.


\subsection{Graph Construction}

% To extract nodes from a given document $D$ within the limited context length of LLM, we first segment $D$ into independent chunks, each with a maximum length of $L$, while striving to maintain the integrity of the paragraph structure. For each chunk, we prompt the LLM to summarize it into a series of atomic facts, which are the smallest indivisible facts that simplify the original text. Meanwhile, we prompt the LLM to extract key elements from each atomic fact, such as essential nouns, verbs, and adjectives critical to the text's narrative.
% After processing all chunks, we normalize the key elements following~\citet{lu2023instag} to address lexical noise and uncontrolled granularity issues, resulting in the final key elements set. Subsequently, we construct each node $v_i = \left\{k_i, \mathcal{A}_i\right\}$ based on the mapping between key elements and atomic facts, where $k_i$ is a key element, and $A_i$ is all atomic facts corresponding to $k_i$. Finally, we link two nodes $v_i$ and $v_j$ if key element $k_i$ occurs in the atomic facts set $A_j$ and vice versa.

To extract nodes from a document \( D \) within the LLM's context limit, we first split \( D \) into chunks of maximum length \( L \) while preserving paragraph structure. For each chunk, we prompt the LLM to summarize it into atomic facts, the smallest indivisible facts that simplify the original text. We also prompt the LLM to extract key elements from each atomic fact like essential nouns, verbs, and adjectives. After processing all chunks, we normalize the key elements as described by \citet{lu2023instag} to handle lexical noise and granularity issues, creating a final set of key elements. We then construct each node \( v_i = \left( k_i, \mathcal{A}_i \right) \), where \( k_i \) is a key element and \( \mathcal{A}_i \) is the set of atomic facts corresponding to \( k_i \). Finally, we link two nodes \( v_i \) and \( v_j \) if key element \( k_i \) appears in \( \mathcal{A}_j \) and vice versa.



% It is worth noting that the graph construction is not bound to any specific question-answer pairs. Consequently, this graph can be reused to respond to various questions, thereby reducing redundant input in scenarios involving multiple QA from a single document or multi-turn QA.

\subsection{Graph Exploration} % Fig 2 和这里对齐


\subsubsection{Agent Initialization}


% Given a graph $\mathcal{G}$ and a question $Q$, our goal is to design an agent capable of autonomously exploring the graph using predefined functions. And the agent should have a notebook to record collected supporting facts, which will be used to reason the final answer. In addition to actions and notebook, the agent is prepared in two further dimensions to efficiently explore the graph: rational plan and initial node.

% \paragraph{rational plan} To address the complex read-world multi-hop questions, pre-planning the solution is crucial. Therefore, the agent decomposes the original question step-by-step and identifies the key information needed as a rational plan.

% \paragraph{Initial Node} A good starting point is crucial for improving search efficiency. The agent checks the key elements of all nodes $\mathcal{V}$ and selects $N$ initial nodes based on the question and the rational plan.
Given a graph \(\mathcal{G}\) and a question \(Q\), our goal is to design an agent that can autonomously explore the graph using predefined functions. The agent begins by maintaining a notebook to record supporting facts, which are eventually used to derive the final answer. Then the agent performs two key initializations: defining the rational plan and selecting the initial node.

\paragraph{Rational Plan} To tackle complex real-world multi-hop questions, pre-planning the solution is crucial. The agent breaks down the original question step-by-step, identifies the key information needed, and forms a rational plan.

\paragraph{Initial Node} Choosing strategic starting points is essential for improving search efficiency. The agent evaluates the key elements of all nodes \(\mathcal{V}\) and selects \(N\) initial nodes based on the question and the rational plan.

\subsubsection{Exploration}

% After selecting $N$ initial nodes, we treat them as the starting points for $N$ diverse paths. An agent is then tasked to begin exploration along each node, guided by the question and the rational plan, concurrently updating the notebook with relevant information acquired during exploration.

After selecting $N$ initial nodes as starting points, an agent explores each initial node by first exploring atomic facts, then chunks of the node. Next, it explores neighboring nodes, guided by the question and rational plan. The agent continuously updates the notebook with relevant information during the exploration process.

\paragraph{Exploring Atomic Facts}
It is impractical to include all original text chunks related to a node within the context window. Therefore, the agent employs a coarse-to-fine strategy, progressing from reading atomic facts to the original text, as all atomic facts can fit within the context window. Initially, all atomic facts associated with a node are grouped by their corresponding chunks, labeled with the respective chunk IDs, and fed to the agent. This allows the agent to capture an overview of each chunk by reading all groups of atomic facts. Meanwhile, the agent utilizes the question, rational plan, and notes in its notebook to reflect on the required clues and determine which chunk is likely to contain useful information. 
Subsequently, the agent is provided with two functions: 1) \textit{read\_chunk}, if the agent identifies certain chunks as valuable for further reading, it will complete the function parameters with the chunk IDs, \ie \textit{read\_chunk(List[ID])}, and append these IDs to a chunk queue. 2) \textit{stop\_and\_read\_neighbor}, conversely, if the agent deems that none of the chunks are worth further reading, it will finish reading this node and proceed to explore neighboring nodes.

\paragraph{Exploring Chunks}
When the chunk queue is non-empty, it indicates that the agent has identified multiple text chunks of interest. We then traverse the queue, reading each chunk. This step is essential because atomic facts merely summarize key information and provide brief clues, whereas specific details are best obtained directly from the original text chunks. 
While reading the chunks, the agent will once again consider the question and the plan, thinking about what can be added to the current notebook. Any supporting facts discovered will be recorded in the notebook. Depending on the updated notebook, the agent will then select one of the following four functions: 1) \textit{search\_more}, if supporting fact is insufficient, the agent will continue exploring chunks in the queue; 2) \textit{read\_previous\_chunk} and 3)\textit{read\_subsequent\_chunk}, due to truncation issues, adjacent chunks might contain relevant and useful information, the agent may insert these IDs to the queue; 4) \textit{termination}, if sufficient information has been gathered for answering the question, the agent will finish exploration.

\paragraph{Exploring Neighbors}
Once the atomic facts and chunk queue of the current node have been fully processed, it indicates that this node has been thoroughly explored, and the agent needs to access the next node. Taking into account the question, rational plan, and the content of the notebook, the agent checks all neighboring nodes, \ie key elements, and performs one of two functions: 1) \textit{read\_neighbor\_node}, the agent selects a neighboring node that might be helpful in answering the question and re-enters the process of exploring atomic facts and chunks; 2) \textit{termination}, the agent determines that none of the neighboring nodes contain useful information, it finish the exploration.

\subsection{Answer Reasoning}  % Fig 2 和这里对齐
After $N$ agents have independently gathered information and stopped their exploration, we will compile all notes from each agent for reasoning and generating the final answer. Employing Chain-of-Thought~\cite{wei2022chain}, the LLM first analyzes each note by considering complementary information from other memories and using a majority voting strategy to resolve any inconsistencies. Ultimately, the LLM will consider all the available information to generate the final answer.





==> content/cache/4_experiments_cache_20240619.tex <==
\section{Experiments}


\subsection{Experimental Settings}

\paragraph{Evaluation Benchmarks} We conduct experiments on two types of long-context QA benchmarks, including multi-hop long-context QA, \ie HotpotQA~\citep{yang-2018-emnlp-hotpotqa}, 2WikiMultihopQA~\citep{ho-2020-coling-2wikimultihopQA}, MuSiQue~\citep{Trivedi-2022-acltrans-musique}, and a single-hop long-context QA benchmark, \ie NarrativeQA~\citep{Kocisky-2018-acltrans-narrativeqa} from LongBench~\cite{Bai2023LongBenchAB}. Additionally, we also incorporate HotpotWikiQA-mixup from LV-Eval~\citep{Yuan2024LVEvalAB}, a multi-hop benchmark that features five levels of text length: 16k, 32k, 64k, 128k, and 256k. Table~\ref{tab: datasets} presents the statistics about these benchmarks, and detailed information is provided in Appendix~\ref{app: datasets}.


\paragraph{Evaluation Metrics} We employ several automatic evaluation metrics, \ie $F_1$ score, Exact Match (EM) score, and an optimized $F_1$* score, as introduced by LV-Eval~\cite{Yuan2024LVEvalAB}. Specifically, $F_1$* first computes the recall of golden answer keywords and only calculates the $F_1$ score if it exceeds a certain threshold. Otherwise, the score defaults to zero. Despite the cost-effectiveness of automatic metrics, their accuracy may be affected by the response format. Hence, we implement LLM Raters for answer correctness evaluation using an LLM, denoted as LLM-Rating-1 (LR-1) and LLM-Rating-1 (LR-2), following ReadAgent~\citep{lee2024human}. Details on the evaluation metrics can be found in Appendix \ref{app: eval_details}.


\paragraph{Baseline Methods} We compare our approach with the following baselines: retrieval augmented generation (RAG), long-context LLM, and agent-based methods.
(1) \textbf{RAG}: We choose Okapi BM25~\citep{Robertson2009ThePR} or OpenAI API embedding model Ada-002~\footnote{https://platform.openai.com/docs/guides/embeddings/\linebreak embedding-models} to retrieve the chunks most relevant to the question and employ GPT-4-128k (\texttt{gpt-4-1106-preview}) to read retrieved chunks and answer the question.
(2) \textbf{Long-context LLM}: We select GPT-4-128k for directly reading full text when the text content fits within the input window, or for segmenting the text into chunks for sequential reading.
(3) \textbf{Agent-based Method}: We select ReadAgent~\citep{lee2024human}, which employs an agent-based system for the execution of retrieval and reading processes for long-context QA.
The detailed description of these methods is provided in Appendix~\ref{app: baseline}.

\paragraph{Implementation Details}

In our experiments, we employ GPT-4-128k for both our method and baseline approaches, setting the temperature to 0.2. 
% When deploying 
For \ourmethod, the input window size is configured to 4k tokens unless stated otherwise. We limit the maximum chunk size to 2k tokens, initiate searches from 5 initial nodes, and impose a function call limit of 10 for each search path.

\begin{table}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrc}
\bottomrule
                  \textbf{Task} & \textbf{Dataset}  & Avg \#Tokens & Max \#Tokens & \#Samples  \\ \midrule
\multirow{4}{*}{\textbf{Multi-hop QA}} & HotpotQA  & 9.4k & 15.9k & 300  \\
                     & 2WikiMultihopQA  & 8.8k & 15.9k & 300 \\
                    & MuSiQue  & 15.5k & 16.0k & 200 \\
                    & HotpotWikiQA-mixup  & 142.4k & 370.8k & 250 \\ \midrule
% \multirow{1}{*}{\textbf{Single-hop QA}} &narrativeQA & English & 29.7k & 200 
\textbf{Single-hop QA} & NarrativeQA  & 29.7k & 63.7k & 200 \\\bottomrule
\end{tabular}
}
\caption{
The statistics of benchmarks employed in our evaluation. The token number is calculated using the GPT-4 tokenizer from the TikToken\protect\footnotemark. \#Samples denote the total number of benchmarks.
}
\label{tab: datasets}
\end{table}
\footnotetext{https://github.com/openai/tiktoken}



%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{lcrrrr|rrrr|rrrr|rrrr}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \textbf{Input} & \multicolumn{4}{c}{\textbf{HotpotQA}} & \multicolumn{4}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{4}{c}{\textbf{MuSiQue}} &  \multicolumn{4}{c}{\textbf{NarrativeQA}}\\ \cline{3-18}
     & \textbf{Window} & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$\\ \midrule
     % \multicolumn{18}{l}{BM25(top-1)} \\ \midrule
    BM25 (top-1) & 4k & 57.7 & 63.0 & 33.7 & 43.8 & 36.0 & 39.0 & 25.0 & 30.4 & 33.0 & 36.5 & 19.0 & 23.9 & 29.5 & 34.5 & 4.0 & 11.3 \\
    BM25 (top-3) & 4k & 74.7 & 78.3 & 45.7 & 58.5 & 59.7 & 62.0 & 42.3 & 51.9 & 43.5 & 49.5 & 25.0 & 31.1 & 44.5 & 52.5 & 7.0 & 20.5 \\ \midrule
% \multicolumn{18}{l}{OpenAI Embedding Retrieval} \\ \midrule
    Ada-002 (top-1) & 4k & 63.0 & 70.7 & 40.0 & 53.2 & 57.0 & 59.3 & 41.0 & 49.4 & 34.5 & 37.0 & 20.0 & 26.6 & 37.5 & 46.5 & 5.0 & 15.5 \\
    Ada-002 (top-3) & 4k & 72.0 & 77.3 & 45.0 & 58.1 & 65.7 & 66.7 & 44.7 & 55.3 & 40.0 & 45.5 & 24.5 & 32.1 & 45.5 & 53.0 & 7.5 & 19.5 \\ \midrule
    GPT-4-128k & $128k$ & \underline{83.3} & \underline{88.3} & \underline{53.0} & \underline{68.4} & 77.3 & 80.0 & \underline{58.7} & \underline{70.0} & 52.0 & 59.5 & 33.5 & 42.7 & \underline{63.5} & \underline{77.0} & \underline{11.5} & \underline{29.4}  \\
    GPT-4-128k (chunk) & $4k$ & 71.3 & 74.7 & 45.7 & 59.5 & 59.3 & 62.3 & 40.7 & 50.5 & 41.0 & 43.0 & 23.0 & 32.1 & 58.0 & 69.5 & 9.50 & 25.5  \\
    GPT-4-128k (chunk w/ notes) & $4k$ & 72.3 & 76.7 & 45.7 & 59.5 & 65.7 & 68.7 & 46.3 & 56.6 & 39.5 & 43.0 & 25.0 & 32.5 & 56.5 & 65.0 & 8.5 & 24.3  \\\midrule
    ReadAgent & $128k$ & 72.3 & 78.7 & 48.0 & 62.0 & \underline{79.0} & \underline{81.0} & 52.7 & 63.7 & \underline{54.5} & \underline{61.0} & \underline{35.0} & \underline{45.1} & 63.0 & 75.5 & 5.0 & 18.9 \\ 
    \ourmethod & $4k$ &\textbf{84.3} & \textbf{89.7} & \textbf{55.0} & \textbf{70.0} & \textbf{83.7} & \textbf{87.0} & \textbf{59.3} & \textbf{70.1} & \textbf{59.0} & \textbf{63.5} & \textbf{38.0} & \textbf{47.4} & \textbf{65.0} & \textbf{80.0} & \textbf{15.5} & \textbf{29.8} \\
    \midrule
    Golden & $4k$ & 92.3 & 93.7 & 57.0 & 73.8 & 88.3 & 89.7 & 63.0 & 73.4 & 66.0 & 69.0 & 45.0 & 56.0 & - & - & - & - \\  \midrule
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) comparison of different baselines on datasets from LongBench. The best performance and the second-best performance are denoted in bold and underlined fonts, respectively. ``Golden'' denotes the settings in which we add question and its supporting facts to LLM directly.}
% \vspace{-0.5cm}
\label{tab: main_result_1}
\end{table*}
%---------------------------------------------------------
 % \multirow{4}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}}} \\
 % & & & & & & & & & & & & & & & & \\
 % & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lcrrr|rrr|rrr|rrr|rrr}
\midrule
 \multirow{3}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}} \\\cline{3-17}
 & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
& & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$*\\ \midrule
% \multicolumn{17}{l}{BM25 Retrieval} \\ \midrule
    BM25 (top-1) & $4k$ & 10.0 & 16.0 & 12.0 & 16.0 & 18.0 & 11.9 & 6.0 & 8.0 & 8.5 & 10.0 & 8.0 & 7.0 & 14.0 & 20.0 & 5.9 \\
    BM25 (top-3) & $4k$ & 16.0 & 22.0 & 13.9 & 18.0 & 28.0 & 13.3 & 16.0 & 18.0 & 11.8 & 12.0 & 16.0 & 11.8 & 12.0 & 22.0 & 9.3 \\ \midrule
% \multicolumn{17}{l}{OpenAI Embedding Retrieval} \\ \midrule
    Ada-002 (top-1) & $4k$ & 10.0 & 12.0 & 14.5 & 14.0 & 18.0 & 11.3 & 10.0 & 12.0 & 12.5 & 12.0 & 14.0 & 9.4 & 8.0 & 8.0 & 7.0 \\
    Ada-002 (top-3) & $4k$ & 24.0 & 28.0 & 21.3 & 20.0 & 30.0 & 19.8 & 14.0 & 20.0 & 12.9 & 16.0 & 20.0 & 12.0 & 14.0 & 18.0 & 10.8 \\  \midrule
    GPT-4-128k & $128k$ & {\underline {38.0}} & {\underline {38.0}} & {\underline {35.7}} & {\underline {26.0}} & {\underline {30.0}} & {\underline {26.0}} & 22.0 & 24.0 & 20.6 & 16.0 & 16.0 & 14.6 & 14.0 & 16.0 & 10.3 \\
    GPT-4-128k (chunk) & $4k$ & 18.0 & 22.0 & 24.6 & 16.0 & 20.0 & 17.7 & 20.0 & 24.0 & 17.0 & 20.0 & 24.0 & 14.7 & {\underline {28.0}} & {\underline {30.0}} & 10.7 \\
    GPT-4-128k (chunk w/ notes) & $4k$ & 22.0 & 32.0 & 24.2 & 26.0 & 30.0 & 21.3 & {\underline {28.0}} & {\underline {32.0}} & {\underline {22.0}} & {\underline {24.0}} & {\underline {26.0}} & {\underline {17.4}} & 26.0 & 26.0 & {\underline {14.8}} \\ \midrule
    ReadAgent & $128k$ & 24.0 & 26.0 & 29.2 & 20.0 & 22.0 & 16.9 & 24.0 & 30.0 & 15.3 & 14.0 & 18.0 & 13.6 & 20.0 & 22.0 & 10.4 \\
    \ourmethod & $4k$ & \textbf{42.0} & \textbf{42.0} & \textbf{38.2} & \textbf{32.0} & \textbf{38.0} & \textbf{36.4} & \textbf{30.0} & \textbf{36.0} & \textbf{32.9} & \textbf{28.0} & \textbf{34.0} & \textbf{30.6} & \textbf{30.0} & \textbf{38.0} & \textbf{33.0} \\
\midrule
\end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) of different baselines on datasets from LV-Eval, where $F_1$* donates LV-Eval's optimized $F_1$. The best performance and the second-best performance are denoted in bold and underlined fonts, respectively. We truncate to keep the longest possible initial fragment while preserving paragraph structure, in contexts that exceed the input window (128k and 256k) for GPT-4-128k.}
% \vspace{-0.5cm}
\label{tab: main_result_2}
\end{table*}
%---------------------------------------------------------
\subsection{Main Results}

\ignore{\paragraph{Evaluation on Single and Multi-hop Long-context Tasks}} The results of three types of methods on four multi-hop long-context benchmarks and one single-hop long-context benchmark are shown in Table~\ref{tab: main_result_1} and Table~\ref{tab: main_result_2}. Based on the results, we have the following findings:

\paragraph{Results of RAG methods}
As the results shown in Table~\ref{tab: main_result_1}, RAG methods based on BM25 and Ada-002 exhibit the worst performance in comparison to long-context LLM and agent-based methods. A possible reason is that text retrieval has difficulty recalling all chunks that contain the supporting facts for answering the input question. Although increasing the number of recalled chunks could improve the performance of text retrieval, the context window will limit the effectiveness of these RAG methods. 

\paragraph{Results of Long-Context LLMs}

From the results shown in Table~\ref{tab: main_result_1}, we can see that employing GPT-4-128k to directly answer the question with long contexts significantly outperforms RAG methods and even outperforms ReadAgent on three long-context benchmarks. This is because of the superior performance of GPT-4-128k in processing long texts and executing multi-hop reasoning tasks. Additionally, the lengths of these four benchmarks are significantly shorter than the 128k context window, thereby mitigating the impact of ``lost in the middle'' on the model's performance. 

\ignore{Moreover, we also observe that GPT-4, despite having a constrained 4k context window, can process input contexts that significantly exceed its context window limitations through sequential reading. By incorporating a memory module, sequential reading with LLM can significantly boost the performance on multi-hop benchmarks. The reason may be that carrying memory with historical information can facilitate LLM in aggregating previous supporting facts. Conversely, for the single-hop benchmark, NarrativeQA, integrating memory results in performance degradation. The reason may be that previous memory introduces noise to LLM and affects its responses. }

\paragraph{Results of Agent-based Methods}


By comparing our approach with all baselines in Table~\ref{tab: main_result_1}, it is obvious that our approach consistently performs better than them on four long-context benchmarks and demonstrates superior performance in multi-hop long-context tasks. In our approach, benefiting from the graph's ability to capture the relationships between detailed information, our method can identify crucial information and search for the supporting facts for the input question efficiently. This strategy significantly boosts the agent's capability in multi-hop reasoning and capturing long-range dependencies of key information in a long context. Moreover, the results in Table~\ref{tab: main_result_1} show that ReadAgent, with a 128k context window setup, underperforms \ourmethod with a 4k context window and even performs worse than GPT-4-128k full-text reading. 
%%% START COMMENTS %%%
%（FROM HANGYU, BEFORE 20240618）We attribute this to ReadAgent's strategy of using page summaries, past memory, and input questions to select pages for acquiring supporting information. Compared to our \ourmethod, the strategy of ReadAgent may restrict the agent's ability to identify specific details and capture long-range dependencies in a long context, consequently affecting its overall performance.
% (FROM XINGYUAN):
We attribute this to ReadAgent's strategy of excessively compressing the original texts into gist memories, and feeding all mixed memories to the model for page number selection. Compared to our \ourmethod, the strategy of ReadAgent may restrict the agent's ability to identify specific details and capture intrinsic connections among key elements in a long context, consequently affecting its overall performance.
%%% END COMMENTS %%%
 This further indicates that our approach can more efficiently unlock the capabilities of constrained context window LLMs in processing long context. Additionally, we observe that the performance of our method closely matches that achieved by directly supplying supporting facts to the LLM (\ie Golden in Table~\ref{tab: main_result_1}). This is because our method incorporates not only pre-planning, reflection, and various actions but also the usage of a graph containing key information, facilitating the agent to search for the correct supporting facts.






\paragraph{Evaluation on Extremely Long Context Tasks} As shown in previous experiments, it demonstrates the effectiveness of employing a limited context window LLM for long-context tasks with our \ourmethod. Here, we would like to study the impact of extremely long context on our \ourmethod. As shown in Table~\ref{tab: main_result_2}, compared with all baselines, our \ourmethod not only consistently outperforms these methods across text lengths ranging from 16k to 256k tokens but also exhibits robustness with the expansion of context length. It indicates that our method is still effective in handling extremely long texts by graph exploration with limited context window LLMs. With the increase in the length of the input context, the performance of GPT-4-128k full-text reading degrades gradually. As a comparison, our method achieves a performance gain of 10.53\% relatively on LR-1 over GPT-4-128k full-text reading under 16k context length. With the context length increasing to 128k, our method achieves a performance gain of 75.00\% relatively over GPT-4-128k. This can be attributed to the fact that as the context length increases, the impact of the ``lost in the middle'' effect on GPT-4-128k becomes progressively more severe. Secondly, we observe that ReadAgent significantly underperforms our method in handling extremely long contexts. This is because the lack of detailed information about the content of each page can make page selection very difficult for ReadAgent, especially when dealing with extremely long contexts. This further demonstrates that our method can effectively address the challenges of processing extremely long context with limited context window LLMs by exploring graphs containing fine-grained information.



\begin{table}[!t]
\centering
% \scriptsize
\resizebox{\columnwidth}{!}{
    \begin{tabular}{clccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Results(\%)}}\\ \cline{3-5} 
     & & LR-1 & LR-2 & $F_1$ \\ \midrule
    \multirow{3}{*}{\textbf{HotpotQA}} & \ourmethod & \textbf{84.3} & \textbf{89.7} & \textbf{70.0} \\
        & \quad w/o Rational Plan & 81.7 & 87.7 & 63.8 \\
        & \quad w/o Node Selection & 66.0 & 71.7 & 54.1 \\\midrule
    \multirow{3}{*}{\textbf{2WikiMultihopQA}}& \ourmethod & \textbf{83.7} & \textbf{87.0} & \textbf{70.1} \\
        & \quad w/o Rational Plan & 81.3 & 86.0 & 65.4 \\
        & \quad w/o Node Selection & 65.3 & 68.7 & 49.7 \\\midrule
    \multirow{3}{*}{\textbf{MuSiQue}} & \ourmethod & \textbf{59.0} & \textbf{63.5} & \textbf{47.4} \\
    & \quad w/o Rational Plan & 56.0 & 61.0 & 42.4 \\
    & \quad w/o Node Selection & 35.0 & 38.5 & 25.2 \\\midrule
    \multirow{3}{*}{\textbf{NarrativeQA}} & \ourmethod & \textbf{65.0} & \textbf{80.0} & \textbf{29.8}  \\
        & \quad w/o Rational Plan & 63.0 & 78.5 & 26.6 \\
        & \quad w/o Node Selection & 53.0 & 65.5 & 24.0 \\
    \bottomrule
    \end{tabular}
}
\vspace{-0.2cm}
\caption{The results of our ablation study. ``w/o Rational Plan'' refers to removing the rational plan in the agent initialization stage, and ``w/o Node Selection'' denotes applying the random selection of initial nodes and neighbor nodes in graph exploration.}
% \vspace{-0.5cm}
\label{tab: ablation}
\end{table}
%---------------------------------------------------------
\subsection{Ablation study}
% We conduct ablation experiments on various benchmarks to investigate the contribution of different components in our approach. 

\paragraph{The Effect of Rational Plan}


% In our graph exploration stage, we introduce the rational plan to assist agent analysis input complex questions step by step and then guide the agent to explore the graph. To verify the effectiveness of the rational plan, we remove it in agent initialization and conduct experiments on four long-context QA benchmarks. As shown in Tabel~\ref{tab: ablation}, we can see that our approach is better than variants without the rational plan (denoted as ``w/o Rational Plan'' in Tabel~\ref{tab: ablation}). It indicates that the rational plan is effective in guiding the agent to node selection and exploration on the graph.
In the graph exploration stage, we introduce a rational plan to help the agent analyze complex input questions step by step, guiding the agent in exploring the graph. To verify the effectiveness of the rational plan, we removed it during agent initialization and conducted experiments on four long-context QA benchmarks. Table~\ref{tab: ablation} shows that the rational plan is effective in guiding the agent in node selection and exploration on the graph.

% \ignore{
% To evaluate the Rational Plan's effectiveness, we remove the pre-planning stage in our method and conduct experiments on four long-context benchmarks. The results are shown in Table~\ref{tab: ablation}. We can observe that removing the rational path in \ourmethod leads to performance degradation. It indicates that the improvement of our methods is due to


% thus confirming the rational plan's beneficial impact on \ourmethod. We can infer that the pre-planning stage enables \ourmethod to deal with various complex questions effectively.
% }


\paragraph{The Effect of Node Selection}
% On the other hand, to demonstrate the effectiveness of our model in selecting which nodes to visit based on reasoning about the required information, we conduct experiments under settings of randomly selecting initial nodes and neighbor nodes. As shown in Table \ref{tab: ablation}, random selection~(denoted as ``w/o Node Selection'' in Tabel~\ref{tab: ablation}) results in the significant performance degradation of our approach, with results across all datasets declining by an average of 18\%. It demonstrates that \ourmethod is thinking carefully when selecting neighbor nodes, and the selected actions are reasonable.
We conduct randomly selecting initial nodes and neighbor nodes experiments to demonstrate the necessity of our system in selecting which nodes to visit based on reasoning about the required information. As shown in Table \ref{tab: ablation}, random selection results in a significant performance drop, with an average decline of 18\%. This demonstrates that \ourmethod carefully considers node selection, leading to more reasonable and effective exploration.

\paragraph{Impact of the Number of Initial Nodes}
% To assess the effect of the number of initial nodes on \ourmethod's performance, we conduct experiments setting different numbers of initial nodes on both multi-hop and single-hop QA datasets, and the results are shown in Figure \ref{fig: nodes}. Firstly, it can be observed that the performance of \ourmethod changes slightly with the number of initial nodes, showing strong robustness. Secondly, within a certain range, an increase in the number of nodes leads to a slight improvement in model performance and the performance is relatively optimal when the initial number of nodes is set to 5, hence we choose this as our default initial node setting. However, surpassing a certain threshold, \ourmethod's performance tends to decline. Notably, this decrement is more apparent in single-hop scenarios. We consider this decline likely due to the increased noise introduced by an excessive number of initial nodes.
We conduct experiments with different initial node counts on multi-hop and single-hop QA datasets to assess the effect of the number of initial nodes on \ourmethod's performance. The results are shown in Figure \ref{fig: nodes}. Increasing the number of nodes improves performance up to a certain point, with optimal performance at 5 initial nodes, which we set as the default. However, beyond this threshold, performance declines, especially in single-hop scenarios, likely due to increased noise from too many initial nodes.

\paragraph{Impact of the Chunk Size}
We investigate the impact of chunk size $L$ on \ourmethod's performance. As shown in Figure \ref{fig: chunk_size_exp}, the best performance is achieved with $L=2k$. When $L$ exceeds a certain threshold, performance declines because larger chunks cause the model to overlook essential details. Conversely, smaller chunks lead to more semantic truncation, hindering comprehension and accuracy in extracting atomic facts. Thus, we chose $L=2k$ as the default chunk size.
% To explore the impact of the chunk size $L$ on the performance of \ourmethod, we conduct experiments with different chunk sizes. As shown in Figure \ref{fig: chunk_size_exp}, the results show that the best performance was achieved when setting $L=2k$. We can see that when $L$ exceeds a certain threshold, the bigger the chunk size, the more obvious the performance decline trend. This corresponds to the model performance degradation on longer texts mentioned earlier, where the model tends to overlook essential details. 
% Moreover, more semantic truncation occurs when $L$ is too small, hampering the model's comprehension of the current context and further affecting the accuracy of extracting atomic facts. Therefore, we finally choose $L=2k$ as our default chunk size setting.

%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/figure3.pdf}
% \vspace{-0.6cm}
\caption{Performance of \ourmethod with different initial node numbers on 2WikiMultihopQA and NarrativeQA. Results show the robustness of \ourmethod towards different initial node numbers.}
\label{fig: nodes}
% \vspace{-0.6cm}
\end{figure}
%---------------------------------------------------------
%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1.0\linewidth]{source/figure4.pdf}
% \vspace{-0.2cm}
\caption{The impact of chunk size $L$ of \ourmethod on the 256k length level of HotpotWikiQA-mixup.}
\label{fig: chunk_size_exp}
% \vspace{-0.2cm}
\end{figure}
%---------------------------------------------------------
% \vspace{-0.2cm}
\subsection{Further Analysis}
% \vspace{-0.1cm}
%For multi-hop QA, having a sufficient number of starting nodes is crucial. For example, in questions involving comparisons, the objects to be compared are often difficult to associate on the memory graph. In such cases, selecting a starting node for each object becomes particularly important for searching for enough information to answmemories of different paths, which confusesnvestigate the impact of the number of initial nodes on the outcomes, we conducted experiments using datasets from both multi-hop QA and single-hop QA. The experimental results shown in Table \ref{tab: starting_nodes}  reveal that when the number of initial nodes is too low, the performance of \ourmethod improves with an increase in the number of initial nodes. However, the final QA performance slightly declines when the number of initial nodes is excessive. We believe this is due to the overabundance of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of initial nodes is more pronounced for single-hop QA.

% Table \ref{tab: starting_nodes} showcases the impact of different numbers of starting nodes, which are the number of search paths, on the final outcome. We selected one dataset each from multi-hop QA and single-hop QA datasets for experimentation to explore their respective effects on multi-hop QA and single-hop QA. The experimental results reveal that when the number of starting nodes is too low, the performance of \ourmethod improves with an increase in the number of starting nodes. However, the final QA performance slightly declines when the number of starting nodes is excessive. We believe this is due to the overabundance and disorganization of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of starting nodes is more pronounced for single-hop QA.
%---------------------------------------------------------
% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \midrule
    
%     \textbf{Dataset} & \textbf{Avg Action Num(per trace)} & \textbf{Stage} & \textbf{Total Ratio} & \textbf{Selected Action} & \textbf{Selection Ratio}\\ \midrule
%      % \multirow{7}{*}{\textbf{MuSiQue}} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{3}{*}{read_chunk} & \multirow{3}{*}{0.312(2185/7002)}
%      \multirow{7}{*}{MuSiQue} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.312(2185/7002)} & \textit{search\_more}s & 0.191(417/2185)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.266(582/2185) \\ 
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.257(561/2185) \\
%     &  &  &  & \textit{stop} & 0.286(625/2185) \\  \cline{3-6}
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.400(2800/7002)} & \textit{read\_chunk} & 0.413(1156/2800) \\ 
%     &  &  &  & \textit{stop} & 0.587(1644/2800) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.288(2017/7002)} & \textit{read\_neighbor\_node} & 0.401(809/2017)  \\ 
%     &  &  &  & stop & 0.599(1208/2017) \\ \midrule
% \multirow{7}{*}{NarrativeQA} & \multirow{7}{*}{3.8475(7695/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.543(4176/7695)} & \textit{search\_more} & 0.041(171/4176)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.353(1475/4176) \\
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.326(1360/4176) \\
%     &  &  &  & \textit{stop} & 0.280(1170/4176) \\ 
%     \cline{3-6} 
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.325(2502/7695)} & \textit{read\_chunk} & 0.645(1615/2502) \\  
%     &  &  &  & \textit{stop} & 0.355(887/2502) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.132(1017/7695)} & \textit{read\_neighbor\_node} & 0.514(523/1017)  \\
%     &  &  &  & \textit{stop} & 0.486(494/1017)  \\
%     \midrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Action statistics of \ourmethod on two datasets.}
% % \vspace{-0.5cm}
% \label{tab: action}
% \end{table*}

% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Avg Ctx. Tokens}} & \multirow{2}{*}{\textbf{Chunk Limit}} & \multirow{2}{*}{\textbf{Token Type}} & \multicolumn{2}{c}{\textbf{Stage}} \\ \cline{5-6} 
%        & & &  & avg atomic facts and key elements tokens & avg agent tokens \\\midrule
%     \multirow{8}{*}{\textbf{HotpotWikiQA-mixup-256k}} & \multirow{8}{*}{366950.70} & \multirow{2}{*}{1k} & input token & 585770.34 & 90624.49   \\
%         & & & output token & 270179.60 &  13558.30 \\\cline{4-6}
        
%     & & \multirow{2}{*}{2k} & input token & 465931.14 & 69821.40 \\
%         & & & output token & 156201.42 & 11057.36  \\\cline{4-6}

%         & & \multirow{2}{*}{4k} & input token & 417449.46 & 93083.31   \\
%         & & & output token & 142652.42 & 10939.20  \\\cline{4-6}

%         & & \multirow{2}{*}{6k} & input token & 400457.94 & 76402.95  \\
%         & & & output token & 131023.17 & 9625.54 \\
       
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Consumption statistics of \ourmethod on two datasets. The input window is set to 4k, with 7 starting nodes, and a maximum of 10 actions. The upper limit of text fragments is 2k.}
% % \vspace{-0.5cm}
% \label{tab: cost}
% \end{table*}
%--------------------------------------------------------------


%---------------------------------------------------------
\begin{table}[!t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc}
\toprule
    Method & Avg. Ctx. \#Tokens & Avg. Cost \#Tokens  \\\midrule
    ReadAgent & 358.3k & 48.7k  \\
    \ourmethod & 358.3k & 52.8k \\\bottomrule
    \end{tabular}
}
\caption{Comparison of token consumption per question between ReadAgent and \ourmethod on HotpotWikiQA-mixup-256k, where ``Avg. Ctx. \#Tokens'' refers to the average token number of the original dataset. The ``Avg. Cost \#Tokens'' comprise both input tokens and output tokens during exploration.}
\label{tab: consumption}
\end{table}
%--------------------------------------------------------------------------


%When $L$ is smaller, it is evident that more resources are consumed during the construction phase of the memory graph. Thus, to balance performance and consumption, a larger and more effective $L$ should be selected as the hyperparameter setting as much as possible.

% To balance consumption and performance, we think $L=2k$ is a good setting.
% To investigate the impact of input window size on \ourmethod, we conducted experiments on HotpotWikiQA-mixup-256k. We used different input window sizes, and the results in Figure \ref{fig: chunk} indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects one action: during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.

% Table \ref{tab: input_window} demonstrates the impact of the input window size on \ourmethod. To facilitate the testing of larger input windows, we conducted experiments on HotpotWikiQA-mixup-256k. The experimental results indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects three actions: less pagination when searching for starting nodes, reading more nodes at once; during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.
%---------------------------------------------------------
% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Input Window}} & \multicolumn{2}{c}{\textbf{Metrics}}\\ \cline{3-4} 
%        &  & LR-1 & LR-2 \\ \midrule
    
%     \multirow{4}{*}{\textbf{HotpotWikiQA-mixup-256k}} & 4k & 30.0 & 38.0 \\
%         & 8k & \textbf{32.0} & \textbf{40.0} \\
%         & 16k & 32.0 & 38.0 \\
%         & 32k & 28.0 & 36.0 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{The impact of the input window size.}
% % \vspace{-0.5cm}
% \label{tab: input_window}
% \end{table}

\paragraph{Cost Analysis}
% 不能让人觉得我们是依靠更多的资源消耗取得的更好的效果
% 
To evaluate the inference cost of our approach, we compare the average token consumption of ReadAgent and \ourmethod for each question. As shown in Table \ref{tab: consumption}, \ourmethod uses only 1.08 times more tokens than ReadAgent but achieves over twice the performance improvement, demonstrating its superiority. Additionally, after the first round of document preprocessing, token consumption in subsequent exploration is significantly reduced and much lower than the original dataset's token count.
% To evaluate the inference cost of our approach, we compare the average token consumption of ReadAgent and \ourmethod when dealing with each question. As shown in Table \ref{tab: consumption}, we can see that the token usage of \ourmethod is only 1.08 times greater than that of ReadAgent, yet it achieves more than 2 times performance improvement, favorably demonstrating the superiority of our method.
% %说明下前提，可以看到在第一轮预处理好文章后后面轮次的消耗都显著减少，并且远少于原始的token数量，但是这里没有数字
% Additionally, it is notable that after the documents are preprocessed in the first round, the consumption in subsequent rounds is significantly reduced and is far less than the token numbers of the origin dataset. 
%This highlights \ourmethod's considerable applicability in multi-round QA scenarios.
%--------------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/recall.pdf}
% \vspace{-0.6cm}
\caption{Recall of supporting facts by different methods on HotpotWikiQA-mixup.}
\label{fig: recall}
% \vspace{-0.6cm}
\end{figure}

\paragraph{Recall Rate Analysis}
% 关键信息召回,这个跟前面的区别
%单看我们的模型始终维持在一个水准，有较强的
To evaluate our method's advantages in key information recall, we utilize GPT-4 to assess the recall of supporting facts on the HotpotWikiQA-mixup dataset. As shown in Figure~\ref{fig: recall}, our model consistently outperforms other baseline methods, regardless of the input length. As context length increases from 16k to 256k, recall of supporting facts declines across all methods. However, \ourmethod maintains around 60\% recall at 256k context length, in contrast to the significant degradation in ReadAgent. This demonstrates \ourmethod's scalability and effectiveness in processing long contexts.
Further details and evaluation prompts can be found in Appendix~\ref{app: recall}. 
% First, we can see that no matter how long the input length is, the performance of our model consistently and significantly outperforms other baseline methods.
% Second, it can be observed that as the context length increases (from $16k$ to $256k$), the recall of supporting facts degrades across all methods. But \ourmethod relatively maintains strong performance, stabilizing at around 60\% at an input length of 256k finally, which is in sharp contrast to the downward trend of ReadAgent. It demonstrates the scalability of \ourmethod that can maintain high performance on very long texts.

%Besides, we notice that as the context length increases (from $16k$ to $256k$), the recall of supporting facts for all methods declines, with ReadAgent experiencing a particularly rapid decrease, while \ourmethod shows a very slow decline. This indicates that \ourmethod has excellent scalability in handling long texts.
\ignore{
To further illustrate the recall capabilities of \ourmethod across varying levels of detail, we assessed the ``Supporting Facts'' and ``Sample'' recall rates utilizing the same method. As depicted in Table \ref{tab: recall}, the ``Supporting Facts" granularity captures the recall rate of all supporting facts throughout the dataset. In contrast, the "Sample" granularity considers the entirety of a sample's supporting facts as the minimal evaluation unit, with recall considered successful only if every atomic fact is identified.

The recall rate associated with the complete notebook marginally exceeds that of the atomic facts. This suggests that \ourmethod excels at deriving more relevant information from segments during exploration, indirectly evidencing its intellectual acumen and efficacy in information retrieval


}

\ignore{For sample granularity, a sample is considered to be recalled only if all of its supporting facts are recalled.}
% As shown in Table \ref{tab: recall},
To further demonstrate the recall rate of \ourmethod at different granularities, we calculate the recall rate of \emph{Supporting Facts} and \emph{Sample} granularity respectively using the same method, detailed in the Appendix~\ref{app: recall}. The granularity of supporting facts refers to the recall rate of all supporting facts across the entire dataset. As for sample granularity, a sample is considered to be recalled only if all of its supporting facts are recalled.
% As for the sample granularity, a sample's total supporting facts are considered the smallest evaluation unit, and recall is deemed successful only when all its atomic facts are retrieved. 
% Our method exhibits slightly higher recall for the final notebook than for atomic facts recall. 
As shown in the Tabel~\ref{tab: recall}, the recall for the final notebook is slightly higher than the recall of atomic facts, which indicates that our method is capable of extracting more valid information from chunks during the exploration, indirectly reflecting its intelligence and effectiveness in exploration.

%--------------------------------------------------------------
\begin{table}[!t]
\centering
% \scriptsize
\resizebox{0.75\columnwidth}{!}{
    \begin{tabular}{ccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Source}}  & \multicolumn{2}{c}{\textbf{Recall(\%)}} \\ \cline{2-3} 
     &  SF-wise & Sample-wise \\ \midrule
    Atomic Facts & 76.4 & 64.7 \\
    Final Notebook & 90.5 & 85.3  \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
% \caption{\ourmethod's recall of supporting facts at various stages. Define a partial\_ratio similarity greater than $0.8$ as a successful recall. We use \textit{gpt-4-1106-preview} for evaluation, with the temperature set to 0.1.}
\caption{\ourmethod's recall performance at different granularities on HotpotQA. ``SF-wise'' refers to the granularity of supporting facts, and ``Sample-wise'' refers to the granularity of sample evaluation.}
\label{tab: recall}
\end{table}
%--------------------------------------------------------------
% To better assess the advantages of our method in identifying key information, we utilized the supporting facts that support answering questions from the HotpotQA dataset. We analyzed \ourmethod's recall of supporting facts at various stages on the HotpotQA dataset.

%Table \ref{tab: recall} presents the experimental results of the recall analysis for \ourmethod, where the two stages of evaluation are specifically: atomic facts extracted from the text and the final memory obtained. The evaluation was conducted using LLM (\textit{gpt-4-1106-preview}, with the specific evaluation prompt shown in Figure \ref{recall_prompt}). The statistics were compiled based on supporting facts (by supporting fact) and by individual cases (by case), where "by supporting fact" refers to whether that supporting fact was recalled, and "by case" indicates whether all supporting facts for a given case were fully recalled.

% The results indicate that under the same LLM evaluation method (with identical prompts), the final memory's recall rate for supporting facts is higher compared to the recall rate for atomic facts. Furthermore, the gap between this recall rate aligns with the assessment results of the LLM-Raters (Figure \ref{tab: main_result_2}, LR-1: 0.843; LR-2: 0.897). This demonstrates \ourmethod's capability to locate corresponding supporting facts from weakly related nodes.
%--------------------------------------------------------------




==> content/cache/approach_cache.tex <==
\section{Approach}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{source/approach_v1.pdf}
    \caption{MT-Bench-101 encompasses three overarching abilities and thirteen distinct tasks within multi-turn dialogue scenarios, facilitating a granular benchmarking from basic perceptivity to advanced interactivity. On the right, a model with a broader range of abilities is considered better in multi-turn scenarios.}
    \label{fig: ourmethod}
    \vspace{-4mm}
\end{figure*}

\subsection{Preliminary}
% Inspired by human reading behaviors, we design a method called \ourmethod based on LLM agent, as illustrated in Figure~\ref{}. The method consists of two stages:   
% %---------------这里直接定义原子事实会让人confusing?
% \textbf{(a) Memory Graph Construction.} We first split a text document $\mathcal{D}$ into a set of pages $\left\{\mathcal{P}_i\right\}$, each $\mathcal{P}_i$ denoting the $i$-th page of $\mathcal{D}$. Subsequently we transform $\left\{\mathcal{P}_i\right\}$ into a set of atomic facts $\mathcal{A}=\left\{a_i\right\}_{i=0}^M$ and key elements $\mathcal{V}=\left\{v_i\right\}_{i=0}^N$, then we construct the Memory Graph $\mathcal{G}=\left\{\mathcal{V}, \mathcal{E}\right\}$, where the edge set $\mathcal{E}=\left\{e_{ij}\right\}$ is determined based on the co-occurrence of $v_i$ and $v_j$ within $a_k$.

% \textbf{(b) Agent Graph Reasoning.} We leverage a LLM $f_{LLM}$ as an agent. When presented with a question $q$, the agent identifies key entities and plans multiple distinct reasoning paths to ensure the diversity of evidence. The agent gathers evidence iteratively by visiting nodes reading the corresponding claims and original texts, and planning subsequent nodes based on the current evidence. When the agent determines that the accumulated evidence is sufficient, it generates a response to the question.

% These two stages enable the LLM to process very long context and address complex, multi-hop questions. The following sections will provide a detailed description of the implementation.

\ourmethod is built on a memory graph $\mathcal{G}=\left\{\mathcal{V}, \mathcal{E}\right\}$, where each node $v_i \in \mathcal{V}$ contains a key element $k_i$ and a set of summarized memories, namely atomic facts $\mathcal{A}_i$. In other words, $v_i = \left\{k_i, \mathcal{A}_i\right\}$. And each edge $e_{ij} \in \mathcal{E}$ represents the relationship between nodes $v_i$ and $v_j$. This graph structure enables \ourmethod to read global information of the input document $D$ within a limited context window, allowing it to decide whether to explore the current node in detail or jump to a neighboring node. During graph exploration, \ourmethod collects supporting facts and terminates the exploration once sufficient information has been gathered to answer the question. As illustrated in Figure~\ref{fig: ourmethod}, the entire process of \ourmethod consists of the following three phases: graph construction, graph exploration, and answer reasoning.
% \ourmethod is built on an information graph $\mathcal{G}=\left\{\mathcal{N}, \mathcal{E}\right\}$, where each node $n_i \in \mathcal{N}$ is represented by a key element $k_i$ and contains a set of atomic facts $\mathcal{A}_i$. And each edge $e_{ij} \in \mathcal{E}$ represents the relationship between nodes $v_i$ and $v_j$. This structure enables \ourmethod to read global information of the input document $D$ within a limited context window, allowing it to decide whether to explore the current node in detail or jump to a neighboring node. During graph exploration, \ourmethod collects supporting facts and terminates the exploration once sufficient information has been gathered to answer the question. As illustrated in Figure~\ref{fig: ourmethod}, the entire process of \ourmethod consists of the following three phases: graph construction, graph exploration, and answer reasoning.


\subsection{Graph Construction}

% In our approach, to represent global information of $D$, we introduce a reusable data structure, the memory graph $\mathcal{G}$. The construction of $\mathcal{G}$ involves a two-stage process. Firstly, we utilize a prompt-based method to extract atomic facts $\mathcal{A}$ and $\mathcal{V}$ from $\mathcal{D}$ utilizing a LLM, where $\mathcal{A} = {\mathcal{A}_i}_{i=1}^N$. Subsequently, we connect these $\mathcal{V}$ based on the co-occurrence within $\mathcal{A}$ to construct the $\mathcal{G}$ for $\mathcal{D}$.


% \paragraph{Atomic Facts and Key Elements Extraction}
% \paragraph{Node Extraction}

% In our approach, key elements denote the essential nouns, verbs, and adjectives critical to the text's narrative, while atomic facts are the smallest, indivisible facts. To extract key elements $\mathcal{V}$ and atomic facts $\mathcal{A}$ accurately and efficiently, we prompt LLM to extract atomic facts $\mathcal{A}^{i}$ and its associated key elements $\mathcal{V}^{i}$ for each page $\mathcal{P}_i$, denoted as:
% \begin{equation}
%     \mathcal{A}^{i}, \mathcal{V}^{i} = f_{LLM}(P^C, \mathcal{P}_i)
% \end{equation}
% Here, $\mathcal{A}^{i}$ and $\mathcal{V}^{i}$ denote the atomic facts and key elements of $\mathcal{P}_i$ respectively, where $\mathcal{A} = \bigcup_{i} \mathcal{A}^{i}$ and $\mathcal{V} = \bigcup_{i} \mathcal{V}^{i}$. $P^C$ serves as the LLM-guiding prompt. To save the cost of calling LLM APIs, we carefully design $P^C$ to guide LLM for extracting $\mathcal{A}$, $\mathcal{E}$ at one time. In addition to integrating specific requirements and definitions of atomic facts and key elements within $P^C$, we also add a short prompt that ensures the key elements are contained within atomic facts. This strategy is designed to force the extraction of atomic facts that accurately represent $\mathcal{D}$’s information while also decreasing redundancy and the cost of utilizing GPT-4.

% In our approach, key elements denote the essential nouns, verbs, and adjectives critical to the text's narrative, while atomic facts are the smallest, indivisible facts. To extract key elements $\mathcal{V}$ and atomic facts $\mathcal{A}$ accurately and efficiently, we prompt LLM to extract atomic facts $\mathcal{A}^{i}$ and its associated key elements $\mathcal{V}^{i}$ for each page $\mathcal{P}_i$. To save the cost of calling LLM APIs, we carefully design the prompt $P^C$ to guide LLM for extracting $\mathcal{A}$, $\mathcal{E}$ at one time. In addition to integrating specific requirements and definitions of atomic facts and key elements within $P^C$, we also add a short prompt that ensures the key elements are contained within atomic facts. This strategy is designed to force the extraction of atomic facts that accurately represent $\mathcal{D}$’s information while also decreasing redundancy and the cost of utilizing GPT-4.


% \paragraph{Edge Linking}
% Through the extraction process described above, we obtain atomic facts $\mathcal{A}$ and key elements $\mathcal{V}$ from the long text document $\mathcal{D}$. 
% To simplify the complexity of graph $\mathcal{G}$ and enhance the agent's reading efficiency, we employ the integrable key elements in $\mathcal{A}$ as nodes within the $\mathcal{G}$. But,  during the implementation of $f_{LLM}$ for information extraction, $\mathcal{A}$ and $\mathcal{V}$ are extracted in one time, inevitably introduces noise into $\mathcal{V}$. Hence, we apply entity-level normalization on extracted key elements $\mathcal{V}$ and construct the $\mathcal{G}$ based on the co-occurrence in $\mathcal{A}$. Concretely, firstly, we transform the elements of set $\mathcal{V}$ into lower characters into lower characters to avoid the influence of capitalization.
% Secondly, we replace all special characters with spaces to unify identical key elements.  Following this, we link key elements based on their co-occurrence within the same atomic facts. To enable the agent to review the original text details in $D$ with key information and relevant atomic facts, we construct a tree for each node within the memory graph. 

% Additionally, in the construction of $\mathcal{G}$, we do not use the input question $q$ as a condition, therefore, $\mathcal{G}$ can assist agents in addressing a variety of questions and instructions, making the graph reusable.

To extract nodes from a given document $D$ within the limited context length of LLM, we first segment $D$ into independent chunks, each with a maximum length of $L$, while striving to maintain the integrity of the paragraph structure. For each chunk, we prompt the LLM to summarize it into a series of atomic facts, which are the smallest indivisible facts that simplify the original text. Meanwhile, we prompt the LLM to extract key elements from each atomic fact, such as essential nouns, verbs, and adjectives critical to the text's narrative.
After processing all chunks, we normalize the key elements following~\citealp{lu2023instag} to address lexical noise and uncontrolled granularity issues, resulting in the final key elements set. Subsequently, we construct each node $v_i = \left\{k_i, \mathcal{A}_i\right\}$ based on the mapping between key elements and atomic facts, where $k_i$ is a key element, and $A_i$ is all atomic facts corresponding to $k_i$. Finally, we link two nodes $v_i$ and $v_j$ if key element $k_i$ occurs in the atomic facts set $A_j$ and vice versa.

It is worth noting that the graph construction is not bound to any specific question answer pairs. Consequently, this graph can be reused to response various questions, thereby reducing redundant input in scenarios involving multiple QA from a single document or multi-turn QA.

\subsection{Graph Exploration}

% After constructing the memory graph $\mathcal{G}$, we can build the long-range dependencies of $D$ to assist the agent in acquiring comprehensive context information. To enable agents to read long texts through graphs, existing studies~\citep{} utilize a two-step process of evidence generation followed by retrieval of the next node for graph traversal. However, these strategies do not facilitate the planning and reflective thinking of LLMs, thereby diminishing the efficacy of these methods. Inspired by recent advances in agent-based studies~\citep{}, we employ a short context window LLM as agent to traverse, reflect, and summarize on $\mathcal{G}$, called \textbf{\ourmethod}. We introduce a three stages methods in agent's reasoning process of our \ourmethod, namely initialization, exploration, and reasoning.


\subsubsection{Initialization of Agent}

% To improve search efficiency of employing an agent to traverse the memory graph $\mathcal{G}$, we refine initialization in our approach from three dimensions: planning, node selection, and agent setup.


% \paragraph{Initial Planning} Inspired by existing work~\citep{}, to effectively analyze the requirements of the input instruction $q$ and guide subsequent agent in deep search on the graph, we introduce pre-planning in our \ourmethod. Specifically, given an instruction $q$, we prompt the LLM to analysis the information that the agent need to acquire from $\mathcal{G}$ to adequately respond to this instruction, severing as guidance and objectives of the agents during the search process. This procedure can be demoted as $p = \text{GPT-4}(q, P_p)$, where $p$ denotes the result of pre-planning based on the input instruction, and $P_p$ serves as the prompt to guide the LLM and is shown in Appendix \ref{app: agent_prompts}.


% \paragraph{Initial Node Selection} Duo to the substantial quantity of extracted key elements $\mathcal{V}$ from $D$, to reduce search steps of \ourmethod and improve the response delay, we employ a score-based strategy for initial node selection in deep search. This strategy utilizes the outcomes of pre-planning $p$, extracted key elements set $\mathcal{V}$ and instruction $q$. Concretely, when the aggregate length of key elements falls within the context window of LLM, we utilize proper prompt for guiding LLM to score the potential to assist in addressing the input instruction $q$. Conversely, if the combined length of the key elements surpasses the context window's capacity, we initially partition $\mathcal{V}$ into sections, then instruct GPT-4 to identify and evaluate the most pertinent key elements from each section, following the aforementioned scoring approach, denoted as:
% \begin{equation}
%     {s_i} = \text{GPT-4}(P^S, \mathcal{V}, q, p)
% \end{equation}
% where $s_i$ indicates the scored relevance of $v_i \in \mathcal{V}$, and $P^S$ designates the scoring prompt for GPT-4, detailed in Appendix~\ref{tab: search_beginning_nodes}. Through this process, we prioritize the $N$ highest-scoring key elements as the initial search nodes in deep search for \ourmethod.

% \paragraph{Initial Agent Setup}

% Inspired by existing works~\citep{}, in order to enhance the efficiency of deep search and augment the agent's capacity for reflection, we introduce a dynamic memory space $\mathcal{M}$ for the agent. This memory will combine previous memory with the key insights and findings about the question with current atomic facts, yielding a comprehensive memory construct. Additionally, to reduce repetitive and redundant actions by the agent and accelerate main search process, we keep a record of the agent's historical actions in a queue $\mathcal{H}$. Therefore, before conducting a deep search search on $\mathcal{G}$, we first reset the memory space $\mathcal{M}$ and action history $\mathcal{H}$ to a blank state.

Given a graph $\mathcal{G}$ and a question $Q$, our goal is to design an agent capable of autonomously exploring the graph using predefined functions. And the agent should have a notebook to record collected supporting facts, which will be used to reasoning the final answer. In addition to actions and notebook, the agent is prepared in two further dimensions to efficiently explore the graph: rational path and initial node.

\paragraph{Rational Path} To address the complex read-world multi-hop questions, pre-planning the solution is crucial. Therefore, the agent decomposes the original question step-by-step and identifies the key information needed as a rational path.

\paragraph{Initial Node} A good starting point is crucial for improving search efficiency. The agent checks the key elements of all nodes $\mathcal{V}$ and selects $N$ initial nodes based on the question and the rational path.


\subsubsection{Exploration}
% Read Node
% Read AF
%   Read TF
% Read NB
After selecting $N$ initial nodes, we treat them as the starting points for $N$ diverse paths. An agent is then tasked to begin exploration along each node, guided by the question and the rational plan, concurrently updating the notebook with relevant information acquired during exploration.

\paragraph{Exploring Node Atomic Facts}
It is impractical to include all original text chunks related to a node within the context window. Therefore, the agent employs a coarse-to-fine strategy, progressing from reading atomic facts to the original text, as all atomic facts can fit within the context window. Initially, all atomic facts associated with a node are grouped by their corresponding chunks, labeled with the respective chunk IDs, and fed to the agent. This allows the agent to gain an overview of each chunk by reading all clusters of atomic facts. Meanwhile, the agent utilizes the question, rational plan, and notes in its notebook to determine whether any of these chunks are of interest. 
Subsequently, the agent are provided two functions: 1) \textit{read\_chunk}, if the agent identifies certain chunks as valuable for further reading, it will complete the function parameters with the chunk IDs, \ie \textit{read\_chunk(List[ID])}, and append these IDs to a chunk queue. 2) \textit{stop\_and\_read\_neighbor}, conversely, if the agent deems that none of the chunks are worth further reading, it will finish reading this node and proceed to explore neighboring nodes.
%===============================================================
\begin{table*}[!ht]
\centering
% \scriptsize
\begin{tabular}{clcccc}
\bottomrule
                  \textbf{Task} & \textbf{Dataset}  & Source & Avg Ctx. Len & Max Ctx. Len & \#data  \\ \hline
\multirow{4}{*}{\textbf{Multi-hop QA}} & HotpotQA\_e & LongBench & 9.4k & 15.9k & 300  \\
                     & 2WikiMultihopQA\_e & LongBench & 8.8k & 15.9k & 300 \\
                    & MuSiQue & LongBench & 15.5k & 16.0k & 200 \\
                    & HotpotWikiQA-mixup & LV-Eval & 142.4k & 370.8k & 50 $\times$ 5 \\ \hline
% \multirow{1}{*}{\textbf{Single-hop QA}} &narrativeQA & English & 29.7k & 200 
\textbf{Single-hop QA} & NarrativeQA & LongBench & 29.7k & 63.7k & 200 \\\bottomrule
\end{tabular}
\caption{The datasets used for evaluation comprise both single-hop and multi-hop QA. "Avg Ctx. Len" and "Max Ctx. Len" respectively refer to the average and maximum number of tokens calculated using the gpt-4 tokenizer from the tiktoken\protect\footnotemark package, and "\#data" indicates the quantity of Context-Question-Answer pairs.}
\label{tab: datasets}
\end{table*}
\footnotetext{https://github.com/openai/tiktoken}
%===============================================================
\paragraph{Exploring Node Chunks}
When the chunk queue is non-empty, it indicates that the agent has identified multiple text chunks of interest. We then traverse the queue, reading each chunk. This step is essential because atomic facts merely summarize key information and provide brief clues, whereas specific details are best obtained directly from the original text chunks. 
While reading the chunks, the most crucial task is to update the notebook based on the question, rational path, and the content of the chunks, thereby collecting supporting facts for answering. Depending on the updated notebook, the agent will then select one of the following four actions: 1) \textit{search\_more}, if supporting fact is insufficient, the agent will continue exploring chunks in queue; 2) \textit{read\_previous\_chunk} and 3)\textit{read\_subsequent\_chunk}, due to truncation issues, adjacent chunks might contain relevant and useful information, the agent may add these IDs to the queue; 4) \textit{termination}, if sufficient information has been gathered for answering the question, the agent will finish exploration.
\paragraph{Exploring Node Neighbors}
Once the atomic facts and chunk queue of the current node have been fully processed, it indicates that this node has been thoroughly explored, and the agent needs to access the next node. Taking into account the question, rational path, and the current memory, the agent checks all neighboring nodes, \ie key elements, and preforms one of two actions: 1) \textit{read\_neighbor\_node}, the agent selects a neighboring node that might be helpful in answering the question and re-enters the process of exploring atomic facts and chunks; 2) \textit{termination}, the agent determines that none of the neighboring nodes contain useful information, it finish exploration.

\subsection{Answer Reasoning}
After $N$ agents have independently gathered information and stopped their exploration, we will compile all notes from each agent for reasoning and generating the final answer. Employing the Chain-of-Thought~\cite{} method, the LLM first analyze each notes by considering complementary information from other memories and using a majority voting strategy to resolve any inconsistencies. Ultimately, the LLM will consider all the available information to generate the final answer.


%initial nodes selection, medium planning, concludes and summary 


==> content/cache/exp_caceh.tex <==
%---------------------------------------------------------
% \begin{table*}[!t]

% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{ccccccc|ccccc|ccccc|ccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Method}} & \textbf{Input} & \multicolumn{5}{c}{\textbf{HotpotQA}} & \multicolumn{5}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{5}{c}{\textbf{MuSiQue}} &  \multicolumn{5}{c}{\textbf{NarrativeQA}}\\ \cline{3-22}
%      & \textbf{Window} & LR-1 & LR-2 & EM & $F_1$ & Rouge-L & LR-1 & LR-2 & EM & $F_1$ & Rouge-L & LR-1 & LR-2 & EM & $F_1$ & Rouge-L & LR-1 & LR-2 & EM & $F_1$ & Rouge-L\\ \hline
%     BM25 Retrieval & $4k$ & 57.7 & 63.0 & 33.7 & 43.8 & 44.4 & 36.0 & 39.0 & 25.0 & 30.4 & 30.9 & 33.0 & 36.5 & 19.0 & 23.9 & 23.9 & 29.5 & 34.5 & 4.0 & 11.3 & 11.1 \\
%     OpenAI Embedding Retrieval & $4k$ & 63.0 & 70.7 & 40.0 & 53.2 & 53.2 & 57.0 & 59.3 & 41.0 & 49.4 & 49.5 & 34.5 & 37.0 & 20.0 & 26.6 & 26.6 & 37.5 & 46.5 & 5.0 & 15.5 & 15.3 \\
%     Full Text Read & $128k$ & \underline{83.3} & \underline{88.3} & \underline{53.0} & \underline{68.4} & \underline{68.4} & 77.3 & 80.0 & \underline{58.7} & \underline{70.0} & \underline{70.0} & 52.0 & 59.5 & 33.5 & 42.7 & 42.4 & \underline{63.5} & \underline{77.0} & \underline{11.5} & \underline{29.4} & \underline{29.1}  \\
%     Chunk Read & $4k$ & 71.3 & 74.7 & 45.7 & 59.5 & 59.7 & 59.3 & 62.3 & 40.7 & 50.5 & 50.5 & 41.0 & 43.0 & 23.0 & 32.1 & 32.0 & 58.0 & 69.5 & 9.50 & 25.5 & 25.4  \\
%     Chunk Read with Memory & $4k$ & 72.3 & 76.7 & 45.7 & 59.5 & 59.7 & 65.7 & 68.7 & 46.3 & 56.6 & 56.7 & 39.5 & 43.0 & 25.0 & 32.5 & 32.1 & 56.5 & 65.0 & 8.5 & 24.3 & 24.0  \\
%     ReadAgent & $128k$ & 72.3 & 78.7 & 48.0 & 62.0 & 62.1 & \underline{79.0} & \underline{81.0} & 52.7 & 63.7 & 63.7 & \underline{54.5} & \underline{61.0} & \underline{35.0} & \underline{45.1} & \underline{44.9} & 63.0 & 75.5 & 5.0 & 18.9 & 18.8  \\ 
%     \ourmethod & $4k$ &\textbf{84.3} & \textbf{89.7} & \textbf{55.0} & \textbf{70.0} & \textbf{70.0} & \textbf{83.7} & \textbf{87.0} & \textbf{59.3} & \textbf{70.1} & \textbf{70.1} & \textbf{59.0} & \textbf{63.5} & \textbf{38.0} & \textbf{47.4} & \textbf{47.4} & \textbf{65.0} & \textbf{80.0} & \textbf{15.5} & \textbf{29.8} & \textbf{29.6} \\
%     \hline
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Performance(\%) of different baselines on datasets from LongBench. The best and runner-up are in bold and underlined.}
% % \vspace{-0.5cm}
% \label{tab: main_result_1}
% \end{table*}

\section{Experiments}

\subsection{Implementation Details}


In the experiments conducted for this study, the LLM used was \textit{gpt-4-1106-preview} for all methods, accessed through API, with the temperature set to $0.2$. This model provided by OpenAI supports a maximum input of $128k$ tokens and an output of $4k$ tokens~($1k=1024$).

In the experiments with \ourmethod, unless otherwise specified, we default to a maximum chunk length of $L=2k$, initiate the search from $5$ initial nodes,  impose a function call limit of $10$ for each search path~(search will stop upon reaching this limit), and set the input window size to $L=4k$.
% We conduct experiments on multiple long text datasets to evaluate the effectiveness of our method. Some datasets come from LongBench~\citep{Bai2023LongBenchAB}, including multi-hop datasets: HotpotQA, 2WikiMultihopQA, MuSiQue, and single-hop dataset: NarrativeQA. 
% % In addition, we also perform experiments on the HotpotWikiQA-mixup dataset from LV-Eval~\citep{Yuan2024LVEvalAB}, which has an ultra-long text length (nearly $100$ times the $4k$ input window), to demonstrate the advantages of our method in handling ultra-long texts.
% Additionally, we conducted experiments on the LV-Eval's HotpotWikiQA-mixup dataset~\citep{Yuan2024LVEvalAB}, a multi-hop dataset with input texts extending up to 256k tokens, thereby evaluating the performance of our method on texts that greatly exceed the input window by dozens of times.\\
% In this study, we employ \textit{gpt-4-1106-preview} for experimentation and evaluation purposes. Further details on the implementation of \ourmethod can be found in Appendix \ref{app: imp_details}.
%===============================================================
\begin{table}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{clccc}
\bottomrule
                  \textbf{Task} & \textbf{Dataset}  & Avg. Ctx. Len & Max Ctx. Len & \#Data  \\ \hline
\multirow{4}{*}{\textbf{Multi-hop QA}} & HotpotQA  & 9.4k & 15.9k & 300  \\
                     & 2WikiMultihopQA  & 8.8k & 15.9k & 300 \\
                    & MuSiQue  & 15.5k & 16.0k & 200 \\
                    & HotpotWikiQA-mixup  & 142.4k & 370.8k & 50 $\times$ 5 \\ \hline
% \multirow{1}{*}{\textbf{Single-hop QA}} &narrativeQA & English & 29.7k & 200 
\textbf{Single-hop QA} & NarrativeQA  & 29.7k & 63.7k & 200 \\\bottomrule
\end{tabular}
}
\caption{The datasets used for evaluation comprise both single-hop and multi-hop QA. "Avg Ctx. Len" and "Max Ctx. Len" respectively refer to the average and maximum number of tokens calculated using the GPT-4 tokenizer from the tiktoken\protect\footnotemark package, and "\#data" indicates the quantity of Context-Question-Answer pairs.}
\label{tab: datasets}
\end{table}
\footnotetext{https://github.com/openai/tiktoken}
%===============================================================
\subsection{Datasets and Evaluation Metrics}
\paragraph{Dataset} We conduct experiments on multiple long-context datasets to evaluate the effectiveness of our method. Some datasets come from LongBench~\citep{Bai2023LongBenchAB}, including multi-hop QA datasets: \textbf{HotpotQA}, \textbf{2WikiMultihopQA,} \textbf{MuSiQue}, and a single-hop QA dataset: \textbf{NarrativeQA}. 
% Additionally, we conducted experiments on the LV-Eval's \textbf{HotpotWikiQA-mixup} dataset~\citep{Yuan2024LVEvalAB},
% a multi-hop dataset with input texts extending up to 256k tokens, thereby evaluating the performance of our method on texts that greatly exceed the input window by dozens of times. 
Moreover, we conducted experiments on the \textbf{HotpotWikiQA-mixup} dataset from LV-Eval~\citep{Yuan2024LVEvalAB}, which is a multi-hop dataset with five length levels ($16k$, $32k$, $64k$, $128k$, and $256k$) reaching up to approximately $370.8k$ (Table \ref{tab: datasets}), nearly one hundred times the size of the $4k$ input window used in our experiments. Statistical information about the datasets is shown in the table \ref{tab: datasets} and a detailed description can be found in the Appendix \ref{app: datasets}.

\paragraph{Evaluation Metrics} We follow the official metrics from each dataset, employing $F_1$ score and EM~(Exact Match) score on the LongBench dataset, and a two-stage $F_1$ score on the LV-Eval dataset which first computes the recall of golden answer keywords and only calculates the $F_1$ score if it exceeds a certain threshold; otherwise, it returns 0. We refer to this as $F_1$*. Although N-gram metrics offer evaluations at a significantly low cost, their accuracy is compromised by the format of LLM responses and the presence of non-informative words within the answers. Therefore, we adopt the approach of employing LLM Raters for answer correctness evaluation using an LLM, as demonstrated by ReadAgent~\citep{lee2024human}. Detailed information about the evaluation process is provided in Appendix \ref{app: eval_details}.

% \ignore{\paragraph{Evaluation Metrics}For datasets from LongBench, evaluation is conducted using the standard $F_1$ score. In addition, we also calculated the score of EM (Exact Match). The LV-Eval dataset undergoes a more detailed process, calculating a two-stage $F_1$ score, which first computes the recall of golden answer keywords and only calculates the $F_1$ score if it exceeds a certain threshold; otherwise, it returns 0. We refer to this as $F_1$*. 
% Although N-gram metrics offer evaluations at a significantly low cost, their accuracy is compromised by the format of LLM responses and the presence of non-informative words within the answers. Therefore, we adopt the approach of employing LLM Raters for answer correctness evaluation using an LLM, as demonstrated by ReadAgent~\citep{lee2024human}. Detailed information about the evaluation process is provided in Appendix \ref{app: eval_details}.}

% More specifically, given a question, the corresponding true answer, and the LLM's response, we use an LLM to evaluate the response based on the question and true answer. Two distinct scores are involved: LLM-Rating-1 (LR-1) and LLM-Rating-2 (LR-2), where LR-1 represents a strict scoring criterion, and LR-2 represents a lenient one. Following ReadAgent, if any LLM raters deem the answer correct, we consider it correct. If the strict rater considers the response incorrect, but the lenient rater sees part of the answer as correct, we consider the answer partially correct; otherwise, we judge it as incorrect.

\subsection{Baseline Methods}
In our experiments, we compared various baselines, including the traditional RAG method: using Okapi BM25~\citep{Robertson2009ThePR} or the OpenAI API embedding model (text-embedding-ada-002)\footnote{https://platform.openai.com/docs/guides/embeddings/\linebreak embedding-models} to retrieve the chunks most relevant to the question, then reading and answering the question based the chunks; direct use of LLM for full-text reading (when the text content fits within the input window) or segmenting into chunks for sequential reading; and agent-based methods like ReadAgent~\citep{lee2024human}. Detailed 
description and implementation of these methods are provided in Appendix \ref{app: baseline}.

% \textbf{Retrieval-Augmented Generation (RAG)}: In this work, we compare the traditional RAG method, including retrieval methods based on Okapi BM25~\citep{Robertson2009ThePR} and the ApenAI API embedding model (text-embedding-ada-002)\footnote{https://platform.openai.com/docs/guides/embeddings/\linebreak embedding-models}. Specifically, we first split the text into fragments in the same method as \ourmethod, then use the aforementioned methods to calculate the relevance scores between the question and these text fragments, and finally combine the fragments with the highest relevance scores with the question for the LLM to answer.
% % To ensure a fair comparison, we control the input window to 4k (4096) in the subsequent experiments. Specifically, we set the maximum length of text fragments to 3800 so that, after including the prompt, it fits just within 4k. We then have the LLM answer based on the text fragment with the highest relevance score. The specific prompt can be found in Appendix \ref{app: rag}.\\

% \textbf{Full or Chunked Text Content}: For texts with fewer tokens than the LLM's input window, we can input the text directly into the LLM to obtain an answer. We refer to this method as "Full Text Read", with the specific prompt provided in Appendix \ref{app: overall_read}. 
% % However, this approach is not applicable to texts exceeding the token limit of the LLM's input window. In such cases, \citeauthor{lee2024human} truncated the text to fit it into the LLM, but this method obviously results in information loss. We propose a method that does not lose information, offering a better comparison. This method involves 
% For texts exceeding the token limit of the LLM's input window, we divide the entire text into text chunks (using the same chunking method as \ourmethod) and then have the LLM read these text chunks sequentially according to the text order, thus enabling the handling of overly long texts with a limited input window. During the reading process, there are two main strategies: Chunk Read and Chunk Read with Memory. In the Chunk Read approach, the LLM only sees the current text fragment during each reading. In the Chunk Read with Memory approach, the LLM can summarize useful information from the current text chunk and provide it to the subsequent reading process.
% % In the Chunk Read approach, the LLM only sees the current text fragment during each reading, which is suitable for single-hop QA tasks. In the Chunk Read with Memory approach, the LLM can summarize useful information from the current text chunk and provide it to the subsequent reading process, which is suitable for multi-hop QA tasks. The specific prompts can be found in Appendix \ref{app: chunk_read}.\\

% \textbf{ReadAgent}: We also compared our method with similar approaches for handling long texts with small input windows, such as ReadAgent~\citep{lee2024human}. ReadAgent is a method that segments long texts and generates gist memories, which are then looked up to search for information in order to answer questions. Implementation details can be found in Appendix \ref{app: readagent_imp_details}.
%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc|cccc|cccc|cccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \textbf{Input} & \multicolumn{4}{c}{\textbf{HotpotQA}} & \multicolumn{4}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{4}{c}{\textbf{MuSiQue}} &  \multicolumn{4}{c}{\textbf{NarrativeQA}}\\ \cline{3-18}
     & \textbf{Window} & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$\\ \hline
     \multicolumn{18}{l}{BM25 Retrieval} \\ \hline
    Top-1 & 4k & 57.7 & 63.0 & 33.7 & 43.8 & 36.0 & 39.0 & 25.0 & 30.4 & 33.0 & 36.5 & 19.0 & 23.9 & 29.5 & 34.5 & 4.0 & 11.3 \\
Top-3 & 4k & 74.7 & 78.3 & 45.7 & 58.5 & 59.7 & 62.0 & 42.3 & 51.9 & 43.5 & 49.5 & 25.0 & 31.1 & 44.5 & 52.5 & 7.0 & 20.5 \\ \hline
\multicolumn{18}{l}{OpenAI Embedding Retrieval} \\ \hline
Top-1 & 4k & 63.0 & 70.7 & 40.0 & 53.2 & 57.0 & 59.3 & 41.0 & 49.4 & 34.5 & 37.0 & 20.0 & 26.6 & 37.5 & 46.5 & 5.0 & 15.5 \\
Top-3 & 4k & 72.0 & 77.3 & 45.0 & 58.1 & 65.7 & 66.7 & 44.7 & 55.3 & 40.0 & 45.5 & 24.5 & 32.1 & 45.5 & 53.0 & 7.5 & 19.5 \\ \hline
    Full Text Read & $128k$ & \underline{83.3} & \underline{88.3} & \underline{53.0} & \underline{68.4} & 77.3 & 80.0 & \underline{58.7} & \underline{70.0} & 52.0 & 59.5 & 33.5 & 42.7 & \underline{63.5} & \underline{77.0} & \underline{11.5} & \underline{29.4}  \\
    Chunk Read & $4k$ & 71.3 & 74.7 & 45.7 & 59.5 & 59.3 & 62.3 & 40.7 & 50.5 & 41.0 & 43.0 & 23.0 & 32.1 & 58.0 & 69.5 & 9.50 & 25.5  \\
    Chunk Read with Memory & $4k$ & 72.3 & 76.7 & 45.7 & 59.5 & 65.7 & 68.7 & 46.3 & 56.6 & 39.5 & 43.0 & 25.0 & 32.5 & 56.5 & 65.0 & 8.5 & 24.3  \\\hline
    ReadAgent & $128k$ & 72.3 & 78.7 & 48.0 & 62.0 & \underline{79.0} & \underline{81.0} & 52.7 & 63.7 & \underline{54.5} & \underline{61.0} & \underline{35.0} & \underline{45.1} & 63.0 & 75.5 & 5.0 & 18.9 \\ 
    \ourmethod & $4k$ &\textbf{84.3} & \textbf{89.7} & \textbf{55.0} & \textbf{70.0} & \textbf{83.7} & \textbf{87.0} & \textbf{59.3} & \textbf{70.1} & \textbf{59.0} & \textbf{63.5} & \textbf{38.0} & \textbf{47.4} & \textbf{65.0} & \textbf{80.0} & \textbf{15.5} & \textbf{29.8} \\
    \hline
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) of different baselines on datasets from LongBench. The best and runner-up are in bold and underlined.}
% \vspace{-0.5cm}
\label{tab: main_result_1}
\end{table*}
%---------------------------------------------------------
 % \multirow{4}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}}} \\
 % & & & & & & & & & & & & & & & & \\
 % & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccc|ccc|ccc|ccc|ccc}
\hline
 \multirow{3}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}} \\
 & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
& & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$*\\ \hline
\multicolumn{17}{l}{BM25 Retrieval} \\ \hline
Top-1 & $4k$ & 10.0 & 16.0 & 12.0 & 16.0 & 18.0 & 11.9 & 6.0 & 8.0 & 8.5 & 10.0 & 8.0 & 7.0 & 14.0 & 20.0 & 5.9 \\
Top-3 & $4k$ & 16.0 & 22.0 & 13.9 & 18.0 & 28.0 & 13.3 & 16.0 & 18.0 & 11.8 & 12.0 & 16.0 & 11.8 & 12.0 & 22.0 & 9.3 \\ \hline
\multicolumn{17}{l}{OpenAI Embedding Retrieval} \\ \hline
Top-1 & $4k$ & 10.0 & 12.0 & 14.5 & 14.0 & 18.0 & 11.3 & 10.0 & 12.0 & 12.5 & 12.0 & 14.0 & 9.4 & 8.0 & 8.0 & 7.0 \\
Top-3 & $4k$ & 24.0 & 28.0 & 21.3 & 20.0 & 30.0 & 19.8 & 14.0 & 20.0 & 12.9 & 16.0 & 20.0 & 12.0 & 14.0 & 18.0 & 10.8 \\  \hline
Full Text Read & $128k$ & {\underline {38.0}} & {\underline {38.0}} & {\underline {35.7}} & {\underline {26.0}} & {\underline {30.0}} & {\underline {26.0}} & 22.0 & 24.0 & 20.6 & 16.0 & 16.0 & 14.6 & 14.0 & 16.0 & 10.3 \\
Chunk Read & $4k$ & 18.0 & 22.0 & 24.6 & 16.0 & 20.0 & 17.7 & 20.0 & 24.0 & 17.0 & 20.0 & 24.0 & 14.7 & {\underline {28.0}} & {\underline {30.0}} & 10.7 \\
Chunk Read with Memory & $4k$ & 22.0 & 32.0 & 24.2 & 26.0 & 30.0 & 21.3 & {\underline {28.0}} & {\underline {32.0}} & {\underline {22.0}} & {\underline {24.0}} & {\underline {26.0}} & {\underline {17.4}} & 26.0 & 26.0 & {\underline {14.8}} \\
ReadAgent & $128k$ & 24.0 & 26.0 & 29.2 & 20.0 & 22.0 & 16.9 & 24.0 & 30.0 & 15.3 & 14.0 & 18.0 & 13.6 & 20.0 & 22.0 & 10.4 \\
\ourmethod & $4k$ & \textbf{42.0} & \textbf{42.0} & \textbf{38.2} & \textbf{32.0} & \textbf{38.0} & \textbf{36.4} & \textbf{30.0} & \textbf{36.0} & \textbf{32.9} & \textbf{28.0} & \textbf{34.0} & \textbf{30.6} & \textbf{30.0} & \textbf{38.0} & \textbf{33.0} \\
\hline
\end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) of different baselines on datasets from LV-Eval, where $F_1$* donates LV-Eval's optimized $F_1$. The best and runner-up are in bold and underlined. We truncate to keep the longest possible initial fragment while preserving paragraph structure, in contexts that exceed the input window ($128k$ and $256k$) for Full Text Read.}
% \vspace{-0.5cm}
\label{tab: main_result_2}
\end{table*}
%---------------------------------------------------------
\subsection{Main Results}
Table \ref{tab: main_result_1} reports the main results of \ourmethod compared with other baselines across different datasets. Our method outperforms all baseline methods across various evaluation metrics on all assessed datasets. These datasets include both single-hop and multi-hop QA datasets, thereby demonstrating the superiority and robustness of \ourmethod in managing various long-context QA scenarios. Notably, the Full Text Read method obtained suboptimal results on several datasets, showcasing the strong capabilities of LLMs in handling QA problems with lengths smaller than the input window. Nevertheless, it is still surpassed by \ourmethod, proving the superiority of our approach in processing text within the input window. 

The RAG method performs the worst, and although selecting more fragments can lead to improved results, the enhancement potential is limited due to the input window restriction, making it challenging to surpass other methods.

For the results of Chunk Read, the method with memory performs better on multi-hop QA datasets than the method without memory because carrying memory evidently makes it easier to gather multiple supporting facts. However, on single-hop QA datasets, the latter performs better. This could be due to the additional memory introducing confusion.

Additionally, we explored the performance of \ourmethod on texts of different lengths, from $16k$ to $256k$. Table \ref{tab: main_result_2} presents the results on different metrics for the HotpotWikiQA-mixup dataset, where the context lengths vary. Our method surpasses all baselines across all lengths (from $16k$ to $256k$). It is noteworthy that using a tokenizer from GPT-4, the maximum context length can reach up to $370k$ (as shown in Table \ref{tab: datasets}), which is nearly a hundred times the size of our employed input window ($4k$).

The experimental results from Table \ref{tab: main_result_2} verify that the capability of our method to handle long contexts extends beyond the limitations of the 4k input window, highlighting our approach's advanced capabilities in managing extremely long contexts.

% Table \ref{tab: main_result_1} and Table \ref{tab: main_result_2} report the main results compared with other baselines on different datasets.
% As shown in Table \ref{tab: main_result_1}, our method outperforms all baseline methods on different evaluation metrics for all evaluation datasets, proving the effectiveness of our method. In particular, our method achieves excellent results on both single-hop and multi-hop datasets, demonstrating its robustness in managing diverse long-context QA scenarios.

% Table \ref{tab: main_result_2} showcases the results of different metrics on the HotpotWikiQA-mixup dataset with varying lengths of context. Our method outperforms all baselines across all lengths from 16k to 256k. Notably, utilizing the tokenizer from gpt-4, the maximum context length reaches up to 370k (as shown in Table \ref{tab: datasets}).
% % , which is nearly a hundred times greater than the input window (4k). This demonstrates the superiority of our approach in handling exceptionally long contexts.
% The capability of \ourmethod in handling long contexts is significantly beyond the limitation of the 4k input window, highlighting our method's advanced proficiency in handling extremely lengthy contexts.

% As shown in Table \ref{tab: main_result_1}, \ourmethod outperforms all baseline methods across all evaluation metrics, particularly on multi-hop datasets such as HotpotQA, 2WikiMultihopQA, and MuSiQue, demonstrating the superiority of our approach in dealing with multi-hop QA. 

% The experimental results of different methods on datasets from LongBench are presented in Table \ref{tab: main_result_1}. Our \ourmethod achieved the best performance across all evaluation metrics, particularly on the multi-hop datasets such as HotpotQA, 2WikiMultihopQA, and MuSiQue, demonstrating the superiority of our approach in dealing with multi-hop QA. Furthermore, \ourmethod also exhibits advantages on the single-hop QA dataset (NarrativeQA), reflecting the effectiveness of our approach in pinpointing fine-grained information. 
% It is worth noting that \ourmethod surpassed Full Text Read to varying extents, strongly proving the effectiveness of our approach.



% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccccccccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input Window}} & \multicolumn{3}{c}{\textbf{HotpotQA}} & \multicolumn{3}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{3}{c}{\textbf{MuSiQue}} &  \multicolumn{3}{c}{\textbf{NarrativeQA}}\\ \cline{3-14} 
%      & & LR-1 & LR-2 & $F_1$ & LR-1 & LR-2 & $F_1$ & LR-1 & LR-2 & $F_1$ & LR-1 & LR-2 & $F_1$\\ \hline
%     w/o pp. & $4k$ & 0.817 & 0.877 & 0.109 & 0.823 & 0.860 & 0.146 & 0.560 & 0.610 & 0.082 & 0.630 & 0.785 &  0.100 \\
%     w/o mem. & $4k$ &  &  &  &  &  &  &  &  &  &  &  &   \\
%     w/o both & $4k$ &  &  &  &  &  &  &  &  &  &  &  &   \\
%     Info-Graph Agent & $4k$ &\textbf{0.843} & \textbf{0.897} & 0.190 & \textbf{0.837} & \textbf{0.870} & \textbf{0.258} & \textbf{0.590} & \textbf{0.635} & \textbf{0.156} & \textbf{0.650} & \textbf{0.800} & 0.160  \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Ablation study on datasets from LongBench.}
% % \vspace{-0.5cm}
% \label{ablation}
% \end{table*}
%---------------------------------------------------------
%---------------------------------------------------------
% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{4}{c}{\textbf{\#Initial Nodes}}\\ \cline{3-6} 
%        &  & 4 & 7 & 10 & 13 \\ \hline
    
%     \multirow{2}{*}{\textbf{2WikiMultihopQA}} & LR-1 & 74.3 & 81.7 & 83.7 & \textbf{85.0} \\
%         & LR-2 & 76.3 & 83.7 & \textbf{87.0} & 85.7 \\\hline

%     \multirow{2}{*}{\textbf{NarrativeQA}} & LR-1 & 57.5 & 58.0 & \textbf{65.0} & 58.5 \\
%         & LR-2 & 71.5 & 73.0 & \textbf{80.0} & 73.5 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Performance(\%) of \ourmethod with changes in the initial nodes. The best are in bold.}
% % \vspace{-0.5cm}
% \label{tab: starting_nodes}
% \end{table}

% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{4}{c}{\textbf{\#Initial Nodes}}\\ \cline{3-6} 
%        &  & 1 & 4 & 7 & 10 \\ \hline
    
%     \multirow{2}{*}{\textbf{2WikiMultihopQA}} & LR-1 & 79.3 & 81.7 & 83.7 & \textbf{85.0} \\
%         & LR-2 & 81.3 & 84.7 & \textbf{87.0} & 85.7 \\\hline

%     \multirow{2}{*}{\textbf{NarrativeQA}} & LR-1 & 59.5 & 62.0 & \textbf{65.0} & 61.5 \\
%         & LR-2 & 74.5 & 76.0 & \textbf{80.0} & 75.5 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Performance(\%) of \ourmethod with changes in the initial nodes. The best are in bold.}
% % \vspace{-0.5cm}
% \label{tab: starting_nodes}
% \end{table}
%---------------------------------------------------------
\begin{table}[!t]
\centering
% \scriptsize
\resizebox{\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Results(\%)}}\\ \cline{3-5} 
     & & LR-1 & LR-2 & $F_1$ \\ \hline
    \multirow{3}{*}{\textbf{HotpotQA}} & \ourmethod & \textbf{84.3} & \textbf{89.7} & \textbf{70.0} \\
        & w/o rational path & 81.7 & 87.7 & 63.8 \\
        & w/o node selection & 66.0 & 71.7 & 54.1 \\\hline
    \multirow{3}{*}{\textbf{2WikiMultihopQA}}& \ourmethod & \textbf{83.7} & \textbf{87.0} & \textbf{70.1} \\
        & w/o rational path & 81.3 & 86.0 & 65.4 \\
        & w/o node selection & 65.3 & 68.7 & 49.7 \\\hline
    \multirow{3}{*}{\textbf{MuSiQue}} & \ourmethod & \textbf{59.0} & \textbf{63.5} & \textbf{47.4} \\
    & w/o rational path & 56.0 & 61.0 & 42.4 \\
    & w/o node selection & 35.0 & 38.5 & 25.2 \\\hline
    \multirow{3}{*}{\textbf{NarrativeQA}} & \ourmethod & \textbf{65.0} & \textbf{80.0} & \textbf{29.8}  \\
        & w/o rational path & 63.0 & 78.5 & 26.6 \\
        & w/o node selection & 53.0 & 65.5 & 24.0 \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{The results of our ablation experiments, where "w/o rational path" refers to the elimination of the pre-planning stage, and "w/o node selection" denotes the random selection of initial nodes and neighbor nodes.}
% \vspace{-0.5cm}
\label{tab: ablation}
\end{table}
%---------------------------------------------------------
\subsection{Ablation study}
We construct ablation experiments on various datasets to investigate the contribution of different components in our approach. 
For the ablation of the rational path, we remove this step during the initialization of the \ourmethod, aiming to explore whether it has a positive effect on the model's path selection. Moreover, we investigate the intelligence of the \ourmethod's selection by randomly choosing initial nodes and randomly replacing the parameter when selecting the read\_neighbor\_node function from candidate neighbor nodes.
% We implement without rational path experiments by removing the pre-planning stage . Without node selection refers to the elimination of the agent's autonomy in selecting initial and neighbor nodes, switching to random selection instead. Specifically, a random selection from all nodes is made for the initial nodes. When the agent chooses to read neighbor nodes, the model-selected neighbor node is replaced with a randomly chosen one from all neighbor nodes.
% Table \ref{tab: ablation} displays the results of our ablation experiments, where w/o pre-planning refers to the removal of the pre-planning stage. In fact, we set the plan to be fixed as "There is no plan to solve this question." W/o select refers to the elimination of the agent's autonomy in selecting starting and neighbor nodes, switching to random selection instead. Specifically, a random selection from all nodes is made for the starting nodes. When the agent chooses to read neighbor nodes, the model-selected neighbor node is replaced with a randomly chosen one from all neighbor nodes. In summary, w/o select implements a form of random walk. 

% The experimental results shown in Table \ref{tab: ablation} illustrate that the performance of \ourmethod declines when pre-planning is removed, and the decline is more significant on multi-hop QA datasets than on single-hop QA datasets, indicating the beneficial role of pre-planning in aiding the agent to pinpoint critical information. When the agent no longer selects nodes autonomously but instead wanders randomly, the performance of \ourmethod significantly drops. This demonstrates that \ourmethod does not merely search for information by traversing all chunks but intelligently selects the next node based on current memory and historical actions.
The experimental results in Table \ref{tab: ablation} show that when the rational path is removed, the performance of \ourmethod decreases, suggesting that the rational path aids \ourmethod in optimizing its exploration paths. With the guidance of a pre-planned rational path, \ourmethod is capable of planning its next move based on current progress. Moreover, the decline is more pronounced on multi-hop QA datasets than on single-hop QA datasets. This is because multi-hop QA requires more complex exploration paths, so without the guidance of the rational path, \ourmethod finds it more challenging to search for sufficient information to answer questions. When \ourmethod no longer autonomously selects nodes but instead wanders randomly, its performance significantly decreases. This indicates that \ourmethod indeed exhibits intelligence in its exploration process on the memory graph, choosing nodes based on the information acquired so far rather than aimlessly wandering and relying on randomness to collect supporting facts.
%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/figure3.pdf}
% \vspace{-0.6cm}
\caption{Performance of \ourmethod with different initial node numbers on 2WikiMultihopQA and NarrativeQA. Results show the robustness of \ourmethod towards different initial node numbers.}
\label{fig: nodes}
% \vspace{-0.6cm}
\end{figure}
%---------------------------------------------------------
\subsection{Further Analysis}
\paragraph{Impact of the Number of Initial Nodes}
To investigate the impact of the number of initial nodes on performances, we conduct experiments on both a multi-hop and a single-hop QA dataset. As shown in Figure \ref{fig: nodes}, when the number of initial nodes is relatively low ($<=7$), the performance of \ourmethod improves as the number of initial nodes increases. This is because more initial nodes usually provide more comprehensive information. 
However, when the number of initial nodes exceeds a certain threshold ($>7$), there is a slight decline in the final question-answering performance. This decline is attributed to the excessive memory of different paths, which leads to model confusion. 
For multi-hop QA, having a sufficient number of starting nodes is crucial. 
For example, in questions involving comparisons, the objects to be compared are often difficult to associate on the memory graph. 
% For example, in common comparative questions, the objects to be compared often have difficulty being associated on the memory graph. 
In such cases, selecting a starting node for each object becomes particularly important for searching for enough information to adequately answer the question.
% To investigate the impact of the number of initial nodes on the outcomes, we conducted experiments using datasets from both multi-hop QA and single-hop QA. The experimental results shown in Table \ref{tab: starting_nodes}  reveal that when the number of initial nodes is too low, the performance of \ourmethod improves with an increase in the number of initial nodes. However, the final QA performance slightly declines when the number of initial nodes is excessive. We believe this is due to the overabundance of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of initial nodes is more pronounced for single-hop QA.

% Table \ref{tab: starting_nodes} showcases the impact of different numbers of starting nodes, which are the number of search paths, on the final outcome. We selected one dataset each from multi-hop QA and single-hop QA datasets for experimentation to explore their respective effects on multi-hop QA and single-hop QA. The experimental results reveal that when the number of starting nodes is too low, the performance of \ourmethod improves with an increase in the number of starting nodes. However, the final QA performance slightly declines when the number of starting nodes is excessive. We believe this is due to the overabundance and disorganization of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of starting nodes is more pronounced for single-hop QA.
%---------------------------------------------------------
% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \hline
    
%     \textbf{Dataset} & \textbf{Avg Action Num(per trace)} & \textbf{Stage} & \textbf{Total Ratio} & \textbf{Selected Action} & \textbf{Selection Ratio}\\ \hline
%      % \multirow{7}{*}{\textbf{MuSiQue}} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{3}{*}{read_chunk} & \multirow{3}{*}{0.312(2185/7002)}
%      \multirow{7}{*}{MuSiQue} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.312(2185/7002)} & \textit{search\_more}s & 0.191(417/2185)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.266(582/2185) \\ 
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.257(561/2185) \\
%     &  &  &  & \textit{stop} & 0.286(625/2185) \\  \cline{3-6}
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.400(2800/7002)} & \textit{read\_chunk} & 0.413(1156/2800) \\ 
%     &  &  &  & \textit{stop} & 0.587(1644/2800) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.288(2017/7002)} & \textit{read\_neighbor\_node} & 0.401(809/2017)  \\ 
%     &  &  &  & stop & 0.599(1208/2017) \\ \hline
% \multirow{7}{*}{NarrativeQA} & \multirow{7}{*}{3.8475(7695/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.543(4176/7695)} & \textit{search\_more} & 0.041(171/4176)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.353(1475/4176) \\
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.326(1360/4176) \\
%     &  &  &  & \textit{stop} & 0.280(1170/4176) \\ 
%     \cline{3-6} 
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.325(2502/7695)} & \textit{read\_chunk} & 0.645(1615/2502) \\  
%     &  &  &  & \textit{stop} & 0.355(887/2502) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.132(1017/7695)} & \textit{read\_neighbor\_node} & 0.514(523/1017)  \\
%     &  &  &  & \textit{stop} & 0.486(494/1017)  \\
%     \hline
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Action statistics of \ourmethod on two datasets.}
% % \vspace{-0.5cm}
% \label{tab: action}
% \end{table*}
\begin{table*}[!t]
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \textbf{Dataset} & \textbf{\#Avg. Function Call} & \textbf{Stage} & \textbf{Stage Ratio(\%)} & \textbf{Function} & \textbf{Call Ratio(\%)}\\ \hline
 
     \multirow{7}{*}{MuSiQue} & \multirow{7}{*}{3.50} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{40.0} & \textit{read\_chunk} & 41.3 \\ 
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 58.7 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks}     & \multirow{4}{*}{31.2} & \textit{search\_more} & 19.1  \\
    &  &  &  & \textit{read\_previous\_chunk} & 26.6 \\ 
    &  &  &  & \textit{read\_subsequent\_chunk} & 25.7 \\
    &  &  &  & \textit{termination} & 28.6 \\  \cline{3-6}
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{28.8} & \textit{read\_neighbor\_node} & 40.1 \\
    &  &  &  & \textit{termination} & 59.9\\ \hline
\multirow{7}{*}{NarrativeQA} & \multirow{7}{*}{3.85} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{32.5} & \textit{read\_chunk} & 64.5 \\  
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 35.5 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks} & \multirow{4}{*}{54.3} & \textit{search\_more} & 4.1 \\
    &  &  &  & \textit{read\_previous\_chunk} & 35.3 \\
    &  &  &  & \textit{read\_subsequent\_chunk} & 32.6 \\
    &  &  &  & \textit{termination} & 28.0 \\ 
    \cline{3-6} 
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{13.2} & \textit{read\_neighbor\_node} & 51.4  \\
    &  &  &  & \textit{termination} & 48.6  \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{Statistics of function calls on MuSiQue and NarrativeQA.}
% \vspace{-0.5cm}
\label{tab: action}
\end{table*}
%---------------------------------------------------------
% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Avg Ctx. Tokens}} & \multirow{2}{*}{\textbf{Chunk Limit}} & \multirow{2}{*}{\textbf{Token Type}} & \multicolumn{2}{c}{\textbf{Stage}} \\ \cline{5-6} 
%        & & &  & avg atomic facts and key elements tokens & avg agent tokens \\\hline
%     \multirow{8}{*}{\textbf{HotpotWikiQA-mixup-256k}} & \multirow{8}{*}{366950.70} & \multirow{2}{*}{1k} & input token & 585770.34 & 90624.49   \\
%         & & & output token & 270179.60 &  13558.30 \\\cline{4-6}
        
%     & & \multirow{2}{*}{2k} & input token & 465931.14 & 69821.40 \\
%         & & & output token & 156201.42 & 11057.36  \\\cline{4-6}

%         & & \multirow{2}{*}{4k} & input token & 417449.46 & 93083.31   \\
%         & & & output token & 142652.42 & 10939.20  \\\cline{4-6}

%         & & \multirow{2}{*}{6k} & input token & 400457.94 & 76402.95  \\
%         & & & output token & 131023.17 & 9625.54 \\
       
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Consumption statistics of \ourmethod on two datasets. The input window is set to 4k, with 7 starting nodes, and a maximum of 10 actions. The upper limit of text fragments is 2k.}
% % \vspace{-0.5cm}
% \label{tab: cost}
% \end{table*}
%--------------------------------------------------------------
%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/figure4.pdf}
% \vspace{-0.2cm}
\caption{The impact of chunk size $L$ on the performance of \ourmethod.}
\label{fig: chunk_size_exp}
% \vspace{-0.2cm}
\end{figure}
%---------------------------------------------------------
\paragraph{Impact of the Chunk Size}

We explored the impact of the chunk's maximum length $L$ on the performance of \ourmethod. As shown in Figure \ref{fig: chunk_size_exp}, the results show that the best performance was achieved when $L=2k$. We believe that when $L$ is too large, the constructed memory graph lacks too much detail, leading to a decrease in performance. When $L=1k$, the performance is similar to $L=2k$, indicating that the latter can already extract details at an appropriate granularity. 

When $L$ is smaller, it is evident that more resources are consumed during the construction phase of the memory graph. Thus, to balance performance and consumption, a larger and more effective $L$ should be selected as the hyperparameter setting as much as possible.

% To balance consumption and performance, we think $L=2k$ is a good setting.
% To investigate the impact of input window size on \ourmethod, we conducted experiments on HotpotWikiQA-mixup-256k. We used different input window sizes, and the results in Figure \ref{fig: chunk} indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects one action: during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.

% Table \ref{tab: input_window} demonstrates the impact of the input window size on \ourmethod. To facilitate the testing of larger input windows, we conducted experiments on HotpotWikiQA-mixup-256k. The experimental results indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects three actions: less pagination when searching for starting nodes, reading more nodes at once; during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.
%---------------------------------------------------------
% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Input Window}} & \multicolumn{2}{c}{\textbf{Metrics}}\\ \cline{3-4} 
%        &  & LR-1 & LR-2 \\ \hline
    
%     \multirow{4}{*}{\textbf{HotpotWikiQA-mixup-256k}} & 4k & 30.0 & 38.0 \\
%         & 8k & \textbf{32.0} & \textbf{40.0} \\
%         & 16k & 32.0 & 38.0 \\
%         & 32k & 28.0 & 36.0 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{The impact of the input window size.}
% % \vspace{-0.5cm}
% \label{tab: input_window}
% \end{table}
%---------------------------------------------------------
\begin{table}[!t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc}
\toprule
    Method & Avg. Token Consumption & Avg. Ctx. Tokens \\\hline
    ReadAgent & 49906.68 & \multirow{2}{*}{366950.7}  \\
    \ourmethod & 54056.25 & \\\bottomrule
    \end{tabular}
}
\caption{Comparison of consumption per question between ReadAgent and \ourmethod on HotpotWikiQA-mixup-256k, where Consumption Tokens include both input tokens and output tokens. The ``Avg. Ctx. Tokens'' refers to the average tokens of the total context.}
\label{tab: consumption}
\end{table}
%--------------------------------------------------------------------------
\paragraph{The Analysis of Function Calls}
To further demonstrate the capabilities of \ourmethod, we made statistics on its function calls at each stage across two datasets.
% Table \ref{tab: action} shows the action statistics of \ourmethod across two datasets. 
We selected one dataset each for single-hop QA and multi-hop QA for analysis. From the statistical results in Table \ref{tab: action}, it can be observed that the proportion difference between the two candidate functions is insignificant during the stages of `Exploring Node Atomic Facts' and `Exploring Node Neighbors'. This outcome further indicates the effectiveness of \ourmethod in selecting initial nodes as the relatively low proportion of choosing \textit{termination} function.

For the ``Exploring Node Chunks'' stage, there is a substantial difference between the single-hop QA dataset (NarrativeQA) and the multi-hop QA dataset (MuSiQue), mainly because on the single-hop QA dataset, the proportion of \ourmethod choosing the \textit{search\_more} function is deficient, only 4.1\%, while on the multi-hop QA dataset, this proportion reaches 19.1\%. This phenomenon is related to the type of questions; for single-hop QA, \ourmethod can obtain the necessary information through a single reading of the chunk, so it seldom returns to search for more information. However, for multi-hop QA, \ourmethod often needs to be read multiple times to gather all the necessary information to answer the question.
%--------------------------------------------------------------------------
\paragraph{Consumption Analysis}
We assessed the average token consumption by ReadAgent and \ourmethod in answering a question, with the results presented in Table \ref{tab: consumption}. \ourmethod requires slightly more tokens to answer a question compared to ReadAgent. Despite a minor increase in consumption, \ourmethod achieves significantly better results than ReadAgent, favorably demonstrating the superiority of our method.

It can also be observed that the average tokens consumed by these two methods to answer a question are significantly less than the average context tokens, indicating that this approach of pre-processing the context has a notable advantage when dealing with multiple QA scenarios.
%--------------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/recall.pdf}
% \vspace{-0.6cm}
\caption{Recall of supporting facts by different methods on HotpotWikiQA-mixup.}
\label{fig: recall}
% \vspace{-0.6cm}
\end{figure}
%--------------------------------------------------------------
\begin{table}[!t]
\centering
% \scriptsize
\resizebox{0.75\columnwidth}{!}{
    \begin{tabular}{ccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Source}}  & \multicolumn{2}{c}{\textbf{Recall(\%)}} \\ \cline{2-3} 
     &  by supporting fact & by case \\ \hline
    Atomic Facts & 76.4 & 64.7 \\
    Final Notebook & 90.5 & 85.3  \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
% \caption{\ourmethod's recall of supporting facts at various stages. Define a partial\_ratio similarity greater than $0.8$ as a successful recall. We use \textit{gpt-4-1106-preview} for evaluation, with the temperature set to 0.1.}
\caption{\ourmethod's recall of supporting facts at various stages. Statistical dimensions: ``by supporting fact'' refers to individual atomic facts; ``by case'' refers to all atomic facts for a QA pair.}
\label{tab: recall}
\end{table}
%--------------------------------------------------------------
\paragraph{Recall Rate Analysis}
To better evaluate the advantage of our method in pinpointing critical information, we used LLMs to assess the recall of supporting facts for various methods on the HotpotWikiQA-mixup dataset. The specific evaluation approach is described in Appendix \ref{app: recall}.

The evaluation results shown in Figure \ref{fig: recall} demonstrate that \ourmethod far surpasses other baseline methods in terms of the recall of supporting facts, proving the superiority of our approach. Besides, we notice that as the context length increases (from $16k$ to $256k$), the recall of supporting facts for all methods declines, with ReadAgent experiencing a particularly rapid decrease, while \ourmethod shows a very slow decline. This indicates that \ourmethod has excellent scalability in handling long texts.

We calculate the recall rate of \ourmethod at various stages using the same method, and Table \ref{tab: recall} presents the experimental results. The recall rate of supporting facts during the Answer Reasoning stage is slightly higher than that of the Memory Graph, indicating that \ourmethod has the ability to supplement and extract valid information from chunks during the exploration process, indirectly showcasing its intelligence and efficiency in exploration.
% To better assess the advantages of our method in identifying key information, we utilized the supporting facts that support answering questions from the HotpotQA dataset. We analyzed \ourmethod's recall of supporting facts at various stages on the HotpotQA dataset.

% Table \ref{recall} presents the experimental results of the recall analysis for \ourmethod, where the two stages of evaluation are specifically: atomic facts extracted from the text and the final memory obtained. The evaluation was conducted using LLM (\textit{gpt-4-1106-preview}, with the specific evaluation prompt shown in Figure \ref{recall_prompt}). The statistics were compiled based on supporting facts (by supporting fact) and by individual cases (by case), where "by supporting fact" refers to whether that supporting fact was recalled, and "by case" indicates whether all supporting facts for a given case were fully recalled.

% The results indicate that under the same LLM evaluation method (with identical prompts), the final memory's recall rate for supporting facts is higher compared to the recall rate for atomic facts. Furthermore, the gap between this recall rate aligns with the assessment results of the LLM-Raters (Figure \ref{tab: main_result_2}, LR-1: 0.843; LR-2: 0.897). This demonstrates \ourmethod's capability to locate corresponding supporting facts from weakly related nodes.
%--------------------------------------------------------------




==> content/cache/exp_cache_15_29.tex <==
\section{Experiments}


\subsection{Experimental Settigns}

\paragraph{Evaluation Benchmarks} We conduct experiments on two types of long-context QA benchmarks, including multi-hop long-context QA, \ie, HotpotQA~\citep{yang-2018-emnlp-hotpotqa}, 2WikiMultihopQA~\citep{ho-2020-coling-2wikimultihopQA}, MuSiQue~\citep{Trivedi-2022-acltrans-musique}, and a single-hop long-context QA benchmark, NarrativeQA~\citep{Kocisky-2018-acltrans-narrativeqa}. Additionally, we also incorporate HotpotWikiQA-mixup from LV-Eval~\citep{Yuan2024LVEvalAB}, a multi-hop benchmark that features five levels of text length: 16k, 32k, 64k, 128k, and 256k, reaching a maximum length of 370.8k. The statistical information about these benchmarks is presented in Table~\ref{tab: datasets} and detailed information is provided in Appendix~\ref{app: datasets}.


\paragraph{Evaluation Metrics} We employ several automatic evaluation metrics, \ie $F_1$ score, Exact Match (EM) score, and an optimized $F_1$* score, as introduced by LV-Eval~\cite{Yuan2024LVEvalAB}. Specifically, $F_1$* first computes the recall of golden answer keywords and only calculates the $F_1$ score if it exceeds a certain threshold, otherwise, the score defaults to zero. Despite the cost-effectiveness of automatic metrics, their accuracy may be affected by the response format. Hence we implement LLM Raters for answer correctness evaluation using an LLM, denoted as LLM-Rating-1 (LR-1) and LLM-Rating-1 (LR-2), as demonstrated by ReadAgent~\citep{lee2024human}. Details on the evaluation metrics can be found in Appendix \ref{app: eval_details}.

\ignore{
\paragraph{Baseline Methods} We compare \ourmethod with three types of baseline methods: model-level, retrieval-level, and agent-level methods, described as follows:

\begin{itemize}[leftmargin=4mm]
\vspace{-0.08cm}
\item \textbf{Model-level Methods} utilize long-context LLM GPT-4-128k for direct full-text reading when the text content fits within the input window or segmenting the text into chunks for sequential reading.

\item \textbf{Retrieval-level Methods} utilize Okapi BM25~\citep{Robertson2009ThePR} or OpenAI API embedding model Ada-002\footnote{https://platform.openai.com/docs/guides/embeddings/\linebreak embedding-models} to retrieve the chunks most relevant to the question and employ LLM to read retrieved chunks and answer the question.

\item \textbf{Agent-level Methods} employ ReadAgent~\citep{lee2024human} for long-context QA, which employs an agent-based system for the execution of retrieval and reading processes.

\end{itemize}

The detailed description and implementation of these methods are provided in Appendix~\ref{app: baseline}.
}


\paragraph{Baseline Methods} We compare \ourmethod with three types of baseline methods: model-level, retrieval-level, and agent-level methods. \textbf{Model-level Methods} utilize long-context LLM GPT-4-128k for direct full-text reading when the text content fits within the input window or segmenting the text into chunks for sequential reading. \textbf{Retrieval-level Methods} utilize Okapi BM25~\citep{Robertson2009ThePR} or OpenAI API embedding model Ada-002\footnote{https://platform.openai.com/docs/guides/embeddings/\linebreak embedding-models} to retrieve the chunks most relevant to the question and employ LLM to read retrieved chunks and answer the question. \textbf{Agent-level Methods} employ ReadAgent~\citep{lee2024human} for long-context QA, which employs an agent-based system for the execution of retrieval and reading processes. The detailed description and implementation of these methods are provided in Appendix~\ref{app: baseline}.

\paragraph{Implementation Details}

In our experiments, we employ the GPT-4 (\texttt{gpt-4-1106-preview}) for both our method and baseline approaches, setting the temperature to 0.2. 
%GPT-4 supports 128k tokens input and can generate 4k tokens.
When deploying \ourmethod, unless otherwise specified, we configure the input window size to 4k tokens, set the maximum length of chunk to 2k tokens, initiate searches from 5 initial nodes, and impose a function call limit of 10 for each search path.

\begin{table}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llccc}
\bottomrule
                  \textbf{Task} & \textbf{Dataset}  & Avg \#Tokens & Max \#Tokens & \#Samples  \\ \hline
\multirow{4}{*}{\textbf{Multi-hop QA}} & HotpotQA  & 9.4k & 15.9k & 300  \\
                     & 2WikiMultihopQA  & 8.8k & 15.9k & 300 \\
                    & MuSiQue  & 15.5k & 16.0k & 200 \\
                    & HotpotWikiQA-mixup  & 142.4k & 370.8k & 250 \\ \hline
% \multirow{1}{*}{\textbf{Single-hop QA}} &narrativeQA & English & 29.7k & 200 
\textbf{Single-hop QA} & NarrativeQA  & 29.7k & 63.7k & 200 \\\bottomrule
\end{tabular}
}
\caption{
The statistical information of benchmarks employed in our evaluation. The token number is calculated using the GPT-4 tokenizer from the TikToken\protect\footnotemark. \#Samples denotes the total number of benchmarks.
}
\label{tab: datasets}
\end{table}
\footnotetext{https://github.com/openai/tiktoken}



%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{lcrrrr|rrrr|rrrr|rrrr}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \textbf{Input} & \multicolumn{4}{c}{\textbf{HotpotQA}} & \multicolumn{4}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{4}{c}{\textbf{MuSiQue}} &  \multicolumn{4}{c}{\textbf{NarrativeQA}}\\ \cline{3-18}
     & \textbf{Window} & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$\\ \hline
     % \multicolumn{18}{l}{BM25(top-1)} \\ \hline
    BM25 (top-1) & 4k & 57.7 & 63.0 & 33.7 & 43.8 & 36.0 & 39.0 & 25.0 & 30.4 & 33.0 & 36.5 & 19.0 & 23.9 & 29.5 & 34.5 & 4.0 & 11.3 \\
    BM25 (top-3) & 4k & 74.7 & 78.3 & 45.7 & 58.5 & 59.7 & 62.0 & 42.3 & 51.9 & 43.5 & 49.5 & 25.0 & 31.1 & 44.5 & 52.5 & 7.0 & 20.5 \\ \hline
% \multicolumn{18}{l}{OpenAI Embedding Retrieval} \\ \hline
    Ada-002 (top-1) & 4k & 63.0 & 70.7 & 40.0 & 53.2 & 57.0 & 59.3 & 41.0 & 49.4 & 34.5 & 37.0 & 20.0 & 26.6 & 37.5 & 46.5 & 5.0 & 15.5 \\
    Ada-002 (top-3) & 4k & 72.0 & 77.3 & 45.0 & 58.1 & 65.7 & 66.7 & 44.7 & 55.3 & 40.0 & 45.5 & 24.5 & 32.1 & 45.5 & 53.0 & 7.5 & 19.5 \\ \hline
    GPT-4-128k & $128k$ & \underline{83.3} & \underline{88.3} & \underline{53.0} & \underline{68.4} & 77.3 & 80.0 & \underline{58.7} & \underline{70.0} & 52.0 & 59.5 & 33.5 & 42.7 & \underline{63.5} & \underline{77.0} & \underline{11.5} & \underline{29.4}  \\
    GPT-4-128k (chunk) & $4k$ & 71.3 & 74.7 & 45.7 & 59.5 & 59.3 & 62.3 & 40.7 & 50.5 & 41.0 & 43.0 & 23.0 & 32.1 & 58.0 & 69.5 & 9.50 & 25.5  \\
    GPT-4-128k (chunk w/ notes) & $4k$ & 72.3 & 76.7 & 45.7 & 59.5 & 65.7 & 68.7 & 46.3 & 56.6 & 39.5 & 43.0 & 25.0 & 32.5 & 56.5 & 65.0 & 8.5 & 24.3  \\\hline
    ReadAgent & \redtext{$128k$} & 72.3 & 78.7 & 48.0 & 62.0 & \underline{79.0} & \underline{81.0} & 52.7 & 63.7 & \underline{54.5} & \underline{61.0} & \underline{35.0} & \underline{45.1} & 63.0 & 75.5 & 5.0 & 18.9 \\ 
    \ourmethod & $4k$ &\textbf{84.3} & \textbf{89.7} & \textbf{55.0} & \textbf{70.0} & \textbf{83.7} & \textbf{87.0} & \textbf{59.3} & \textbf{70.1} & \textbf{59.0} & \textbf{63.5} & \textbf{38.0} & \textbf{47.4} & \textbf{65.0} & \textbf{80.0} & \textbf{15.5} & \textbf{29.8} \\
    \hline
    Golden & $4k$ & 92.3 & 93.7 & 57.0 & 73.8 & 88.3 & 89.7 & 63.0 & 73.4 & 66.0 & 69.0 & 45.0 & 56.0 & - & - & - & - \\  \hline
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) comparison of different baselines on datasets from LongBench. The best performance and the second-best performance are denoted in bold and underlined fonts, respectively. Golden denotes the settings that we add question and its supporting facts to LLM directly.}
% \vspace{-0.5cm}
\label{tab: main_result_1}
\end{table*}
%---------------------------------------------------------
 % \multirow{4}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}}} \\
 % & & & & & & & & & & & & & & & & \\
 % & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lcrrr|rrr|rrr|rrr|rrr}
\hline
 \multirow{3}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}} \\\cline{3-17}
 & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
& & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$*\\ \hline
% \multicolumn{17}{l}{BM25 Retrieval} \\ \hline
    BM25 (top-1) & $4k$ & 10.0 & 16.0 & 12.0 & 16.0 & 18.0 & 11.9 & 6.0 & 8.0 & 8.5 & 10.0 & 8.0 & 7.0 & 14.0 & 20.0 & 5.9 \\
    BM25 (top-3) & $4k$ & 16.0 & 22.0 & 13.9 & 18.0 & 28.0 & 13.3 & 16.0 & 18.0 & 11.8 & 12.0 & 16.0 & 11.8 & 12.0 & 22.0 & 9.3 \\ \hline
% \multicolumn{17}{l}{OpenAI Embedding Retrieval} \\ \hline
    Ada-002 (top-1) & $4k$ & 10.0 & 12.0 & 14.5 & 14.0 & 18.0 & 11.3 & 10.0 & 12.0 & 12.5 & 12.0 & 14.0 & 9.4 & 8.0 & 8.0 & 7.0 \\
    Ada-002 (top-3) & $4k$ & 24.0 & 28.0 & 21.3 & 20.0 & 30.0 & 19.8 & 14.0 & 20.0 & 12.9 & 16.0 & 20.0 & 12.0 & 14.0 & 18.0 & 10.8 \\  \hline
    GPT-4-128k & $128k$ & {\underline {38.0}} & {\underline {38.0}} & {\underline {35.7}} & {\underline {26.0}} & {\underline {30.0}} & {\underline {26.0}} & 22.0 & 24.0 & 20.6 & 16.0 & 16.0 & 14.6 & 14.0 & 16.0 & 10.3 \\
    GPT-4-128k (chunk) & $4k$ & 18.0 & 22.0 & 24.6 & 16.0 & 20.0 & 17.7 & 20.0 & 24.0 & 17.0 & 20.0 & 24.0 & 14.7 & {\underline {28.0}} & {\underline {30.0}} & 10.7 \\
    GPT-4-128k (chunk w/ notes) & $4k$ & 22.0 & 32.0 & 24.2 & 26.0 & 30.0 & 21.3 & {\underline {28.0}} & {\underline {32.0}} & {\underline {22.0}} & {\underline {24.0}} & {\underline {26.0}} & {\underline {17.4}} & 26.0 & 26.0 & {\underline {14.8}} \\
    ReadAgent & \redtext{$128k$} & 24.0 & 26.0 & 29.2 & 20.0 & 22.0 & 16.9 & 24.0 & 30.0 & 15.3 & 14.0 & 18.0 & 13.6 & 20.0 & 22.0 & 10.4 \\
    \ourmethod & $4k$ & \textbf{42.0} & \textbf{42.0} & \textbf{38.2} & \textbf{32.0} & \textbf{38.0} & \textbf{36.4} & \textbf{30.0} & \textbf{36.0} & \textbf{32.9} & \textbf{28.0} & \textbf{34.0} & \textbf{30.6} & \textbf{30.0} & \textbf{38.0} & \textbf{33.0} \\
\hline
\end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) of different baselines on datasets from LV-Eval, where $F_1$* donates LV-Eval's optimized $F_1$. The best performance and the second-best performance are denoted in bold and underlined fonts, respectively. We truncate to keep the longest possible initial fragment while preserving paragraph structure, in contexts that exceed the input window (128k and 256k) for GPT-4-128k.}
% \vspace{-0.5cm}
\label{tab: main_result_2}
\end{table*}
%---------------------------------------------------------
\subsection{Main Results}

In this part, we conduct a series of experiments on multi-hop and single-hop long-context QA tasks. 


\paragraph{Evaluation on Single and Multi-hop Long-context Tasks} The results of three types of methods on three multi-hop long-context QA and one single-hop long-context QA are shown in Tabel~\ref{tab: main_result_1}. Based on the results, we have the following findings:

Firstly, we observe that sparse retrieval BM25 and dense retrieval Ada-002 exhibit the worst performance in comparison to model-level and agent-level approaches. A possible reason is that text retrieval fails to recall all documents that contain the supporting facts for answering the input question. Although increasing the quantity of recalled documents could improve text retrieval's performance, the constrained context window LLM restricts the number of documents that can be read, thereby limiting the effectiveness of these retrieval-level methods. 

Secondly, we see that employing GPT-4-128k for direct reading of long texts significantly outperforms retrieval-level methods, and even outperforms ReadAgent on three long-context benchmarks. This is because of the superior performance of GPT-4-128k in processing long texts and executing multi-hop reasoning. Additionally, the lengths of these four benchmarks are significantly shorter than 128k context window, thereby mitigating the impact of ``lost in the middle'' on the model's performance. Moreover, we also observe that GPT-4, despite having a constrained 4k context window, can process input contexts that significantly exceed its context window limitations through sequential reading and still outperform retrieval-based methods. Furthermore, incorporating a memory module into sequential reading with LLM can significantly improve the performance of sequential reading on multi-hop benchmarks. The reason may be that carrying memory with history information can facilitate LLM in aggregating previous supporting facts. Conversely, for the single-hop benchmark, NarrativeQA, integrating memory results in performance degradation. The reason may be that previous memory introduces noise to LLM and affects its responses. 

Thirdly, we can also see that the previous agent-level method ReadAgent demonstrates impressive performance in these four long-context benchmarks. This is because the agent-level method introduces diverse actions, memory, and reflection in reading strategies, which fully harnesses LLM's reasoning ability. However, even the effectiveness, ReadAgent slightly underperforms GPT-4-128k full-text reading. We attribute this to the ReadAgent's strategy, which relies on summarizing each page, leveraging past memories, and analyzing the input question to select pages for gathering supporting information. This approach may restrict the agent's ability to identify specific details and capture long-range dependencies in long context, consequently affecting its overall performance.


Finally, by comparing our approach with all baselines, it is obvious that our approach performs consistently better them on four long-context benchmarks and demonstrates more superior performance in multi-hop QA than sing-hop QA. In our approach, we transform long context into key elements and atomic facts，which are subsequently organized into a graph. Benefiting from the graph's ability to capture the relationships between detailed information, our method can identifies crucial information and search the supporting facts for the input question efficiently. This strategy significantly boosts the agent's capability in multi-hop reasoning and capturing long-range dependencies of key information in long context. And we observe that the performance of our method closely matches that achieved by directly supplying supporting facts to the LLM (\ie Golden in Table~\ref{tab: main_result_1}). This is because our method not only incorporates pre-planning, reflection, and various actions but also the usage of a graph containing key information, facilitating the agent to search for the correct supporting facts. Additionally, it is noteworthy that our method, employing merely a 4k context window, outperforms ReadAgent's 128k context window setup. It further indicates that our approach can more efficiently unlock the capabilities of constrained context window LLMs in processing long context.


%正如之前的实验，我们发现我们的方法在多跳和单跳长文本任务上均取得了成功。这里我们we would like to study the effectiveness of our approach on the更长的长文本benchmark上的表现。如表3结果所示，相比于baseline中其他方法，我们的方法在16k to 256k的所有长度任务上表现都会更好。这进一表明了我们的方法在面对超长文本时，仍然可以通过构建图的方式，使得短窗口的大语言模型处理超长文本。首先作为对比，我们可以看到随着窗口长度增加，gpt-4-128k full text reading的性能逐渐下降，而采用了我们的方法后，在16k长度时，LR-1性能增益仅有21%，而当长度增加到128k时，使用我们方法，性能增益达到了56%。这是因为随着长度增加，gpt-4受到lost in the middle影响会逐渐加重。而我们的方法并不会受到文本长度变长时表现地更加鲁棒。第二，我们看到readagent在长文本上表现明显差于我们的方法，这可能是因为，readagent在处理超长文本时需要同时决策阅读哪些页，由于缺乏每一页内容细粒度信息，这使得readagent难以收集更多关于问题的证据。这进一步表明了我们方法通过构建图并在图上探索的方法可以有效的完成超长文本的问题，并展现了可以扩展到更长文本上的可能性。

\paragraph{Evaluation on Ultra-long Context Tasks} As shown in previous experiments, it demonstrates the  utility of employing a limited context window LLM for long-context QA with our \ourmethod. Here, we would like to study the effectiveness of our approach on the longer multi-hop long-context QA tasks. As shown in Table~\ref{tab: main_result_2}, compared with all baselines, our \ourmethod not only consistently outperforms these methods across text lengths ranging from 16k to 256k tokens but also exhibits robustness with the expansion of context length. It further indicates that our method remains effective in handling ultra-long texts by constructing graphs and graph exploration, thereby allowing constrained context window LLMs to process extensive texts efficiently. As a comparison, we can see that with the increase in the length of the input context, the performance of GPT-4-128k full-text reading  degrades gradually. However, employing our method, at context length of 16k, the LR-1 performance gain is merely 10.53\%, whereas by extending the context length to 128k, our method achieves a performance gain of 75.00\%. This can be attributed to the fact that as the context length increases, the impact of the ``lost in the middle'' effect on GPT-4-128k becomes progressively more severe. Secondly, we observe that ReadAgent significantly underperforms our method in handling ultra-long contexts. This is because the lack of detailed information about the content of each page can make page selection very difficult for ReadAgent, especially when dealing with extremely long contexts. This further demonstrates that our method, by constructing and exploring graphs with fine-grained information, can effectively address the challenges of processing ultra-long context with limited context window LLMs.


\begin{table}[!t]
\centering
% \scriptsize
\resizebox{\columnwidth}{!}{
    \begin{tabular}{clccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Results(\%)}}\\ \cline{3-5} 
     & & LR-1 & LR-2 & $F_1$ \\ \hline
    \multirow{3}{*}{\textbf{HotpotQA}} & \ourmethod & \textbf{84.3} & \textbf{89.7} & \textbf{70.0} \\
        & \quad w/o Rational Plan & 81.7 & 87.7 & 63.8 \\
        & \quad w/o Node Selection & 66.0 & 71.7 & 54.1 \\\hline
    \multirow{3}{*}{\textbf{2WikiMultihopQA}}& \ourmethod & \textbf{83.7} & \textbf{87.0} & \textbf{70.1} \\
        & \quad w/o Rational Plan & 81.3 & 86.0 & 65.4 \\
        & \quad w/o Node Selection & 65.3 & 68.7 & 49.7 \\\hline
    \multirow{3}{*}{\textbf{MuSiQue}} & \ourmethod & \textbf{59.0} & \textbf{63.5} & \textbf{47.4} \\
    & \quad w/o Rational Plan & 56.0 & 61.0 & 42.4 \\
    & \quad w/o Node Selection & 35.0 & 38.5 & 25.2 \\\hline
    \multirow{3}{*}{\textbf{NarrativeQA}} & \ourmethod & \textbf{65.0} & \textbf{80.0} & \textbf{29.8}  \\
        & \quad w/o Rational Plan & 63.0 & 78.5 & 26.6 \\
        & \quad w/o Node Selection & 53.0 & 65.5 & 24.0 \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{The results of our ablation study. ``w/o Rational Plan'' refers to removing the rational plan in agent initialization stage, and ``w/o Node Selection'' denotes applying the random selection of initial nodes and neighbor nodes in graph exploration.}
% \vspace{-0.5cm}
\label{tab: ablation}
\end{table}
%---------------------------------------------------------
\subsection{Ablation study}
We conduct ablation experiments on various benchmarks to investigate the contribution of different components in our approach. 

\paragraph{The Effect of Rational Plan}


In our graph exploration stage, we introduce rational plan to assist agent analysis input complex question step by step then guide agent to explore on graph. In this part, to verify the effectiveness, we remove rational plan in agent initialization and conduct experiments on four long-context QA benchmarks. As shown in Tabel~\ref{tab: ablation}, we can see that our approach is better than variants without rational plan (denoted as ``w/o Rational Plan'' in Tabel~\ref{tab: ablation}). It indicates that rational plan is effective to guide the agent to node selection and explore on graph.

\ignore{
To evaluate the Rational Plan's effectiveness, we remove pre-planning stage in our method and conduct experiments on four long-context benchmarks. The results are shown in Table~\ref{tab: ablation}. We can observe that removing the rational path in \ourmethod leads to performance degradation. It indicates that the improvement of our methods is due to


thus confirming the rational plan's beneficial impact on \ourmethod. We can infer that the pre-planning stage enables \ourmethod to deal with various complex questions effectively.
}

\paragraph{The Effect of Graph-Based Agent}
On the other hand, to prove that the model chooses which nodes to visit based on reasoning about the information needed, we conduct experiments under settings with randomly selecting initial nodes. As shown in Table \ref{tab: ablation}, Setting to random selection results in the significant performance degradation of our approach, with results across all datasets declining by an average of 18\%. This indicates that \ourmethod indeed exhibits intelligence in its exploration process on the graph, selecting nodes through the reasoning ability of the accumulated information rather than engaging in arbitrary exploration dependent on the chance to collect supporting facts.


%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/figure3.pdf}
% \vspace{-0.6cm}
\caption{Performance of \ourmethod with different initial node numbers on 2WikiMultihopQA and NarrativeQA. Results show the robustness of \ourmethod towards different initial node numbers.}
\label{fig: nodes}
% \vspace{-0.6cm}
\end{figure}
%---------------------------------------------------------
\subsection{Further Analysis}
\paragraph{Impact of the Number of Initial Nodes}
To assess the effect of the number of initial nodes on \ourmethod's performance, we conduct experiments setting different numbers of initial nodes on both multi-hop and single-hop QA datasets, and the results are shown in Figure \ref{fig: nodes}. Firstly, we can find the performance of \ourmethod changes slightly with the number of initial nodes, showing strong robustness to it. Secondly, within a certain range, an increase in the number of nodes leads to a slight improvement in model performance and the performance is relatively optimal when the initial number of nodes is set to 5, hence we choose this as our default initial node setting. However, surpassing a certain threshold, \ourmethod's performance tends to decline. Notably, this decrement is more apparent in single-hop scenarios. We can consider that this is because more noise interferes with the model by an excessive number of initial nodes.

%For multi-hop QA, having a sufficient number of starting nodes is crucial. For example, in questions involving comparisons, the objects to be compared are often difficult to associate on the memory graph. In such cases, selecting a starting node for each object becomes particularly important for searching for enough information to answer the question adequately.


% To investigate the impact of the number of initial nodes on the outcomes, we conducted experiments using datasets from both multi-hop QA and single-hop QA. The experimental results shown in Table \ref{tab: starting_nodes}  reveal that when the number of initial nodes is too low, the performance of \ourmethod improves with an increase in the number of initial nodes. However, the final QA performance slightly declines when the number of initial nodes is excessive. We believe this is due to the overabundance of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of initial nodes is more pronounced for single-hop QA.

% Table \ref{tab: starting_nodes} showcases the impact of different numbers of starting nodes, which are the number of search paths, on the final outcome. We selected one dataset each from multi-hop QA and single-hop QA datasets for experimentation to explore their respective effects on multi-hop QA and single-hop QA. The experimental results reveal that when the number of starting nodes is too low, the performance of \ourmethod improves with an increase in the number of starting nodes. However, the final QA performance slightly declines when the number of starting nodes is excessive. We believe this is due to the overabundance and disorganization of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of starting nodes is more pronounced for single-hop QA.
%---------------------------------------------------------
% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \hline
    
%     \textbf{Dataset} & \textbf{Avg Action Num(per trace)} & \textbf{Stage} & \textbf{Total Ratio} & \textbf{Selected Action} & \textbf{Selection Ratio}\\ \hline
%      % \multirow{7}{*}{\textbf{MuSiQue}} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{3}{*}{read_chunk} & \multirow{3}{*}{0.312(2185/7002)}
%      \multirow{7}{*}{MuSiQue} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.312(2185/7002)} & \textit{search\_more}s & 0.191(417/2185)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.266(582/2185) \\ 
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.257(561/2185) \\
%     &  &  &  & \textit{stop} & 0.286(625/2185) \\  \cline{3-6}
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.400(2800/7002)} & \textit{read\_chunk} & 0.413(1156/2800) \\ 
%     &  &  &  & \textit{stop} & 0.587(1644/2800) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.288(2017/7002)} & \textit{read\_neighbor\_node} & 0.401(809/2017)  \\ 
%     &  &  &  & stop & 0.599(1208/2017) \\ \hline
% \multirow{7}{*}{NarrativeQA} & \multirow{7}{*}{3.8475(7695/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.543(4176/7695)} & \textit{search\_more} & 0.041(171/4176)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.353(1475/4176) \\
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.326(1360/4176) \\
%     &  &  &  & \textit{stop} & 0.280(1170/4176) \\ 
%     \cline{3-6} 
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.325(2502/7695)} & \textit{read\_chunk} & 0.645(1615/2502) \\  
%     &  &  &  & \textit{stop} & 0.355(887/2502) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.132(1017/7695)} & \textit{read\_neighbor\_node} & 0.514(523/1017)  \\
%     &  &  &  & \textit{stop} & 0.486(494/1017)  \\
%     \hline
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Action statistics of \ourmethod on two datasets.}
% % \vspace{-0.5cm}
% \label{tab: action}
% \end{table*}
\begin{table*}[!t]
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{cccccr}
    \toprule
    \textbf{Dataset} & \textbf{\#Avg. Function Call} & \textbf{Stage} & \textbf{Stage Ratio(\%)} & \textbf{Function} & \textbf{Call Ratio(\%)}\\ \hline

    \multirow{7}{*}{HotpotQA} & \multirow{7}{*}{3.0} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{42.0} & \textit{read\_chunk} & 46.5 \\ 
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 53.5 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks}     & \multirow{4}{*}{31.9} & \textit{search\_more} & 12.1  \\
    &  &  &  & \textit{read\_previous\_chunk} & 21.1 \\ 
    &  &  &  & \textit{read\_subsequent\_chunk} & 22.9 \\
    &  &  &  & \textit{termination} & 43.9 \\  \cline{3-6}
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{26.1} & \textit{read\_neighbor\_node} & 35.5 \\
    &  &  &  & \textit{termination} & 65.5\\ \hline

    \multirow{7}{*}{2WikiMultihopQA} & \multirow{7}{*}{3.2} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{40.4} & \textit{read\_chunk} & 48.6 \\  
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 51.4 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks} & \multirow{4}{*}{34.5} & \textit{search\_more} & 14.5 \\
    &  &  &  & \textit{read\_previous\_chunk} & 25.1 \\
    &  &  &  & \textit{read\_subsequent\_chunk} & 23.3 \\
    &  &  &  & \textit{termination} & 37.1 \\ 
    \cline{3-6} 
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{25.1} & \textit{read\_neighbor\_node} & 37.3  \\
    &  &  &  & \textit{termination} & 62.7  \\\hline
 
     \multirow{7}{*}{MuSiQue} & \multirow{7}{*}{3.5} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{40.0} & \textit{read\_chunk} & 41.3 \\ 
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 58.7 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks}     & \multirow{4}{*}{31.2} & \textit{search\_more} & 19.1  \\
    &  &  &  & \textit{read\_previous\_chunk} & 26.6 \\ 
    &  &  &  & \textit{read\_subsequent\_chunk} & 25.7 \\
    &  &  &  & \textit{termination} & 28.6 \\  \cline{3-6}
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{28.8} & \textit{read\_neighbor\_node} & 40.1 \\
    &  &  &  & \textit{termination} & 59.9\\ \hline
\multirow{7}{*}{NarrativeQA} & \multirow{7}{*}{3.9} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{32.5} & \textit{read\_chunk} & 64.5 \\  
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 35.5 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks} & \multirow{4}{*}{54.3} & \textit{search\_more} & 4.1 \\
    &  &  &  & \textit{read\_previous\_chunk} & 35.3 \\
    &  &  &  & \textit{read\_subsequent\_chunk} & 32.6 \\
    &  &  &  & \textit{termination} & 28.0 \\ 
    \cline{3-6} 
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{13.2} & \textit{read\_neighbor\_node} & 51.4  \\
    &  &  &  & \textit{termination} & 48.6  \\
    
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{Statistics of function calls on MuSiQue and NarrativeQA.}
% \vspace{-0.5cm}
\label{tab: action}
\end{table*}
%---------------------------------------------------------
% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Avg Ctx. Tokens}} & \multirow{2}{*}{\textbf{Chunk Limit}} & \multirow{2}{*}{\textbf{Token Type}} & \multicolumn{2}{c}{\textbf{Stage}} \\ \cline{5-6} 
%        & & &  & avg atomic facts and key elements tokens & avg agent tokens \\\hline
%     \multirow{8}{*}{\textbf{HotpotWikiQA-mixup-256k}} & \multirow{8}{*}{366950.70} & \multirow{2}{*}{1k} & input token & 585770.34 & 90624.49   \\
%         & & & output token & 270179.60 &  13558.30 \\\cline{4-6}
        
%     & & \multirow{2}{*}{2k} & input token & 465931.14 & 69821.40 \\
%         & & & output token & 156201.42 & 11057.36  \\\cline{4-6}

%         & & \multirow{2}{*}{4k} & input token & 417449.46 & 93083.31   \\
%         & & & output token & 142652.42 & 10939.20  \\\cline{4-6}

%         & & \multirow{2}{*}{6k} & input token & 400457.94 & 76402.95  \\
%         & & & output token & 131023.17 & 9625.54 \\
       
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Consumption statistics of \ourmethod on two datasets. The input window is set to 4k, with 7 starting nodes, and a maximum of 10 actions. The upper limit of text fragments is 2k.}
% % \vspace{-0.5cm}
% \label{tab: cost}
% \end{table*}
%--------------------------------------------------------------
%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=0.8\linewidth]{source/figure4.pdf}
% \vspace{-0.2cm}
\caption{The impact of chunk size $L$ of \ourmethod on the 256k length level of HotpotWikiQA-mixup.}
\label{fig: chunk_size_exp}
% \vspace{-0.2cm}
\end{figure}
%---------------------------------------------------------
\paragraph{Impact of the Chunk Size}

To explore the impact of the chunk size $L$ on the performance of \ourmethod, we set up multiple sets of comparative experiments with different chunk sizes. As shown in Figure \ref{fig: chunk_size_exp}, the results show that the best performance was achieved when $L=2k$. Initially, We find that when $L$ exceeds a certain threshold, the bigger the chunk size, the more obvious the performance decline trend. We infer that this corresponds to the model performance degradation on longer texts mentioned earlier, where the model is prone to overlooking essential details. Moreover, when $L$ is too small, more semantic truncation occurs, hampering the model's comprehension of the current context and 
further affecting the accuracy of extracting atomic facts. So, we finally choose $L=2k$ as our default chunk size setting.

%When $L$ is smaller, it is evident that more resources are consumed during the construction phase of the memory graph. Thus, to balance performance and consumption, a larger and more effective $L$ should be selected as the hyperparameter setting as much as possible.

% To balance consumption and performance, we think $L=2k$ is a good setting.
% To investigate the impact of input window size on \ourmethod, we conducted experiments on HotpotWikiQA-mixup-256k. We used different input window sizes, and the results in Figure \ref{fig: chunk} indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects one action: during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.

% Table \ref{tab: input_window} demonstrates the impact of the input window size on \ourmethod. To facilitate the testing of larger input windows, we conducted experiments on HotpotWikiQA-mixup-256k. The experimental results indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects three actions: less pagination when searching for starting nodes, reading more nodes at once; during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.
%---------------------------------------------------------
% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Input Window}} & \multicolumn{2}{c}{\textbf{Metrics}}\\ \cline{3-4} 
%        &  & LR-1 & LR-2 \\ \hline
    
%     \multirow{4}{*}{\textbf{HotpotWikiQA-mixup-256k}} & 4k & 30.0 & 38.0 \\
%         & 8k & \textbf{32.0} & \textbf{40.0} \\
%         & 16k & 32.0 & 38.0 \\
%         & 32k & 28.0 & 36.0 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{The impact of the input window size.}
% % \vspace{-0.5cm}
% \label{tab: input_window}
% \end{table}
%---------------------------------------------------------
\begin{table}[!t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc}
\toprule
    Method & Avg. Ctx. \#Tokens & Avg. Consumption \#Tokens  \\\hline
    ReadAgent & 358.3k & 48.7k  \\
    \ourmethod & 358.3k & 52.8k \\\bottomrule
    \end{tabular}
}
\caption{Comparison of token consumption per question between ReadAgent and \ourmethod during the agent phase on HotpotWikiQA-mixup-256k, where ``Avg. Consumption \#Tokens'' comprise both input tokens and output tokens. The ``Avg. Ctx. \#Tokens'' refers to the average number of context tokens of the original dataset.}
\label{tab: consumption}
\end{table}
%--------------------------------------------------------------------------
\paragraph{The Analysis of Function Calls}
%这块是证明我们设计的动作的合理性和有用性，同时资源消耗较少，不会跳来跳去

To verify the rationality and utility of agent actions under various circumstances of \ourmethod, we made statistics on its function calls at each stage across two datasets. 
From the statistical results in Table \ref{tab: action}, it can be observed that each piece of data will perform an average of 3 to 4 actions, corresponding to the average number of function calls in the table. This indicates the effectiveness of the graph we constructed, with \ourmethod being able to swiftly locate key information while minimizing resource usage. 
Furthermore, each action has a certain probability of being chosen, justifying the rationality of the action set. Among them, the most commonly used action on multi-hop QA tasks is to read neighbor nodes, and the most common action on single-hop QA tasks is to read chunks. This difference is caused by the fact that multi-hop questions need to gather information contained by multiple nodes to answer questions, while single-hop data sets often require only one atomic fact.
%--------------------------------------------------------------------------
\paragraph{Consumption Analysis}
% 不能让人觉得我们是依靠更多的资源消耗取得的更好的效果
% 
To justify the inference cost of our approach, we evaluated the average token consumption of ReadAgent and \ourmethod when answering questions, with the results presented in Table \ref{tab: consumption}. The results indicate that \ourmethod's token usage is only 1.08 times greater than that of ReadAgent, yet it achieves more than 2 times performance improvement, favorably demonstrating the superiority of our method.
%说明下前提，可以看到在第一轮预处理好文章后后面轮次的消耗都显著减少，并且远少于原始的token数量，但是这里没有数字
It can also be observed that after the documents are preprocessed in the first round, the consumption in subsequent rounds is significantly reduced and is far less than the context tokens of the origin dataset. This has strong implementation value in multi-round QA scenarios.
%--------------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/recall.pdf}
% \vspace{-0.6cm}
\caption{Recall of supporting facts by different methods on HotpotWikiQA-mixup.}
\label{fig: recall}
% \vspace{-0.6cm}
\end{figure}
%--------------------------------------------------------------
\begin{table}[!t]
\centering
% \scriptsize
\resizebox{0.75\columnwidth}{!}{
    \begin{tabular}{ccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Source}}  & \multicolumn{2}{c}{\textbf{Recall(\%)}} \\ \cline{2-3} 
     &  by supporting fact & by case \\ \hline
    Atomic Facts & 76.4 & 64.7 \\
    Final Notebook & 90.5 & 85.3  \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
% \caption{\ourmethod's recall of supporting facts at various stages. Define a partial\_ratio similarity greater than $0.8$ as a successful recall. We use \textit{gpt-4-1106-preview} for evaluation, with the temperature set to 0.1.}
\caption{\ourmethod's recall of supporting facts at various stages. Statistical dimensions: ``by supporting fact'' refers to individual atomic facts; ``by case'' refers to all atomic facts for a QA pair.}
\label{tab: recall}
\end{table}
%--------------------------------------------------------------
\paragraph{Recall Rate Analysis}
To better evaluate the advantage of our method in pinpointing critical information, we used LLMs to assess the recall of supporting facts for various methods on the HotpotWikiQA-mixup dataset. The specific evaluation approach is described in Appendix \ref{app: recall}.

The evaluation results shown in Figure \ref{fig: recall} demonstrate that \ourmethod far surpasses other baseline methods in terms of the recall of supporting facts, proving the superiority of our approach. Besides, we notice that as the context length increases (from $16k$ to $256k$), the recall of supporting facts for all methods declines, with ReadAgent experiencing a particularly rapid decrease, while \ourmethod shows a very slow decline. This indicates that \ourmethod has excellent scalability in handling long texts.

We calculate the recall rate of \ourmethod at various stages using the same method, and Table \ref{tab: recall} presents the experimental results. The recall rate of supporting facts during the Answer Reasoning stage is slightly higher than that of the Memory Graph, indicating that \ourmethod has the ability to supplement and extract valid information from chunks during the exploration process, indirectly showcasing its intelligence and efficiency in exploration.
% To better assess the advantages of our method in identifying key information, we utilized the supporting facts that support answering questions from the HotpotQA dataset. We analyzed \ourmethod's recall of supporting facts at various stages on the HotpotQA dataset.

% Table \ref{recall} presents the experimental results of the recall analysis for \ourmethod, where the two stages of evaluation are specifically: atomic facts extracted from the text and the final memory obtained. The evaluation was conducted using LLM (\textit{gpt-4-1106-preview}, with the specific evaluation prompt shown in Figure \ref{recall_prompt}). The statistics were compiled based on supporting facts (by supporting fact) and by individual cases (by case), where "by supporting fact" refers to whether that supporting fact was recalled, and "by case" indicates whether all supporting facts for a given case were fully recalled.

% The results indicate that under the same LLM evaluation method (with identical prompts), the final memory's recall rate for supporting facts is higher compared to the recall rate for atomic facts. Furthermore, the gap between this recall rate aligns with the assessment results of the LLM-Raters (Figure \ref{tab: main_result_2}, LR-1: 0.843; LR-2: 0.897). This demonstrates \ourmethod's capability to locate corresponding supporting facts from weakly related nodes.
%--------------------------------------------------------------




==> content/cache/intro_cache.tex <==
%-----表述需要注意的：短文本llms和长文本llms表述

\section{Introduction}
Large language models~(LLMs) have made great progress on natural language understanding and generation~\citep{Zhao-2023-arxiv-survey}. However, transformer-based LLMs still struggle in handling long contexts due to the limitation of context window and memory usage. Thus concerns about improving the long-context capabilities of LLMs have drawn significant attention from the research community~\citep{}.


\ignore{To improve the capability of LLMs in processing long context, two primary approaches have been adopted: long-context LLMs finetuned with extrapolated or interpolated positional embeddings~\cite{chen2023extending} and employing agent to process extensive contexts with the constrained context window LLM~\cite{wu2020memformer, lee2024human}. These methods are quite effective, but they still have certain drawbacks. For approaches employing positional interpolation, they typically rely on training with texts of the target length~\citep{}, which results in the challenge of constructing training datasets and incurs high training costs. Furthermore, long-context LLMs optimized with positional interpolation are prone to overlooking crucial details within extended contexts, potentially leading to information loss in the midst~\cite{liu2024lost}. For approaches that employ agents, their mechanisms for constructing information—such as the usage of tiled pagination~\citep{lee2024human} or tree structures~\citep{chen2023walking}—tend to omit key details from the text and lack long-range dependencies (which are highly effective in resolving multi-hop QA challenges), consequently leading to limiting the potential effectiveness of these approaches.}



To improve the capability of LLMs in processing long context, researchers have primarily implemented four strategies: finetuning with modified positional embeddings~\cite{chen2023extending}, training directly on long-context data, applying transformer variants with modified attention mechanisms~\citep{} and employing agent to process long contexts with the limited context window LLM~\cite{wu2020memformer, lee2024human}. Despite the effectiveness, there are several shortcomings in these four methods. For the first three methods, they typically rely on training with texts of the target length~\citep{}, which results in the challenge of constructing training datasets and incurs high training costs. Furthermore, long-context LLMs optimized with these three methods tend to overlook crucial details in long contexts, \aka lost in the middle~\cite{liu2024lost}. For approaches that employ agents to handle long context input, typically, they transform the input text into paginated pages~\citep{lee2024human} or a tree~\citep{chen2023walking}, which fail to support the agents in capturing multi-hop and long-range dependencies, thus limiting the effectiveness of these methods.

% Despite the effectiveness of these long-context LLMs, there are three major shortcomings in these methods. Firstly, these methods often rely on training on texts with target length, leading to challenges in constructing training datasets and incurring high training costs. Secondly, long-context LLMs optimized with positional interpolation may overlook crucial details in long contexts, \ie lost in the middle~\cite{liu2024lost}. Lastly, tasks that exceed the window limitations of LLMs will persist, presenting ongoing challenges.

% To overcome the challenges posed by long-context LLMs, some works have proposed using agents to handle long context with limited context window LLMs. Typically, given a long text input, these studies firstly split original text into multiple segments, subsequently analyze the relationships among these segments, and employing agents to look up segments interactively with summaries of these segments. These methods empower LLMs to process texts that significantly exceed their inherent context window limits, even handling of texts with infinite length. However, current studies that organize documents into pages~\citep{} and trees~\citep{} has not succeeded in establishing long-range dependencies, thus limiting the potential effectiveness of these methods.


% To address these issues, in this paper, we propose a method that extracts critical \textbf{Info}rmation from long texts and organizes it into a \textbf{Graph}-based structure, subsequently employing an agent for interactive reading input long text and follow user instructions, namely \textbf{Info-Graph}. Specifically, as illustrated in Figure~\ref{}, our method comprises three stages. Firstly, we divide the long text into multiple segments, followed by extracting factual claims from these segments. Secondly, we construct a graph wherein claims as nodes linked by entities to represent the potential relationships among segments. Through this approach, we achieve modeling the long-range dependencies within the long content. Lastly, the Info-Graph Agent employs pre-planned strategies to conduct a depth-first search from multiple initial claims within the graph. Based on user input, it interactively reads, generates memory, and concludes once the agent deems the memory sufficient to fulfill the given instructions.

% In the real world, the cognitive process humans use for long-text reading comprehension is significantly more complex than the aforementioned methods. Typically, human reading of lengthy texts involves two primary steps: (1) reading through the entire text, (2) organizing the content based on key clues. When addressing long-text question answering, humans usually follow four distinct parts: (1) planning for the information needed to answer the question, (2) recalling parts of the text relevant to the required information, (3) conducting a detailed reading of these relevant sections to gather information, (4) summarizing the acquired information to determine whether it's sufficient to answer the question or if further information is needed.


\ignore{We draw inspiration from the cognitive processes that humans employ for reading comprehension of long texts in the real world. Typically, when humans tackle long-text QA problems, they involve two main stages, which are further broken down into steps: (1) reading the question and planning the information needed to answer it; (2) identifying several key terms based on the question; (3) searching the long text for content related to the key terms; and (4) integrating the gathered information to formulate a response. Drawing on these insights, we propose \textbf{\ourmethod}, a method that organizes information from long text into a graph, and employ an agent to plan the problem-solving process based on the input question to search and summarize information within the graph as needed. Specifically, we segment long texts and extract key elements and atomic facts from them, constructing a graph with these key elements as nodes and the atomic facts as the content of the nodes. These nodes are connected based on their co-occurrence within the atomic facts, effectively preserving essential information and modeling the long-range dependencies present in the text.
% Specifically, we segment the long text and extract key elements and atomic facts from them, constructing a graph with these claims as nodes interconnected by entities to depict inter-segment relationships, effectively modeling long-range dependencies within the text. 
The \ourmethod, guided by pre-planned strategies, undertakes a depth-first search from the selected initial nodes. It dynamically reads, accumulates memories, and concludes, responding interactively to user input until it gathers enough information to meet the given instructions.}


We draw inspiration from the cognitive processes that humans employ for reading comprehension of long texts in the real world. When tackling long-text QA problems, humans typically divide the process into four-stage process:(1) understanding the question and reasoning the key information to answer it; (2) identifying several key terms based on the question; (3) searching the content in long text related to the selected key terms; and (4) integrating the gathered information to generate the response of the question. Drawing on these insights, we propose \textbf{\ourmethod}, a novel approach that organizes information from long text into a graph, and employ an agent to travel on the graph based on the input question to search and summarize information within the graph as needed. Specifically, we first segment long texts into chunks, followed by extracting key elements and atomic facts from them. Then we construct a graph with these key elements as nodes and incorporating atomic facts and original chunks as their content to model the global information of input long text. Lastly, our \ourmethod performs a depth-first search from the selected initial nodes. It dynamically reads, accumulates memories, and concludes, responding interactively to user input until it gathers enough information to fulfill the given question.


To


In summary, our main contributions are as follows:
\begin{itemize}[leftmargin=4mm]
\vspace{-0.08cm}
\item We propose \ourmethod, a novel agent system that utilizes a memory mechanism and graph-driven traversal to handle long-context tasks with limited context window LLMs.
\vspace{-0.08cm}
% \item Our approach, leveraging smaller language models, approximates and even surpasses the performance of GPT-4-turbo with a 128K context window, demonstrating a David-versus-Goliath dynamic, as well as scalability in handling text length.
\item In addressing long text issues, our approach leverages the LLM with 4K context window, achieving performance on par with or even exceeding that of LLM with 128K context window.
\vspace{-0.08cm}
\item Experimental results show that \ourmethod achieves superior performance in single-hop and multi-hop long context tasks. Notably, Info-Graph Agent achieves a xx of xx on HotpotQA, xx on 2WikiMultiHopQA, and xx on MuSiQue based on GPT-4 with 4K context window, even outperforming GPT-4-turbo with 128K context window.
\end{itemize}


==> content/cache/intro_cache2.tex <==
%-----注释过多的版本放在了cache的intro cache2中

\section{Introduction}

Large language models~(LLMs) have made great progress on natural language understanding and generation~\citep{Zhao-2023-arxiv-survey}. However, transformer-based LLMs still struggle in handling long contexts due to the limitation of context window and memory usage. 
% Thus concerns about improving the long-context capabilities of LLMs have drawn significant attention from the research community~\citep{}.


Current techniques for improving the long-context capabilities of LLMs can be divided into two perspectives: 1) Model-level, which includes fine-tuning on target long-context data~\cite{chen2023extending,fu2024data,bai2024longalign}, positional extrapolation or interpolation without training~\cite{su2024roformer,ding2024longrope,peng2023yarn}, and applying transformer variants with modified attention mechanisms~\citep{dai2019transformer,munkhdalai2024leave,gu2023mamba}; 2) Agent-level, \aka employing retrieval-augmented LLM or agent to process long contexts with a limited context window LLM~\cite{nakano2021webgpt,lee2024human}.
Model-level methods typically train LLMs with target length texts, posing challenges in constructing training datasets and incurring high training costs~\cite{zhu2023pose}. Additionally, long-context LLMs optimized with these methods tend to overlook crucial details in long contexts, known as ``lost in the middle''~\cite{liu2024lost}, limiting their ability to address complex tasks, such as multi-hop questions. Agent-level approaches transform input text into a tree~\citep{chen2023walking} or paginated pages~\citep{lee2024human}, failing to capture multi-hop and long-range dependencies, thus limiting their effectiveness on very long contexts, as shown in Figure~\ref{fig: motivation}.

% The model-level methods typically rely on training with texts of the target length~\citep{}, which results in the challenge of constructing training datasets and incurs high training costs. Furthermore, long-context LLMs optimized with these three methods tend to overlook crucial details in long contexts, \aka lost in the middle~\cite{liu2024lost}, limiting handling multi-hop problems of long-context LLMs. Agent-level approaches transform the input text into paginated pages~\citep{lee2024human} or a tree~\citep{chen2023walking}, which fail to support the agents in capturing multi-hop and long-range dependencies, thus limiting the effectiveness of these methods.


\ignore{
We draw inspiration from the cognitive processes that humans employ for reading comprehension of long texts in the real world. When tackling long-text QA problems, humans typically divide the process into four-stage process:(1) understanding the question and reasoning the key information to answer it; (2) identifying several key terms based on the question; (3) searching the content in long text related to the selected key terms; and (4) integrating the gathered information to generate the response of the question. Drawing on these insights, we propose \textbf{\ourmethod}, a novel approach that organizes information from long text into a graph, and employ an agent to travel on the graph based on the input question to search and summarize information within the graph as needed. Specifically, we first segment long texts into chunks, followed by extracting key elements and atomic facts from them. Then we construct a graph with these key elements as nodes and incorporating atomic facts and original chunks as their content to model the global information of input long text. Lastly, our \ourmethod performs a depth-first search from the selected initial nodes. It dynamically reads, accumulates memories, and concludes, responding interactively to user input until it gathers enough information to fulfill the given question.
}
\begin{figure}[t]
    \centering
    % \setlength{\abovecaptionskip}{0.15cm}  
    % \setlength{\belowcaptionskip}{-0.2cm}
    \includegraphics[width=0.99\linewidth]{source/figure1.pdf}
    \caption{Performance on LV-Eval at 5 context length level. GraphReader outperforms existing open-sourced and close-sourced models while demonstrating a scalable performance in very long contexts. In contrast, other models exhibit a significant decrease in performance as context length increase.}
    \label{fig: motivation}
    % \vspace{-4mm}
\end{figure}


To address these issues, we propose a graph-based agent named \textbf{\ourmethod}. As illustrated in Figure~\ref{fig: ourmethod}, \ourmethod first segment long texts into discrete chunks, extract essential information, and compresses these into key elements and atomic facts. They are then used to construct a graph with nodes representing key elements and their associated content derived from atomic facts. This graph structure effectively captures long-range dependencies and multi-hop relationships within long text.
Subsequently, \ourmethod autonomously explores this graph using predefined functions, guided by a step-by-step rational path. Based on a given question, the agent progressively accesses information from coarse key elements and atomic facts to detailed original text chunks, taking notes and reflecting until it gathers sufficient information to generate an answer.
In summary, our main contributions are threefold:

\begin{itemize}[leftmargin=4mm]
\vspace{-0.08cm}
% \item We propose \ourmethod, a novel agent system that uses a memory mechanism and graph-driven traversal to handle long-context tasks with limited context window LLMs, achieving performance comparable to or exceeding that of LLMs with a 128K context window.
% \vspace{-0.08cm}
% % \item Our approach, leveraging smaller language models, approximates and even surpasses the performance of GPT-4-turbo with a 128K context window, demonstrating a David-versus-Goliath dynamic, as well as scalability in handling text length.
% \item In addressing long text issues, our approach leverages the LLM with 4K context window, achieving performance on par with or even exceeding that of LLM with 128K context window.
\vspace{-0.08cm}
% \item Experimental results show that \ourmethod achieves superior performance in single-hop and multi-hop long context tasks. Notably, Info-Graph Agent achieves a xx of xx on HotpotQA, xx on 2WikiMultiHopQA, and xx on MuSiQue based on GPT-4 with 4K context window, even outperforming GPT-4-turbo with 128K context window.
\item We introduce \ourmethod, a novel agent system designed to organize long texts into a graph structure, leveraging predefined functions and notebook to facilitate planning and reflection during exploration.%, thereby enabling the effective handling of long-context tasks.

\item \ourmethod establishes a scalable long-context capability based on a 4k context window, demonstrating performance that is comparable to or surpasses GPT-4 with a 128k context window across varying context lengths.

\item Extensive experiments conducted on four challenging banchmarks demonstrate that \ourmethod achieves superior performance in complex single-hop and multi-hop QA tasks.
\end{itemize}






% draft
% Large language models~(LLMs) have made great progress on natural language understanding and generation~\citep{Zhao-2023-arxiv-survey}. However, transformer-based LLMs still struggle in handling long contexts due to the limitation of context window and memory usage. 


% Current work primarily implemented four strategies to improve the capability of LLMs in processing long context: finetuning with modified positional embeddings~\cite{chen2023extending}, training directly on long-context data, applying transformer variants with modified attention mechanisms~\citep{} and employing agent to process long contexts with the limited context window LLM~\cite{wu2020memformer, lee2024human}. Despite the effectiveness, there are several shortcomings in these four methods. For the first three methods, they typically rely on training with texts of the target length~\citep{}, which results in the challenge of constructing training datasets and incurs high training costs. Furthermore, long-context LLMs optimized with these three methods tend to overlook crucial details in long contexts, \aka lost in the middle~\cite{liu2024lost}, limiting handling multi-hop problems of long-context LLMs. For approaches that employ agents to handle long context input, typically, they transform the input text into paginated pages~\citep{lee2024human} or a tree~\citep{chen2023walking}, which fail to support the agents in capturing multi-hop and long-range dependencies, thus limiting the effectiveness of these methods.


% \ignore{
% We draw inspiration from the cognitive processes that humans employ for reading comprehension of long texts in the real world. When tackling long-text QA problems, humans typically divide the process into four-stage process:(1) understanding the question and reasoning the key information to answer it; (2) identifying several key terms based on the question; (3) searching the content in long text related to the selected key terms; and (4) integrating the gathered information to generate the response of the question. Drawing on these insights, we propose \textbf{\ourmethod}, a novel approach that organizes information from long text into a graph, and employ an agent to travel on the graph based on the input question to search and summarize information within the graph as needed. Specifically, we first segment long texts into chunks, followed by extracting key elements and atomic facts from them. Then we construct a graph with these key elements as nodes and incorporating atomic facts and original chunks as their content to model the global information of input long text. Lastly, our \ourmethod performs a depth-first search from the selected initial nodes. It dynamically reads, accumulates memories, and concludes, responding interactively to user input until it gathers enough information to fulfill the given question.
% }

% To address these issues, in this paper, we propose a method that extracts critical information from long texts and organizes it into a graph, subsequently employing an agent for interactive reading input long text and follow user instructions, namely \textbf{\ourmethod}. Specifically, as illustrated in Figure~\ref{}, our method comprises two main stages: Firstly, we divide the long text into multiple chunks, followed by extracting key information from these chunks. Secondly, we construct a graph wherein key information as nodes and incorporating original chunks as nodes' content. Through this structure, we achieve modeling the long-range dependencies and multi-hop relation within the key information of input long text. Secondly, the \ourmethod employs pre-planned strategies to conduct a depth-first search from multiple initial nodes within the graph. Based on user input, it interactively reads, generates memory, responding interactively to user input until it gathers enough information to fulfill the given question.


% In summary, our main contributions are as follows:
% \begin{itemize}[leftmargin=4mm]
% \vspace{-0.08cm}
% \item We propose \ourmethod, a novel agent system that utilizes a memory mechanism and graph-driven traversal to handle long-context tasks with limited context window LLMs.
% \vspace{-0.08cm}
% % \item Our approach, leveraging smaller language models, approximates and even surpasses the performance of GPT-4-turbo with a 128K context window, demonstrating a David-versus-Goliath dynamic, as well as scalability in handling text length.
% \item In addressing long text issues, our approach leverages the LLM with 4K context window, achieving performance on par with or even exceeding that of LLM with 128K context window.
% \vspace{-0.08cm}
% \item Experimental results show that \ourmethod achieves superior performance in single-hop and multi-hop long context tasks. Notably, Info-Graph Agent achieves a xx of xx on HotpotQA, xx on 2WikiMultiHopQA, and xx on MuSiQue based on GPT-4 with 4K context window, even outperforming GPT-4-turbo with 128K context window.
% \end{itemize}
\section{Experiments}


\subsection{Experimental Settigns}

\paragraph{Evaluation Benchmarks} We conduct experiments on two types of long-context QA benchmarks, including multi-hop long-context QA, \ie, HotpotQA~\citep{yang-2018-emnlp-hotpotqa}, 2WikiMultihopQA~\citep{ho-2020-coling-2wikimultihopQA}, MuSiQue~\citep{Trivedi-2022-acltrans-musique}, and a single-hop long-context QA benchmark, NarrativeQA~\citep{Kocisky-2018-acltrans-narrativeqa}. Additionally, we also incorporate HotpotWikiQA-mixup from LV-Eval~\citep{Yuan2024LVEvalAB}, a multi-hop benchmark that features five levels of text length: 16k, 32k, 64k, 128k, and 256k, reaching a maximum length of 370.8k. The statistical information about these benchmarks is presented in Table~\ref{tab: datasets} and detailed information is provided in Appendix~\ref{app: datasets}.


\paragraph{Evaluation Metrics} We employ several automatic evaluation metrics, \ie $F_1$ score, Exact Match (EM) score, and an optimized $F_1$* score, as introduced by LV-Eval~\cite{Yuan2024LVEvalAB}. Specifically, $F_1$* first computes the recall of golden answer keywords and only calculates the $F_1$ score if it exceeds a certain threshold, otherwise, the score defaults to zero. Despite the cost-effectiveness of automatic metrics, their accuracy may be affected by the response format. Hence we implement LLM Raters for answer correctness evaluation using an LLM, denoted as LLM-Rating-1 (LR-1) and LLM-Rating-1 (LR-2), as demonstrated by ReadAgent~\citep{lee2024human}. Comprehensive details on the evaluation metrics can be found in Appendix \ref{app: eval_details}.

\ignore{
\paragraph{Baseline Methods} We compare \ourmethod with three types of baseline methods: model-level, retrieval-level, and agent-level methods, described as follows:

\begin{itemize}[leftmargin=4mm]
\vspace{-0.08cm}
\item \textbf{Model-level Methods} utilize long-context LLM GPT-4-128k for direct full-text reading when the text content fits within the input window or segmenting the text into chunks for sequential reading.

\item \textbf{Retrieval-level Methods} utilize Okapi BM25~\citep{Robertson2009ThePR} or OpenAI API embedding model Ada-002\footnote{https://platform.openai.com/docs/guides/embeddings/\linebreak embedding-models} to retrieve the chunks most relevant to the question and employ LLM to read retrieved chunks and answer the question.

\item \textbf{Agent-level Methods} employ ReadAgent~\citep{lee2024human} for long-context QA, which employs an agent-based system for the execution of retrieval and reading processes.

\end{itemize}

The detailed description and implementation of these methods are provided in Appendix~\ref{app: baseline}.
}


\paragraph{Baseline Methods} We compare \ourmethod with three types of baseline methods: model-level, retrieval-level, and agent-level methods. \textbf{Model-level Methods} utilize long-context LLM GPT-4-128k for direct full-text reading when the text content fits within the input window or segmenting the text into chunks for sequential reading. \textbf{Retrieval-level Methods} utilize Okapi BM25~\citep{Robertson2009ThePR} or OpenAI API embedding model Ada-002\footnote{https://platform.openai.com/docs/guides/embeddings/\linebreak embedding-models} to retrieve the chunks most relevant to the question and employ LLM to read retrieved chunks and answer the question. \textbf{Agent-level Methods} employ ReadAgent~\citep{lee2024human} for long-context QA, which employs an agent-based system for the execution of retrieval and reading processes. The detailed description and implementation of these methods are provided in Appendix~\ref{app: baseline}.

\paragraph{Implementation Details}

In our experiments, we employ the GPT-4 (gpt-4-1106-preview) for both our method and baseline approaches, setting the temperature to 0.2. 
%GPT-4 supports 128k tokens input and can generate 4k tokens.
When deploying \ourmethod, unless otherwise specified, we configure the input window size to 4k tokens, set the maximum length of chunk to 2k tokens, initiate searches from 5 initial nodes, and impose a function call limit of 10 for each search path.

\begin{table}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrr}
\bottomrule
                  \textbf{Task} & \textbf{Dataset}  & Avg \#Tokens & Max \#Tokens & \#Samples  \\ \hline
\multirow{4}{*}{\textbf{Multi-hop QA}} & HotpotQA  & 9.4k & 15.9k & 300  \\
                     & 2WikiMultihopQA  & 8.8k & 15.9k & 300 \\
                    & MuSiQue  & 15.5k & 16.0k & 200 \\
                    & HotpotWikiQA-mixup  & 142.4k & 370.8k & 250 \\ \hline
% \multirow{1}{*}{\textbf{Single-hop QA}} &narrativeQA & English & 29.7k & 200 
\textbf{Single-hop QA} & NarrativeQA  & 29.7k & 63.7k & 200 \\\bottomrule
\end{tabular}
}
\caption{
The statistical information of benchmarks employed in our evaluation. The token number is calculated using the GPT-4 tokenizer from the TikToken\protect\footnotemark. \#Samples denotes the total number of benchmarks.
}
\label{tab: datasets}
\end{table}
\footnotetext{https://github.com/openai/tiktoken}



%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{lcrrrr|rrrr|rrrr|rrrr}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \textbf{Input} & \multicolumn{4}{c}{\textbf{HotpotQA}} & \multicolumn{4}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{4}{c}{\textbf{MuSiQue}} &  \multicolumn{4}{c}{\textbf{NarrativeQA}}\\ \cline{3-18}
     & \textbf{Window} & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$ & LR-1 & LR-2 & EM & $F_1$\\ \hline
     % \multicolumn{18}{l}{BM25(top-1)} \\ \hline
    BM25 (top-1) & 4k & 57.7 & 63.0 & 33.7 & 43.8 & 36.0 & 39.0 & 25.0 & 30.4 & 33.0 & 36.5 & 19.0 & 23.9 & 29.5 & 34.5 & 4.0 & 11.3 \\
    BM25 (top-3) & 4k & 74.7 & 78.3 & 45.7 & 58.5 & 59.7 & 62.0 & 42.3 & 51.9 & 43.5 & 49.5 & 25.0 & 31.1 & 44.5 & 52.5 & 7.0 & 20.5 \\ \hline
% \multicolumn{18}{l}{OpenAI Embedding Retrieval} \\ \hline
    Ada-002 (top-1) & 4k & 63.0 & 70.7 & 40.0 & 53.2 & 57.0 & 59.3 & 41.0 & 49.4 & 34.5 & 37.0 & 20.0 & 26.6 & 37.5 & 46.5 & 5.0 & 15.5 \\
    Ada-002 (top-3) & 4k & 72.0 & 77.3 & 45.0 & 58.1 & 65.7 & 66.7 & 44.7 & 55.3 & 40.0 & 45.5 & 24.5 & 32.1 & 45.5 & 53.0 & 7.5 & 19.5 \\ \hline
    GPT-4-128k & $128k$ & \underline{83.3} & \underline{88.3} & \underline{53.0} & \underline{68.4} & 77.3 & 80.0 & \underline{58.7} & \underline{70.0} & 52.0 & 59.5 & 33.5 & 42.7 & \underline{63.5} & \underline{77.0} & \underline{11.5} & \underline{29.4}  \\
    GPT-4-128k (chunk) & $4k$ & 71.3 & 74.7 & 45.7 & 59.5 & 59.3 & 62.3 & 40.7 & 50.5 & 41.0 & 43.0 & 23.0 & 32.1 & 58.0 & 69.5 & 9.50 & 25.5  \\
    GPT-4-128k (chunk w/ notes) & $4k$ & 72.3 & 76.7 & 45.7 & 59.5 & 65.7 & 68.7 & 46.3 & 56.6 & 39.5 & 43.0 & 25.0 & 32.5 & 56.5 & 65.0 & 8.5 & 24.3  \\\hline
    ReadAgent & \redtext{$128k$} & 72.3 & 78.7 & 48.0 & 62.0 & \underline{79.0} & \underline{81.0} & 52.7 & 63.7 & \underline{54.5} & \underline{61.0} & \underline{35.0} & \underline{45.1} & 63.0 & 75.5 & 5.0 & 18.9 \\ 
    \ourmethod & $4k$ &\textbf{84.3} & \textbf{89.7} & \textbf{55.0} & \textbf{70.0} & \textbf{83.7} & \textbf{87.0} & \textbf{59.3} & \textbf{70.1} & \textbf{59.0} & \textbf{63.5} & \textbf{38.0} & \textbf{47.4} & \textbf{65.0} & \textbf{80.0} & \textbf{15.5} & \textbf{29.8} \\
    \hline
    Golden & $4k$ & 92.3 & 93.7 & 57.0 & 73.8 & 88.3 & 89.7 & 63.0 & 73.4 & 66.0 & 69.0 & 45.0 & 56.0 & - & - & - & - \\  \hline
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) of different baselines on datasets from LongBench. The best performance and the second-best performance are denoted in bold and underlined fonts, respectively. Golden denotes the settings that we add question and its supporting facts to LLM directly.}
% \vspace{-0.5cm}
\label{tab: main_result_1}
\end{table*}
%---------------------------------------------------------
 % \multirow{4}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}}} \\
 % & & & & & & & & & & & & & & & & \\
 % & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
%---------------------------------------------------------
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.1}
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lcrrr|rrr|rrr|rrr|rrr}
\hline
 \multirow{3}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input}} & \multicolumn{15}{c}{\textbf{HotpotWikiQA-mixup}} \\\cline{3-17}
 & \multirow{2}{*}{\textbf{Window}} & \multicolumn{3}{c}{\textbf{16k}} & \multicolumn{3}{c}{\textbf{32k}} & \multicolumn{3}{c}{\textbf{64k}} & \multicolumn{3}{c}{\textbf{128k}} & \multicolumn{3}{c}{\textbf{256k}} \\ \cline{3-17}
& & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$* & LR-1 & LR-2 & $F_1$*\\ \hline
% \multicolumn{17}{l}{BM25 Retrieval} \\ \hline
    BM25 (top-1) & $4k$ & 10.0 & 16.0 & 12.0 & 16.0 & 18.0 & 11.9 & 6.0 & 8.0 & 8.5 & 10.0 & 8.0 & 7.0 & 14.0 & 20.0 & 5.9 \\
    BM25 (top-3) & $4k$ & 16.0 & 22.0 & 13.9 & 18.0 & 28.0 & 13.3 & 16.0 & 18.0 & 11.8 & 12.0 & 16.0 & 11.8 & 12.0 & 22.0 & 9.3 \\ \hline
% \multicolumn{17}{l}{OpenAI Embedding Retrieval} \\ \hline
    Ada-002 (top-1) & $4k$ & 10.0 & 12.0 & 14.5 & 14.0 & 18.0 & 11.3 & 10.0 & 12.0 & 12.5 & 12.0 & 14.0 & 9.4 & 8.0 & 8.0 & 7.0 \\
    Ada-002 (top-3) & $4k$ & 24.0 & 28.0 & 21.3 & 20.0 & 30.0 & 19.8 & 14.0 & 20.0 & 12.9 & 16.0 & 20.0 & 12.0 & 14.0 & 18.0 & 10.8 \\  \hline
    GPT-4-128k & $128k$ & {\underline {38.0}} & {\underline {38.0}} & {\underline {35.7}} & {\underline {26.0}} & {\underline {30.0}} & {\underline {26.0}} & 22.0 & 24.0 & 20.6 & 16.0 & 16.0 & 14.6 & 14.0 & 16.0 & 10.3 \\
    GPT-4-128k (chunk) & $4k$ & 18.0 & 22.0 & 24.6 & 16.0 & 20.0 & 17.7 & 20.0 & 24.0 & 17.0 & 20.0 & 24.0 & 14.7 & {\underline {28.0}} & {\underline {30.0}} & 10.7 \\
    GPT-4-128k (chunk w/ notes) & $4k$ & 22.0 & 32.0 & 24.2 & 26.0 & 30.0 & 21.3 & {\underline {28.0}} & {\underline {32.0}} & {\underline {22.0}} & {\underline {24.0}} & {\underline {26.0}} & {\underline {17.4}} & 26.0 & 26.0 & {\underline {14.8}} \\
    ReadAgent & \redtext{$128k$} & 24.0 & 26.0 & 29.2 & 20.0 & 22.0 & 16.9 & 24.0 & 30.0 & 15.3 & 14.0 & 18.0 & 13.6 & 20.0 & 22.0 & 10.4 \\
    \ourmethod & $4k$ & \textbf{42.0} & \textbf{42.0} & \textbf{38.2} & \textbf{32.0} & \textbf{38.0} & \textbf{36.4} & \textbf{30.0} & \textbf{36.0} & \textbf{32.9} & \textbf{28.0} & \textbf{34.0} & \textbf{30.6} & \textbf{30.0} & \textbf{38.0} & \textbf{33.0} \\
\hline
\end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance~(\%) of different baselines on datasets from LV-Eval, where $F_1$* donates LV-Eval's optimized $F_1$. The best performance and the second-best performance are denoted in bold and underlined fonts, respectively. We truncate to keep the longest possible initial fragment while preserving paragraph structure, in contexts that exceed the input window ($128k$ and $256k$) for GPT-4-128k.}
% \vspace{-0.5cm}
\label{tab: main_result_2}
\end{table*}
%---------------------------------------------------------
\subsection{Main Results}

In this part, we conduct a series of experiments on multi-hop and single-hop long-context QA tasks. 


\paragraph{Evaluation on Single- and Multi-hop Long-context Tasks} The results of three types of methods on three multi-hop long-context QA and one single-hop long-context QA are shown in Tabel~\ref{tab: main_result_1}. Based on the results, we have the following findings:

Firstly, we observe that sparse retrieval BM25 and dense retrieval Ada-002 exhibit the worst performance in comparison to model-level and agent-level approaches. A possible reason is that text retrieval fails to recall all documents that contain the supporting facts for answering the input question. Although increasing the quantity of recalled documents could improve text retrieval's performance, the constrained context window LLM restricts the number of documents that can be read, thereby limiting the effectiveness of these retrieval-level methods. 

Secondly, we see that employing GPT-4-128k for direct reading of long texts significantly outperforms retrieval-level methods, and even outperforms ReadAgent on three long-context benchmarks. This is because of the superior performance of GPT-4-128k in processing long texts and executing multi-hop reasoning. Additionally, the lengths of these four benchmarks are significantly shorter than 128k context window, thereby mitigating the impact of ``lost in the middle'' on the model's performance. Moreover, we also observe that GPT-4, despite having a constrained 4k context window, can process input contexts that significantly exceed its context window limitations through sequential reading and still outperform retrieval-based methods. Furthermore, incorporating a memory module into sequential reading with LLM can significantly improve the performance of sequential reading on multi-hop benchmarks. The reason may be that carrying memory with history information can facilitate LLM in aggregating previously missed supporting facts. Conversely, for the single-hop benchmark, NarrativeQA, integrating memory results in performance degradation. The reason may be that previous memory introduces noise to LLM and affects its responses. 

Thirdly, we can also see that the previous agent-level method ReadAgent demonstrates impressive performance in these four long-context benchmarks. This is because the agent-level method introduces diverse actions, memory, and reflection in reading strategies, which fully harnesses LLM's reasoning ability. However, even the effectiveness, ReadAgent slightly underperforms GPT-4-128k full-text reading. We attribute this to the ReadAgent's strategy, which relies on summarizing each page, leveraging past memories, and analyzing the input question to select pages for gathering supporting information. This approach may restrict the agent's ability to identify specific details and capture long-range dependencies in long context, consequently affecting its overall performance.


Finally, by comparing our approach with all baselines, it is obvious that our approach performs consistently better them on four long-context benchmarks and demonstrates more superior performance in multi-hop QA than sing-hop QA. In our approach, we transform long context into key elements and atomic facts，which are subsequently organized into a graph. Benefiting from the graph's ability to capture the relationships between detailed information, our method can identifies crucial information and search the supporting facts for the input question efficiently. This strategy significantly boosts the agent's capability in multi-hop reasoning and capturing long-range dependencies of key information in long context. And we observe that the performance of our method closely matches that achieved by directly supplying supporting facts to the LLM (\ie Golden in Table~\ref{tab: main_result_1}). This is because our method not only incorporates pre-planning, reflection, and various actions but also the usage of a graph containing key information, facilitating the agent to search for the correct supporting facts. Additionally, it is noteworthy that our method, employing merely a 4k context window, outperforms ReadAgent's 128k context window setup. It further indicates that our approach can more efficiently unlock the capabilities of constrained context window LLMs in processing long context.


%正如之前的实验，我们发现我们的方法在多跳和单跳长文本任务上均取得了成功。这里我们we would like to study the effectiveness of our approach on the更长的长文本benchmark上的表现。如表3结果所示，相比于baseline中其他方法，我们的方法在16k to 256k的所有长度任务上表现都会更好。这进一表明了我们的方法在面对超长文本时，仍然可以通过构建图的方式，使得短窗口的大语言模型处理超长文本。首先作为对比，我们可以看到随着窗口长度增加，gpt-4-128k full text reading的性能逐渐下降，而采用了我们的方法后，在16k长度时，LR-1性能增益仅有21%，而当长度增加到128k时，使用我们方法，性能增益达到了56%。这是因为随着长度增加，gpt-4受到lost in the middle影响会逐渐加重。而我们的方法并不会受到文本长度变长时表现地更加鲁棒。第二，我们看到readagent在长文本上表现明显差于我们的方法，这可能是因为，readagent在处理超长文本时需要同时决策阅读哪些页，由于缺乏每一页内容细粒度信息，这使得readagent难以收集更多关于问题的证据。这进一步表明了我们方法通过构建图并在图上探索的方法可以有效的完成超长文本的问题，并展现了可以扩展到更长文本上的可能性。

\paragraph{Evaluation on Ultra-long Context Tasks} As shown in previous experiments, it demonstrates the  utility of employing a limited context window LLM for long-context QA with our \ourmethod. Here, we would like to study the effectiveness of our approach on the longer multi-hop long-context QA tasks. As shown in Table~\ref{tab: main_result_2}, compared with all baselines, our \ourmethod not only consistently outperforms these methods across text lengths ranging from 16k to 256k tokens but also exhibits robustness with the expansion of context length. It further indicates that our method remains effective in handling ultra-long texts by constructing graphs and graph exploration, thereby allowing constrained context window LLMs to process extensive texts efficiently. As a comparison, we can see that with the increase in the length of the input context, the performance of GPT-4-128k full-text reading  degrades gradually. However, employing our method, at context length of 16k, the LR-1 performance gain is merely 10.53\%, whereas by extending the context length to 128k, our method achieves a performance gain of 75.00\%. This can be attributed to the fact that as the context length increases, the impact of the ``lost in the middle'' effect on GPT-4-128k becomes progressively more severe. Secondly, we observe that ReadAgent significantly underperforms our method in handling long contexts. This is because that ReadAgent's need to make decisions about which pages to read when dealing with long context. The lack of detailed information on the content of each page makes it challenging for ReadAgent to gather more evidence relating to the input question. This further demonstrates that our method, by constructing and exploring graphs, can effectively address the challenges of processing ultra-long context with limited context window LLMs.






\ignore{
Table \ref{tab: main_result_1} reports the main results of \ourmethod compared with other baselines across different datasets. Our method outperforms all baseline methods across various evaluation metrics on all assessed datasets. 
The impressive performance of \ourmethod on both single-hop and multi-hop datasets demonstrates its superiority and robustness in managing a variety of long text QA scenarios. 

The RAG methods (BM25 Retrieval and OpenAI Embedding Retrieval) perform the worst, and although selecting more fragments can lead to improved results, the limitations of the input window make it still difficult to outperform the other methods.

For the results of Chunk Read, the method with memory performs better on multi-hop QA datasets than the method without memory because carrying memory evidently makes it easier to gather multiple supporting facts. However, on single-hop QA datasets, the latter performs better. This could be due to the additional memory introducing confusion.

The Full Text Read method obtains decent results on several datasets, showcasing the strong capabilities of LLMs in handling QA tasks with context lengths smaller than the input window.
Nevertheless, it is still surpassed by \ourmethod, proving the superiority of our approach in processing long context within a limited input window.

Additionally, we explored the performance of \ourmethod on texts of different lengths, from $16k$ to $256k$. Table \ref{tab: main_result_2} presents the results on different metrics for the HotpotWikiQA-mixup dataset, where the context lengths vary. Our method surpasses all baselines across all lengths (from $16k$ to $256k$). It is noteworthy that using a tokenizer from GPT-4, the maximum context length can reach up to $370k$ (as shown in Table \ref{tab: datasets}), which is nearly a hundred times the size of our employed input window ($4k$).
The experimental results from Table \ref{tab: main_result_2} verify that the capability of our method to handle long contexts extends beyond the limitations of the 4k input window, highlighting our approach's advanced capabilities in managing extremely long contexts.
}
% Table \ref{tab: main_result_1} and Table \ref{tab: main_result_2} report the main results compared with other baselines on different datasets.
% As shown in Table \ref{tab: main_result_1}, our method outperforms all baseline methods on different evaluation metrics for all evaluation datasets, proving the effectiveness of our method. In particular, our method achieves excellent results on both single-hop and multi-hop datasets, demonstrating its robustness in managing diverse long-context QA scenarios.

% Table \ref{tab: main_result_2} showcases the results of different metrics on the HotpotWikiQA-mixup dataset with varying lengths of context. Our method outperforms all baselines across all lengths from 16k to 256k. Notably, utilizing the tokenizer from gpt-4, the maximum context length reaches up to 370k (as shown in Table \ref{tab: datasets}).
% % , which is nearly a hundred times greater than the input window (4k). This demonstrates the superiority of our approach in handling exceptionally long contexts.
% The capability of \ourmethod in handling long contexts is significantly beyond the limitation of the 4k input window, highlighting our method's advanced proficiency in handling extremely lengthy contexts.

% As shown in Table \ref{tab: main_result_1}, \ourmethod outperforms all baseline methods across all evaluation metrics, particularly on multi-hop datasets such as HotpotQA, 2WikiMultihopQA, and MuSiQue, demonstrating the superiority of our approach in dealing with multi-hop QA. 

% The experimental results of different methods on datasets from LongBench are presented in Table \ref{tab: main_result_1}. Our \ourmethod achieved the best performance across all evaluation metrics, particularly on the multi-hop datasets such as HotpotQA, 2WikiMultihopQA, and MuSiQue, demonstrating the superiority of our approach in dealing with multi-hop QA. Furthermore, \ourmethod also exhibits advantages on the single-hop QA dataset (NarrativeQA), reflecting the effectiveness of our approach in pinpointing fine-grained information. 
% It is worth noting that \ourmethod surpassed Full Text Read to varying extents, strongly proving the effectiveness of our approach.



% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccccccccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input Window}} & \multicolumn{3}{c}{\textbf{HotpotQA}} & \multicolumn{3}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{3}{c}{\textbf{MuSiQue}} &  \multicolumn{3}{c}{\textbf{NarrativeQA}}\\ \cline{3-14} 
%      & & LR-1 & LR-2 & $F_1$ & LR-1 & LR-2 & $F_1$ & LR-1 & LR-2 & $F_1$ & LR-1 & LR-2 & $F_1$\\ \hline
%     w/o pp. & $4k$ & 0.817 & 0.877 & 0.109 & 0.823 & 0.860 & 0.146 & 0.560 & 0.610 & 0.082 & 0.630 & 0.785 &  0.100 \\
%     w/o mem. & $4k$ &  &  &  &  &  &  &  &  &  &  &  &   \\
%     w/o both & $4k$ &  &  &  &  &  &  &  &  &  &  &  &   \\
%     Info-Graph Agent & $4k$ &\textbf{0.843} & \textbf{0.897} & 0.190 & \textbf{0.837} & \textbf{0.870} & \textbf{0.258} & \textbf{0.590} & \textbf{0.635} & \textbf{0.156} & \textbf{0.650} & \textbf{0.800} & 0.160  \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Ablation study on datasets from LongBench.}
% % \vspace{-0.5cm}
% \label{ablation}
% \end{table*}
%---------------------------------------------------------
%---------------------------------------------------------
% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{4}{c}{\textbf{\#Initial Nodes}}\\ \cline{3-6} 
%        &  & 4 & 7 & 10 & 13 \\ \hline
    
%     \multirow{2}{*}{\textbf{2WikiMultihopQA}} & LR-1 & 74.3 & 81.7 & 83.7 & \textbf{85.0} \\
%         & LR-2 & 76.3 & 83.7 & \textbf{87.0} & 85.7 \\\hline

%     \multirow{2}{*}{\textbf{NarrativeQA}} & LR-1 & 57.5 & 58.0 & \textbf{65.0} & 58.5 \\
%         & LR-2 & 71.5 & 73.0 & \textbf{80.0} & 73.5 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Performance(\%) of \ourmethod with changes in the initial nodes. The best are in bold.}
% % \vspace{-0.5cm}
% \label{tab: starting_nodes}
% \end{table}

% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{4}{c}{\textbf{\#Initial Nodes}}\\ \cline{3-6} 
%        &  & 1 & 4 & 7 & 10 \\ \hline
    
%     \multirow{2}{*}{\textbf{2WikiMultihopQA}} & LR-1 & 79.3 & 81.7 & 83.7 & \textbf{85.0} \\
%         & LR-2 & 81.3 & 84.7 & \textbf{87.0} & 85.7 \\\hline

%     \multirow{2}{*}{\textbf{NarrativeQA}} & LR-1 & 59.5 & 62.0 & \textbf{65.0} & 61.5 \\
%         & LR-2 & 74.5 & 76.0 & \textbf{80.0} & 75.5 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Performance(\%) of \ourmethod with changes in the initial nodes. The best are in bold.}
% % \vspace{-0.5cm}
% \label{tab: starting_nodes}
% \end{table}
%---------------------------------------------------------
\begin{table}[!t]
\centering
% \scriptsize
\resizebox{\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Results(\%)}}\\ \cline{3-5} 
     & & LR-1 & LR-2 & $F_1$ \\ \hline
    \multirow{3}{*}{\textbf{HotpotQA}} & \ourmethod & \textbf{84.3} & \textbf{89.7} & \textbf{70.0} \\
        & w/o rational plan & 81.7 & 87.7 & 63.8 \\
        & w/o node selection & 66.0 & 71.7 & 54.1 \\\hline
    \multirow{3}{*}{\textbf{2WikiMultihopQA}}& \ourmethod & \textbf{83.7} & \textbf{87.0} & \textbf{70.1} \\
        & w/o rational plan & 81.3 & 86.0 & 65.4 \\
        & w/o node selection & 65.3 & 68.7 & 49.7 \\\hline
    \multirow{3}{*}{\textbf{MuSiQue}} & \ourmethod & \textbf{59.0} & \textbf{63.5} & \textbf{47.4} \\
    & w/o rational plan & 56.0 & 61.0 & 42.4 \\
    & w/o node selection & 35.0 & 38.5 & 25.2 \\\hline
    \multirow{3}{*}{\textbf{NarrativeQA}} & \ourmethod & \textbf{65.0} & \textbf{80.0} & \textbf{29.8}  \\
        & w/o rational plan & 63.0 & 78.5 & 26.6 \\
        & w/o node selection & 53.0 & 65.5 & 24.0 \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{The results of our ablation experiments, where ``w/o rational plan'' refers to removing the pre-planning stage, and ``w/o node selection'' denotes the random selection of initial nodes and neighbor nodes.}
% \vspace{-0.5cm}
\label{tab: ablation}
\end{table}
%---------------------------------------------------------
\subsection{Ablation study}
We construct ablation experiments on various datasets to investigate the contribution of different components in our approach. 

\paragraph{Effects of Rational Plan.}
To evaluate the Rational Plan's effectiveness, we remove our method's pre-planning stage, and the results are shown in Table \ref{tab: ablation}. We can find that excluding the rational path leads to a deterioration in \ourmethod's performance, thus confirming the rational plan's beneficial impact on \ourmethod. We can infer that the pre-planning stage enables \ourmethod to deal with various complex questions effectively.

\paragraph{Effects of Graph-Based Agent.}
On the other hand, to prove that the model chooses which nodes to visit based on reasoning about the information needed, we conduct experiments under settings with randomly selecting initial nodes. As shown in Table \ref{tab: ablation}, Setting to random selection results in the significant performance degradation of our approach, with results across all datasets declining by an average of 18\%. This indicates that \ourmethod indeed exhibits intelligence in its exploration process on the graph, selecting nodes through the reasoning ability of the accumulated information rather than engaging in arbitrary exploration dependent on the chance to collect supporting facts.

% On the other hand, to prove that the model is really thinking about the information needed to choose which nodes to visit, we conduct experiments under settings with randomly choosing initial nodes and randomly replacing the parameter when selecting the read\_neighbor\_node function from candidate neighbor nodes.When \ourmethod no longer autonomously selects nodes but instead wanders randomly, its performance significantly decreases. This indicates that \ourmethod indeed exhibits intelligence in its exploration process on the memory graph, choosing nodes based on the information acquired so far rather than aimlessly wandering and relying on randomness to collect supporting facts.
% We implement without rational plan experiments by removing the pre-planning stage . Without node selection refers to the elimination of the agent's autonomy in selecting initial and neighbor nodes, switching to random selection instead. Specifically, a random selection from all nodes is made for the initial nodes. When the agent chooses to read neighbor nodes, the model-selected neighbor node is replaced with a randomly chosen one from all neighbor nodes.
% Table \ref{tab: ablation} displays the results of our ablation experiments, where w/o pre-planning refers to the removal of the pre-planning stage. In fact, we set the plan to be fixed as "There is no plan to solve this question." W/o select refers to the elimination of the agent's autonomy in selecting starting and neighbor nodes, switching to random selection instead. Specifically, a random selection from all nodes is made for the starting nodes. When the agent chooses to read neighbor nodes, the model-selected neighbor node is replaced with a randomly chosen one from all neighbor nodes. In summary, w/o select implements a form of random walk. 

% The experimental results shown in Table \ref{tab: ablation} illustrate that the performance of \ourmethod declines when pre-planning is removed, and the decline is more significant on multi-hop QA datasets than on single-hop QA datasets, indicating the beneficial role of pre-planning in aiding the agent to pinpoint critical information. When the agent no longer selects nodes autonomously but instead wanders randomly, the performance of \ourmethod significantly drops. This demonstrates that \ourmethod does not merely search for information by traversing all chunks but intelligently selects the next node based on current memory and historical actions.
%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/figure3.pdf}
% \vspace{-0.6cm}
\caption{Performance of \ourmethod with different initial node numbers on 2WikiMultihopQA and NarrativeQA. Results show the robustness of \ourmethod towards different initial node numbers.}
\label{fig: nodes}
% \vspace{-0.6cm}
\end{figure}
%---------------------------------------------------------
\subsection{Further Analysis}
\paragraph{Impact of the Number of Initial Nodes}
To assess the effect of the number of initial nodes on \ourmethod's performance, we conduct experiments setting different numbers of initial nodes on both multi-hop and single-hop QA datasets, and the results are shown in Figure \ref{fig: nodes}. Firstly, we can find the performance of \ourmethod changes slightly with the number of initial nodes, showing strong robustness to it. Secondly, within a certain range, an increase in the number of nodes leads to a slight improvement in model performance and the performance is relatively optimal when the initial number of nodes is set to 5, hence we choose this as our default initial node setting. However, surpassing a certain threshold, \ourmethod's performance tends to decline. Notably, this decrement is more apparent in single-hop scenarios. We can consider that this is because more noise interferes with the model by an excessive number of initial nodes.

For multi-hop QA, having a sufficient number of starting nodes is crucial. For example, in questions involving comparisons, the objects to be compared are often difficult to associate on the memory graph. In such cases, selecting a starting node for each object becomes particularly important for searching for enough information to answer the question adequately.
% To investigate the impact of the number of initial nodes on the outcomes, we conducted experiments using datasets from both multi-hop QA and single-hop QA. The experimental results shown in Table \ref{tab: starting_nodes}  reveal that when the number of initial nodes is too low, the performance of \ourmethod improves with an increase in the number of initial nodes. However, the final QA performance slightly declines when the number of initial nodes is excessive. We believe this is due to the overabundance of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of initial nodes is more pronounced for single-hop QA.

% Table \ref{tab: starting_nodes} showcases the impact of different numbers of starting nodes, which are the number of search paths, on the final outcome. We selected one dataset each from multi-hop QA and single-hop QA datasets for experimentation to explore their respective effects on multi-hop QA and single-hop QA. The experimental results reveal that when the number of starting nodes is too low, the performance of \ourmethod improves with an increase in the number of starting nodes. However, the final QA performance slightly declines when the number of starting nodes is excessive. We believe this is due to the overabundance and disorganization of different paths' memories, confusing the model. This phenomenon was indeed observed in actual tests. The decline in performance caused by an excessive number of starting nodes is more pronounced for single-hop QA.
%---------------------------------------------------------
% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \hline
    
%     \textbf{Dataset} & \textbf{Avg Action Num(per trace)} & \textbf{Stage} & \textbf{Total Ratio} & \textbf{Selected Action} & \textbf{Selection Ratio}\\ \hline
%      % \multirow{7}{*}{\textbf{MuSiQue}} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{3}{*}{read_chunk} & \multirow{3}{*}{0.312(2185/7002)}
%      \multirow{7}{*}{MuSiQue} & \multirow{7}{*}{3.501(7002/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.312(2185/7002)} & \textit{search\_more}s & 0.191(417/2185)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.266(582/2185) \\ 
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.257(561/2185) \\
%     &  &  &  & \textit{stop} & 0.286(625/2185) \\  \cline{3-6}
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.400(2800/7002)} & \textit{read\_chunk} & 0.413(1156/2800) \\ 
%     &  &  &  & \textit{stop} & 0.587(1644/2800) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.288(2017/7002)} & \textit{read\_neighbor\_node} & 0.401(809/2017)  \\ 
%     &  &  &  & stop & 0.599(1208/2017) \\ \hline
% \multirow{7}{*}{NarrativeQA} & \multirow{7}{*}{3.8475(7695/2000)} & \multirow{4}{*}{read\_chunk}     & \multirow{3}{*}{0.543(4176/7695)} & \textit{search\_more} & 0.041(171/4176)  \\
%     &  &  &  & \textit{read\_previous\_chunk} & 0.353(1475/4176) \\
%     &  &  &  & \textit{read\_subsequent\_chunk} & 0.326(1360/4176) \\
%     &  &  &  & \textit{stop} & 0.280(1170/4176) \\ 
%     \cline{3-6} 
%     &  & \multirow{2}{*}{read\_claims} & \multirow{2}{*}{0.325(2502/7695)} & \textit{read\_chunk} & 0.645(1615/2502) \\  
%     &  &  &  & \textit{stop} & 0.355(887/2502) \\ \cline{3-6} 
%     &  & \multirow{2}{*}{read\_neighbors} & \multirow{2}{*}{0.132(1017/7695)} & \textit{read\_neighbor\_node} & 0.514(523/1017)  \\
%     &  &  &  & \textit{stop} & 0.486(494/1017)  \\
%     \hline
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Action statistics of \ourmethod on two datasets.}
% % \vspace{-0.5cm}
% \label{tab: action}
% \end{table*}
\begin{table*}[!t]
\centering
% \scriptsize
\resizebox{\textwidth}{!}{
    \begin{tabular}{cccccr}
    \toprule
    \textbf{Dataset} & \textbf{\#Avg. Function Call} & \textbf{Stage} & \textbf{Stage Ratio(\%)} & \textbf{Function} & \textbf{Call Ratio(\%)}\\ \hline

    % \multirow{7}{*}{HotpotQA} & \multirow{7}{*}{3.0} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{42.0} & \textit{read\_chunk} & 46.5 \\ 
    % &  &  &  & \textit{stop\_and\_read\_neighbor} & 53.5 \\ \cline{3-6} 
    % & & \multirow{4}{*}{Exploring Chunks}     & \multirow{4}{*}{31.9} & \textit{search\_more} & 19.1  \\
    % &  &  &  & \textit{read\_previous\_chunk} & 26.6 \\ 
    % &  &  &  & \textit{read\_subsequent\_chunk} & 25.7 \\
    % &  &  &  & \textit{termination} & 28.6 \\  \cline{3-6}
    % &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{26.1} & \textit{read\_neighbor\_node} & 40.1 \\
    % &  &  &  & \textit{termination} & 59.9\\ \hline

    \multirow{7}{*}{2WikiMultihopQA} & \multirow{7}{*}{3.2} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{40.4} & \textit{read\_chunk} & 48.6 \\  
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 51.4 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks} & \multirow{4}{*}{34.5} & \textit{search\_more} & 14.5 \\
    &  &  &  & \textit{read\_previous\_chunk} & 25.1 \\
    &  &  &  & \textit{read\_subsequent\_chunk} & 23.3 \\
    &  &  &  & \textit{termination} & 37.1 \\ 
    \cline{3-6} 
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{25.1} & \textit{read\_neighbor\_node} & 37.3  \\
    &  &  &  & \textit{termination} & 62.7  \\\hline
 
     \multirow{7}{*}{MuSiQue} & \multirow{7}{*}{3.5} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{40.0} & \textit{read\_chunk} & 41.3 \\ 
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 58.7 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks}     & \multirow{4}{*}{31.2} & \textit{search\_more} & 19.1  \\
    &  &  &  & \textit{read\_previous\_chunk} & 26.6 \\ 
    &  &  &  & \textit{read\_subsequent\_chunk} & 25.7 \\
    &  &  &  & \textit{termination} & 28.6 \\  \cline{3-6}
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{28.8} & \textit{read\_neighbor\_node} & 40.1 \\
    &  &  &  & \textit{termination} & 59.9\\ \hline
\multirow{7}{*}{NarrativeQA} & \multirow{7}{*}{3.9} & \multirow{2}{*}{Exploring Atomic Facts} & \multirow{2}{*}{32.5} & \textit{read\_chunk} & 64.5 \\  
    &  &  &  & \textit{stop\_and\_read\_neighbor} & 35.5 \\ \cline{3-6} 
    & & \multirow{4}{*}{Exploring Chunks} & \multirow{4}{*}{54.3} & \textit{search\_more} & 4.1 \\
    &  &  &  & \textit{read\_previous\_chunk} & 35.3 \\
    &  &  &  & \textit{read\_subsequent\_chunk} & 32.6 \\
    &  &  &  & \textit{termination} & 28.0 \\ 
    \cline{3-6} 
    &  & \multirow{2}{*}{Exploring Neighbors} & \multirow{2}{*}{13.2} & \textit{read\_neighbor\_node} & 51.4  \\
    &  &  &  & \textit{termination} & 48.6  \\
    
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
\caption{Statistics of function calls on MuSiQue and NarrativeQA.}
% \vspace{-0.5cm}
\label{tab: action}
\end{table*}
%---------------------------------------------------------
% \begin{table*}[!t]
% \centering
% % \scriptsize
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Avg Ctx. Tokens}} & \multirow{2}{*}{\textbf{Chunk Limit}} & \multirow{2}{*}{\textbf{Token Type}} & \multicolumn{2}{c}{\textbf{Stage}} \\ \cline{5-6} 
%        & & &  & avg atomic facts and key elements tokens & avg agent tokens \\\hline
%     \multirow{8}{*}{\textbf{HotpotWikiQA-mixup-256k}} & \multirow{8}{*}{366950.70} & \multirow{2}{*}{1k} & input token & 585770.34 & 90624.49   \\
%         & & & output token & 270179.60 &  13558.30 \\\cline{4-6}
        
%     & & \multirow{2}{*}{2k} & input token & 465931.14 & 69821.40 \\
%         & & & output token & 156201.42 & 11057.36  \\\cline{4-6}

%         & & \multirow{2}{*}{4k} & input token & 417449.46 & 93083.31   \\
%         & & & output token & 142652.42 & 10939.20  \\\cline{4-6}

%         & & \multirow{2}{*}{6k} & input token & 400457.94 & 76402.95  \\
%         & & & output token & 131023.17 & 9625.54 \\
       
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{Consumption statistics of \ourmethod on two datasets. The input window is set to 4k, with 7 starting nodes, and a maximum of 10 actions. The upper limit of text fragments is 2k.}
% % \vspace{-0.5cm}
% \label{tab: cost}
% \end{table*}
%--------------------------------------------------------------
%---------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=0.8\linewidth]{source/figure4.pdf}
% \vspace{-0.2cm}
\caption{The impact of chunk size $L$ of \ourmethod on the 256k length level of HotpotWikiQA-mixup.}
\label{fig: chunk_size_exp}
% \vspace{-0.2cm}
\end{figure}
%---------------------------------------------------------
\paragraph{Impact of the Chunk Size}

To explore the impact of the chunk size $L$ on the performance of \ourmethod, we set up multiple sets of comparative experiments with different chunk sizes. As shown in Figure \ref{fig: chunk_size_exp}, the results show that the best performance was achieved when $L=2k$. Initially, We find that when $L$ exceeds a certain threshold, the bigger the chunk size, the more obvious the performance decline trend. We infer that this corresponds to the model performance degradation on longer texts mentioned earlier, where the model is prone to overlooking essential details. Moreover, when $L$ is too small, more semantic truncation occurs, hampering the model's comprehension of the current context and 
further affecting the accuracy of extracting atomic facts. So, we finally choose $L=2k$ as our default chunk size setting.

%When $L$ is smaller, it is evident that more resources are consumed during the construction phase of the memory graph. Thus, to balance performance and consumption, a larger and more effective $L$ should be selected as the hyperparameter setting as much as possible.

% To balance consumption and performance, we think $L=2k$ is a good setting.
% To investigate the impact of input window size on \ourmethod, we conducted experiments on HotpotWikiQA-mixup-256k. We used different input window sizes, and the results in Figure \ref{fig: chunk} indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects one action: during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.

% Table \ref{tab: input_window} demonstrates the impact of the input window size on \ourmethod. To facilitate the testing of larger input windows, we conducted experiments on HotpotWikiQA-mixup-256k. The experimental results indicate that increasing the input window size from 4k to 32k does not significantly alter the outcomes. In fact, when the upper limit of text fragments is fixed at 2k, enlarging the input window only affects three actions: less pagination when searching for starting nodes, reading more nodes at once; during the reading of atomic facts, more atomic facts can be read with fewer being filtered out due to similarity; and similarly, when reading neighboring nodes. Therefore, the insignificant variation in experimental results with increasing input window size suggests that: 1. When searching for starting nodes, reading more nodes does not pose significant difficulty for the agent, indicating that the agent has the capability to select starting nodes from a large number of nodes. 2. When reading atomic facts and neighboring nodes, similarity filtering effectively extracts relevant content.
%---------------------------------------------------------
% \begin{table}[!t]
% \centering
% % \scriptsize
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccc}
%     \bottomrule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Input Window}} & \multicolumn{2}{c}{\textbf{Metrics}}\\ \cline{3-4} 
%        &  & LR-1 & LR-2 \\ \hline
    
%     \multirow{4}{*}{\textbf{HotpotWikiQA-mixup-256k}} & 4k & 30.0 & 38.0 \\
%         & 8k & \textbf{32.0} & \textbf{40.0} \\
%         & 16k & 32.0 & 38.0 \\
%         & 32k & 28.0 & 36.0 \\
%     \bottomrule
%     \end{tabular}
% }
% % \vspace{-0.2cm}
% \caption{The impact of the input window size.}
% % \vspace{-0.5cm}
% \label{tab: input_window}
% \end{table}
%---------------------------------------------------------
\begin{table}[!t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc}
\toprule
    Method & Avg. Ctx. Tokens & Avg. Token Consumption \\\hline
    ReadAgent & 366,950.7 & 49,906.7  \\
    \ourmethod & 366,950.7 & 54,056.3 \\\bottomrule
    \end{tabular}
}
\caption{Comparison of token consumption per question between ReadAgent and \ourmethod on HotpotWikiQA-mixup-256k, where Consumption Tokens comprise both input tokens and output tokens. The ``Avg. Ctx. Tokens'' refers to the average number of context tokens from the original dataset.}
\label{tab: consumption}
\end{table}
%--------------------------------------------------------------------------
\paragraph{The Analysis of Function Calls}
%这块是证明我们设计的动作的合理性和有用性，同时资源消耗较少，不会跳来跳去

To verify the rationality and utility of agent actions under various circumstances of \ourmethod, we made statistics on its function calls at each stage across two datasets. 
From the statistical results in Table \ref{tab: action}, it can be observed that each piece of data will perform an average of 3 to 4 actions, corresponding to the average number of function calls in the table. This indicates the effectiveness of the graph we constructed, with \ourmethod being able to swiftly locate key information while minimizing resource usage. 
Furthermore, each action has a certain probability of being chosen, justifying the rationality of the action set. Among them, the most commonly used action on multi-hop QA tasks is to read neighbor nodes, and the most common action on single-hop QA tasks is to read chunks. This difference is caused by the fact that multi-hop questions need to gather information contained by multiple nodes to answer questions, while single-hop data sets often require only one atomic fact.
%--------------------------------------------------------------------------
\paragraph{Consumption Analysis}
We assessed the average token consumption by ReadAgent and \ourmethod in answering a question, with the results presented in Table \ref{tab: consumption}. \ourmethod requires slightly more tokens to answer a question compared to ReadAgent. Despite a minor increase in consumption, \ourmethod achieves significantly better results than ReadAgent, favorably demonstrating the superiority of our method.

It can also be observed that the average tokens consumed by these two methods to answer a question are significantly less than the average context tokens, indicating that this approach of pre-processing the context has a notable advantage when dealing with multiple QA scenarios.
%--------------------------------------------------------------
\begin{figure}[!t]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.3cm}  
% \resizebox{0.48\textwidth}{!}{}
\includegraphics[width=1\linewidth]{source/recall.pdf}
% \vspace{-0.6cm}
\caption{Recall of supporting facts by different methods on HotpotWikiQA-mixup.}
\label{fig: recall}
% \vspace{-0.6cm}
\end{figure}
%--------------------------------------------------------------
\begin{table}[!t]
\centering
% \scriptsize
\resizebox{0.75\columnwidth}{!}{
    \begin{tabular}{ccc}
    \bottomrule
    \multirow{2}{*}{\textbf{Source}}  & \multicolumn{2}{c}{\textbf{Recall(\%)}} \\ \cline{2-3} 
     &  by supporting fact & by case \\ \hline
    Atomic Facts & 76.4 & 64.7 \\
    Final Notebook & 90.5 & 85.3  \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
% \caption{\ourmethod's recall of supporting facts at various stages. Define a partial\_ratio similarity greater than $0.8$ as a successful recall. We use \textit{gpt-4-1106-preview} for evaluation, with the temperature set to 0.1.}
\caption{\ourmethod's recall of supporting facts at various stages. Statistical dimensions: ``by supporting fact'' refers to individual atomic facts; ``by case'' refers to all atomic facts for a QA pair.}
\label{tab: recall}
\end{table}
%--------------------------------------------------------------
\paragraph{Recall Rate Analysis}
To better evaluate the advantage of our method in pinpointing critical information, we used LLMs to assess the recall of supporting facts for various methods on the HotpotWikiQA-mixup dataset. The specific evaluation approach is described in Appendix \ref{app: recall}.

The evaluation results shown in Figure \ref{fig: recall} demonstrate that \ourmethod far surpasses other baseline methods in terms of the recall of supporting facts, proving the superiority of our approach. Besides, we notice that as the context length increases (from $16k$ to $256k$), the recall of supporting facts for all methods declines, with ReadAgent experiencing a particularly rapid decrease, while \ourmethod shows a very slow decline. This indicates that \ourmethod has excellent scalability in handling long texts.

We calculate the recall rate of \ourmethod at various stages using the same method, and Table \ref{tab: recall} presents the experimental results. The recall rate of supporting facts during the Answer Reasoning stage is slightly higher than that of the Memory Graph, indicating that \ourmethod has the ability to supplement and extract valid information from chunks during the exploration process, indirectly showcasing its intelligence and efficiency in exploration.
% To better assess the advantages of our method in identifying key information, we utilized the supporting facts that support answering questions from the HotpotQA dataset. We analyzed \ourmethod's recall of supporting facts at various stages on the HotpotQA dataset.

% Table \ref{recall} presents the experimental results of the recall analysis for \ourmethod, where the two stages of evaluation are specifically: atomic facts extracted from the text and the final memory obtained. The evaluation was conducted using LLM (\textit{gpt-4-1106-preview}, with the specific evaluation prompt shown in Figure \ref{recall_prompt}). The statistics were compiled based on supporting facts (by supporting fact) and by individual cases (by case), where "by supporting fact" refers to whether that supporting fact was recalled, and "by case" indicates whether all supporting facts for a given case were fully recalled.

% The results indicate that under the same LLM evaluation method (with identical prompts), the final memory's recall rate for supporting facts is higher compared to the recall rate for atomic facts. Furthermore, the gap between this recall rate aligns with the assessment results of the LLM-Raters (Figure \ref{tab: main_result_2}, LR-1: 0.843; LR-2: 0.897). This demonstrates \ourmethod's capability to locate corresponding supporting facts from weakly related nodes.
%--------------------------------------------------------------



